A Dynamic Stochastic Block Model for Multidimensional Networks

The availability of relational data can offer new insights into the functioning of the economy. Nevertheless, modeling the dynamics in network data with multiple types of relationships is still a challenging issue. Stochastic block models provide a parsimonious and flexible approach to network analysis. We propose a new stochastic block model for multidimensional networks, where layer-specific hidden Markov-chain processes drive the changes in community formation. The changes in the block membership of a node in a given layer may be influenced by its own past membership in other layers. This allows for clustering overlap, clustering decoupling, or more complex relationships between layers, including settings of unidirectional, or bidirectional, non-linear Granger block causality. We address the overparameterization issue of a saturated specification by assuming a Multi-Laplacian prior distribution within a Bayesian framework. Data augmentation and Gibbs sampling are used to make the inference problem more tractable. Through simulations, we show that standard linear models and the pairwise approach are unable to detect block causality in most scenarios. In contrast, our model can recover the true Granger causality structure. As an application to international trade, we show that our model offers a unified framework, encompassing community detection and Gravity equation modeling. We found new evidence of block Granger causality of trade agreements and flows and core-periphery structure in both layers on a large sample of countries.

==> Tables/App_MCMC_conn_res0.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:33:04 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters} 
\label{tab: MCMCcon}
\begin{tabular}{ccccccccc}
  \hline
Parameters & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0.52 & 0.01 & 0 & 18929.93 & 0.24 & 0.54 & 0 & 3787 \\ 
  $\alpha^{(1)}_{2}$ & 0.52 & 0.01 & 0 & 18929.93 & 0.24 & 0.54 & 0 & 3787 \\ 
  $\nu^{(1)}_{11}$ & 0 & 0.18 & 0.11 & 5158.4 & 0.61 & 0.71 & 0 & 8336 \\ 
  $\nu^{(1)}_{21}$ & 0 & 0.27 & 0.14 & 3413.82 & 0.23 & 0.53 & 0 & 9616 \\ 
  $\nu^{(1)}_{12}$ & 0 & 0.3 & 0.17 & 3452.71 & 0.9 & 0.77 & 0 & 14361 \\ 
  $\nu^{(1)}_{22}$ & 0 & 0.07 & 0.02 & 10898.23 & 0.63 & 0.78 & 0 & 3906 \\ 
  $\beta^{(1)}_{0,11}$ & 0 & 0.09 & 0.04 & 10073.09 & 0.8 & 0.8 & 0 & 3897 \\ 
  $\beta^{(1)}_{0,21}$ & 0 & 0.04 & 0.01 & 13613.34 & 0.71 & 0.56 & 0 & 3913 \\ 
  $\beta^{(1)}_{0,12}$ & 0 & 0.05 & 0.03 & 14087.14 & 0.34 & 0.84 & 0 & 3897 \\ 
  $\beta^{(1)}_{0,22}$ & 0 & 0.06 & 0.02 & 14056.69 & 0.65 & 0.58 & 0 & 3842 \\ 
  $\beta^{(1)}_{1,11}$ & 0.03 & 0.01 & 0 & 19433.19 & 0.38 & 0.57 & 0 & 3740 \\ 
  $\beta^{(1)}_{1,21}$ & 0 & 0.03 & 0.01 & 14468.94 & 0.42 & 0.81 & 0 & 3929 \\ 
  $\beta^{(1)}_{1,12}$ & 0 & 0.04 & 0.01 & 14460.63 & 0.73 & 0.87 & 0 & 3849 \\ 
  $\beta^{(1)}_{1,22}$ & 0 & 0.05 & 0.04 & 11315.65 & 0.63 & 0.75 & 0 & 3771 \\ 
  $\beta^{(1)}_{2,11}$ & 0 & 0.13 & 0.06 & 6809.35 & 0.36 & 0.97 & 0 & 3994 \\ 
  $\beta^{(1)}_{2,21}$ & 0.01 & 0.02 & 0.01 & 17974.37 & 0.19 & 0.62 & 0 & 3881 \\ 
  $\beta^{(1)}_{2,12}$ & 0 & 0.05 & 0.01 & 12138.36 & 0.05 & 0.24 & 0 & 3913 \\ 
  $\beta^{(1)}_{2,22}$ & 0 & 0.07 & 0.03 & 9878.97 & 0.15 & 0.15 & 0 & 3897 \\ 
  $\beta^{(1)}_{3,11}$ & 0 & 0.03 & 0.01 & 16882.38 & 0.11 & 0.43 & 0 & 3771 \\ 
  $\beta^{(1)}_{3,21}$ & 0 & 0.04 & 0.02 & 13191.57 & 0.19 & 0.71 & 0 & 4112 \\ 
  $\beta^{(1)}_{3,12}$ & 0 & 0.05 & 0.02 & 14457.71 & 0.39 & 0.39 & 0 & 3945 \\ 
  $\beta^{(1)}_{3,22}$ & 0 & 0.08 & 0.05 & 10379.59 & 0.01 & 0.1 & 0 & 3849 \\ 
  $\sigma^{(1)2}_{11}$ & 0.68 & 0.01 & 0 & 18987.71 & 0.79 &  &  & 3834 \\ 
  $\sigma^{(1)2}_{21}$ & 0 & 0.07 & 0.04 & 12057.65 & 0.93 &  &  & 3897 \\ 
  $\sigma^{(1)2}_{12}$ & 0 & 0.05 & 0.02 & 12419.52 & 0.43 &  &  & 3850 \\ 
  $\sigma^{(1)2}_{22}$ & 0 & 0.26 & 0.15 & 3673.68 & 0.28 &  &  & 9412 \\ 
  $\alpha^{(2)}_{1}$ & 0.32 & 0 & 0 & 20000 & 0.68 & 0.64 & 0 & 3802 \\ 
  $\alpha^{(2)}_{2}$ & 0.32 & 0 & 0 & 20000 & 0.68 & 0.64 & 0 & 3802 \\ 
  $\nu^{(2)}_{11}$ & 0.03 & -0.01 & 0.01 & 19721.19 & 0.56 & 0.26 & 0 & 3725 \\ 
  $\nu^{(2)}_{21}$ & 0.59 & 0 & 0.01 & 20000 & 0.94 & 0.28 & 0 & 3771 \\ 
  $\nu^{(2)}_{12}$ & 0.74 & 0.01 & -0.01 & 20000 & 0.06 & 0.08 & 0 & 3802 \\ 
  $\nu^{(2)}_{22}$ & 0.54 & 0 & 0 & 20000 & 0.59 & 0.47 & 0 & 3802 \\ 
  $\rho^{(1)}$ & 0 & 0.42 & 0.09 & 5649.62 & 0.51 & 0.62 & 0.02 & 10466 \\ 
  $\rho^{(2)}$ & 0 & 0.39 & 0.09 & 4500.16 & 0.76 & 0.42 & 0.02 & 10910 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_conn_res0_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:33:04 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters} 
\label{tab: MCMCcon}
\begin{tabular}{ccccccccc}
  \hline
Parameters & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0.73 & 0.03 & 0 & 2000 & 0.25 & 0.86 & 0 &  \\ 
  $\alpha^{(1)}_{2}$ & 0.73 & 0.03 & 0 & 2000 & 0.25 & 0.86 & 0.01 &  \\ 
  $\nu^{(1)}_{11}$ & 0.49 & 0.06 & 0 & 1771.83 & 0.68 & 0.76 & 0 &  \\ 
  $\nu^{(1)}_{21}$ & 0 & 0.11 & 0.04 & 1610.96 & 0.09 & 0.79 & 0 &  \\ 
  $\nu^{(1)}_{12}$ & 0.01 & 0.09 & 0 & 1677.26 & 0.48 & 0.14 & 0 &  \\ 
  $\nu^{(1)}_{22}$ & 0.36 & 0.03 & 0 & 1875.84 & 0.86 & 0.87 & 0 &  \\ 
  $\beta^{(1)}_{0,11}$ & 0 & 0.02 & -0.04 & 19621.8 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,21}$ & 0 & -0.03 & 0.04 & 13129.56 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,12}$ & 0 & 0.01 & 0.01 & 24373.01 & 0.99 & 0.99 & 0 &  \\ 
  $\beta^{(1)}_{0,22}$ & 0 & -0.01 & -0.02 & 17440.61 & 0.97 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,11}$ & 0 & -0.04 & -0.01 & 17473.13 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,21}$ & 0 & 0 & 0.04 & 15483.93 & 0.99 & 0.87 & 0 &  \\ 
  $\beta^{(1)}_{1,12}$ & 0 & 0.05 & -0.03 & 29075.77 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,22}$ & 0 & 0.03 & 0.01 & 19648.49 & 0.97 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,11}$ & 0 & 0.06 & -0.02 & 29114.97 & 1 & 0.99 & 0 &  \\ 
  $\beta^{(1)}_{2,21}$ & 0 & -0.03 & 0.01 & 13228.07 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,12}$ & 0 & 0.02 & 0.02 & 13560.93 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,22}$ & 0 & -0.03 & -0.04 & 25009.48 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,11}$ & 0 & 0.03 & -0.02 & 15142.02 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,21}$ & 0 & -0.03 & 0.01 & 26064.87 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,12}$ & 0 & 0.01 & 0.03 & 35430.37 & 0.99 & 0.9 & 0 &  \\ 
  $\beta^{(1)}_{3,22}$ & 0 & 0.03 & 0.01 & 16406.26 & 0.99 & 1 & 0 &  \\ 
  $\sigma^{(1)2}_{11}$ & 0.45 & 0.02 & -0.02 & 2000 & 0.84 &  &  &  \\ 
  $\sigma^{(1)2}_{21}$ & 0.91 & -0.01 & -0.02 & 2000 & 0.91 &  &  &  \\ 
  $\sigma^{(1)2}_{12}$ & 0.38 & 0 & -0.02 & 2000 & 0.06 &  &  &  \\ 
  $\sigma^{(1)2}_{22}$ & 0 & 0.08 & -0.03 & 1421.79 & 0.24 &  &  &  \\ 
  $\alpha^{(2)}_{1}$ & 0.84 & 0.02 & 0.01 & 2000 & 0.63 & 0.13 & 0.01 &  \\ 
  $\alpha^{(2)}_{2}$ & 0.84 & 0.02 & 0.01 & 2000 & 0.63 & 0.13 & 0 &  \\ 
  $\nu^{(2)}_{11}$ & 0.59 & -0.03 & 0 & 2134.11 & 0.44 & 0.79 & 0 &  \\ 
  $\nu^{(2)}_{21}$ & 0.68 & 0.01 & -0.02 & 2000 & 0.66 & 0.98 & 0 &  \\ 
  $\nu^{(2)}_{12}$ & 0.19 & 0.01 & 0.01 & 1861.87 & 0.26 & 0.28 & 0 &  \\ 
  $\nu^{(2)}_{22}$ & 0.98 & -0.02 & -0.01 & 2000 & 0.2 & 0.71 & 0 &  \\ 
  $\rho^{(1)}$ & 0.62 & 0.03 & 0.01 & 1871.45 & 0.36 & 0.86 & 0.04 &  \\ 
  $\rho^{(2)}$ & 0.04 & 0.07 & 0.01 & 1733.36 & 0.31 & 0.37 & 0.04 &  \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_conn_res1.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:36:57 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters} 
\label{tab: MCMCcon}
\begin{tabular}{ccccccccc}
  \hline
Parameters & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0.12 & 0.02 & -0.01 & 19171.7 & 0.44 & 0.73 & 0 & 3802 \\ 
  $\alpha^{(1)}_{2}$ & 0.12 & 0.02 & -0.01 & 19171.7 & 0.44 & 0.73 & 0 & 3802 \\ 
  $\nu^{(1)}_{11}$ & 0 & 0.08 & 0.04 & 11401.28 & 0.65 & 0.99 & 0 & 3865 \\ 
  $\nu^{(1)}_{21}$ & 0 & 0.28 & 0.16 & 3402.42 & 0.03 & 0.22 & 0 & 14445 \\ 
  $\nu^{(1)}_{12}$ & 0 & 0.34 & 0.19 & 2899.18 & 0.05 & 0.19 & 0 & 11895 \\ 
  $\nu^{(1)}_{22}$ & 0 & 0.24 & 0.14 & 3727.11 & 0.31 & 0.6 & 0 & 8242 \\ 
  $\beta^{(1)}_{0,11}$ & 0 & 0.07 & 0.03 & 11011.73 & 0.92 & 0.56 & 0 & 3849 \\ 
  $\beta^{(1)}_{0,21}$ & 0 & 0.05 & 0.02 & 12600.4 & 0.01 & 0.12 & 0 & 3849 \\ 
  $\beta^{(1)}_{0,12}$ & 0 & 0.05 & 0.03 & 12448.23 & 0.08 & 0.22 & 0 & 3834 \\ 
  $\beta^{(1)}_{0,22}$ & 0 & 0.08 & 0.03 & 11861.81 & 0.9 & 0.67 & 0 & 3913 \\ 
  $\beta^{(1)}_{1,11}$ & 0 & 0.07 & 0.03 & 10887.99 & 0.6 & 0.83 & 0 & 3834 \\ 
  $\beta^{(1)}_{1,21}$ & 0 & 0.05 & 0.02 & 14564.92 & 0.08 & 0.71 & 0 & 3849 \\ 
  $\beta^{(1)}_{1,12}$ & 0 & 0.04 & 0.02 & 14727.83 & 0.38 & 0.21 & 0 & 3834 \\ 
  $\beta^{(1)}_{1,22}$ & 0 & 0.01 & 0.02 & 17937.67 & 0.62 & 0.58 & 0 & 3787 \\ 
  $\beta^{(1)}_{2,11}$ & 0 & 0.1 & 0.05 & 8012.31 & 0.52 & 0.7 & 0 & 3978 \\ 
  $\beta^{(1)}_{2,21}$ & 0 & 0.05 & 0.03 & 11220.83 & 0.21 & 0.56 & 0 & 3818 \\ 
  $\beta^{(1)}_{2,12}$ & 0 & 0.03 & 0.01 & 13254.78 & 0.08 & 0.07 & 0 & 3849 \\ 
  $\beta^{(1)}_{2,22}$ & 0 & 0.11 & 0.05 & 8724.36 & 0.42 & 0.72 & 0 & 4061 \\ 
  $\beta^{(1)}_{3,11}$ & 0 & 0.12 & 0.06 & 6951.15 & 0.09 & 0.25 & 0 & 3945 \\ 
  $\beta^{(1)}_{3,21}$ & 0 & 0.06 & 0.02 & 14012.83 & 0.08 & 0.28 & 0 & 3818 \\ 
  $\beta^{(1)}_{3,12}$ & 0 & 0.06 & 0.04 & 9652.02 & 0.93 & 0.45 & 0 & 3826 \\ 
  $\beta^{(1)}_{3,22}$ & 0 & 0.03 & 0.01 & 18574.69 & 0.2 & 0.64 & 0 & 3802 \\ 
  $\sigma^{(1)2}_{11}$ & 0 & 0.29 & 0.18 & 3222.14 & 0.49 &  &  & 12291 \\ 
  $\sigma^{(1)2}_{21}$ & 0 & 0.07 & 0.04 & 9626.63 & 0.17 &  &  & 3849 \\ 
  $\sigma^{(1)2}_{12}$ & 0 & 0.09 & 0.06 & 8173.24 & 0.35 &  &  & 3834 \\ 
  $\sigma^{(1)2}_{22}$ & 0.16 & 0.01 & 0.01 & 19137.21 & 0.2 &  &  & 3818 \\ 
  $\alpha^{(2)}_{1}$ & 0.42 & 0.01 & 0 & 20000 & 0.51 & 0.86 & 0 & 3755 \\ 
  $\alpha^{(2)}_{2}$ & 0.73 & 0.01 & 0.01 & 19579.54 & 0.79 & 0.53 & 0 & 3802 \\ 
  $\alpha^{(2)}_{3}$ & 0.66 & 0 & 0 & 19521.66 & 0.4 & 0.12 & 0 & 3710 \\ 
  $\alpha^{(2)}_{4}$ & 0.76 & 0 & 0 & 20000 & 0.12 & 0.05 & 0 & 3849 \\ 
  $\nu^{(2)}_{11}$ & 0 & 0.21 & 0.14 & 1496.84 & 0.95 & 0.75 & 0 & 8916 \\ 
  $\nu^{(2)}_{21}$ & 0 & 0.21 & 0.21 & 211.32 & 0.82 & 0.09 & 0.01 & 123318 \\ 
  $\nu^{(2)}_{31}$ & 0 & 0.12 & 0.11 & 1031.01 & 0.49 & 0.6 & 0 & 28805 \\ 
  $\nu^{(2)}_{41}$ & 0.69 & 0 & 0 & 20000 & 0.97 & 0.07 & 0 & 3756 \\ 
  $\nu^{(2)}_{12}$ & 0 & 0.2 & 0.18 & 245.58 & 0.08 & 0.09 & 0.01 & 132432 \\ 
  $\nu^{(2)}_{22}$ & 0 & 0.21 & 0.09 & 4987.24 & 0.54 & 0.4 & 0 & 4197 \\ 
  $\nu^{(2)}_{32}$ & 0 & 0.55 & 0.55 & 29.22 & 0.64 & 0.22 & 0.01 & 208796 \\ 
  $\nu^{(2)}_{42}$ & 0.85 & 0 & 0 & 20000 & 0.55 & 0.19 & 0 & 3725 \\ 
  $\nu^{(2)}_{13}$ & 0 & 0.13 & 0.06 & 8127.17 & 0.07 & 0.47 & 0 & 7548 \\ 
  $\nu^{(2)}_{23}$ & 0 & 0.21 & 0.09 & 6486.91 & 0.97 & 0.67 & 0 & 4012 \\ 
  $\nu^{(2)}_{33}$ & 0.55 & 0.01 & 0 & 19544.49 & 0.74 & 0.99 & 0 & 3834 \\ 
  $\nu^{(2)}_{43}$ & 0.66 & 0 & -0.01 & 20000 & 0.45 & 0.82 & 0 & 3755 \\ 
  $\nu^{(2)}_{14}$ & 0.36 & 0.01 & -0.01 & 20000 & 0.15 & 0.7 & 0 & 3802 \\ 
  $\nu^{(2)}_{24}$ & 0 & 0.04 & 0.01 & 13616.42 & 0.18 & 0.56 & 0 & 3913 \\ 
  $\nu^{(2)}_{34}$ & 0.87 & 0.01 & 0.01 & 20000 & 0.84 & 0.89 & 0 & 3787 \\ 
  $\nu^{(2)}_{44}$ & 0.27 & -0.01 & 0.01 & 21158.04 & 0.67 & 0.8 & 0 & 3755 \\ 
  $\rho^{(1)}$ & 0 & 0.49 & 0.1 & 4813.16 & 0.03 & 0.06 & 0.02 & 9256 \\ 
  $\rho^{(2)}$ & 0 & 0.68 & 0.36 & 1388.76 & 0.05 & 0.26 & 0.03 & 89925 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_conn_res1_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:36:58 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters} 
\label{tab: MCMCcon}
\begin{tabular}{ccccccccc}
  \hline
Parameters & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0.07 & 0.02 & 0.02 & 2084.93 & 0.71 & 0.9 & 0.01 &  \\ 
  $\alpha^{(1)}_{2}$ & 0.07 & 0.02 & 0.02 & 2084.93 & 0.71 & 0.9 & 0 &  \\ 
  $\nu^{(1)}_{11}$ & 0.23 & 0.02 & 0 & 2000 & 0.14 & 0.21 & 0 &  \\ 
  $\nu^{(1)}_{21}$ & 0.01 & 0.07 & -0.01 & 1730.94 & 0.1 & 0.24 & 0 &  \\ 
  $\nu^{(1)}_{12}$ & 0 & 0.12 & -0.03 & 1566.32 & 0.03 & 0.4 & 0 &  \\ 
  $\nu^{(1)}_{22}$ & 0.13 & 0.06 & 0.02 & 1664.96 & 0.92 & 0.98 & 0 &  \\ 
  $\beta^{(1)}_{0,11}$ & 0 & -0.03 & -0.03 & 29654.05 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,21}$ & 0 & 0.03 & -0.01 & 16151.91 & 0.99 & 0.98 & 0 &  \\ 
  $\beta^{(1)}_{0,12}$ & 0 & 0.05 & 0.02 & 12004.06 & 0.98 & 0.86 & 0 &  \\ 
  $\beta^{(1)}_{0,22}$ & 0 & -0.01 & 0.02 & 20032.38 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,11}$ & 0 & 0.02 & 0.01 & 17267.26 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,21}$ & 0 & -0.02 & -0.03 & 17236.35 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,12}$ & 0 & 0.02 & -0.01 & 12905.91 & 0.99 & 0.98 & 0 &  \\ 
  $\beta^{(1)}_{1,22}$ & 0 & 0.02 & 0.01 & 19171.26 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,11}$ & 0 & 0.01 & 0 & 36686.23 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,21}$ & 0 & 0 & -0.04 & 16445.32 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,12}$ & 0 & 0.04 & 0.01 & 13789.56 & 0.99 & 0.82 & 0 &  \\ 
  $\beta^{(1)}_{2,22}$ & 0 & 0.02 & 0.03 & 18514.35 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,11}$ & 0 & -0.02 & -0.03 & 30096.66 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,21}$ & 0 & 0.05 & 0.04 & 17962.41 & 0.99 & 0.95 & 0 &  \\ 
  $\beta^{(1)}_{3,12}$ & 0 & 0.06 & 0.02 & 20101.21 & 0.96 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,22}$ & 0 & -0.03 & 0.01 & 23748.7 & 0.99 & 1 & 0 &  \\ 
  $\sigma^{(1)2}_{11}$ & 0 & 0.12 & 0.01 & 1608.12 & 0.3 &  &  &  \\ 
  $\sigma^{(1)2}_{21}$ & 0.98 & 0.01 & -0.01 & 2000 & 0.46 &  &  &  \\ 
  $\sigma^{(1)2}_{12}$ & 0.49 & 0 & 0.04 & 2000 & 0.03 &  &  &  \\ 
  $\sigma^{(1)2}_{22}$ & 0.21 & 0.05 & 0.03 & 1821.32 & 0.3 &  &  &  \\ 
  $\alpha^{(2)}_{1}$ & 0.59 & 0.01 & 0 & 2000 & 0.7 & 0.66 & 0 &  \\ 
  $\alpha^{(2)}_{2}$ & 0.51 & -0.01 & 0.03 & 2000 & 0.25 & 0.22 & 0 &  \\ 
  $\alpha^{(2)}_{3}$ & 0.48 & -0.02 & -0.01 & 1779.16 & 0.05 & 0.09 & 0.01 &  \\ 
  $\alpha^{(2)}_{4}$ & 0.92 & 0.02 & 0 & 2000 & 0.87 & 0.8 & 0.01 &  \\ 
  $\nu^{(2)}_{11}$ & 0 & 0.13 & 0.1 & 487.94 & 0.03 & 0.22 & 0 &  \\ 
  $\nu^{(2)}_{21}$ & 0 & 0.2 & 0.23 & 71.36 & 0.83 & 0.25 & 0 &  \\ 
  $\nu^{(2)}_{31}$ & 0 & 0.11 & 0.07 & 541.25 & 0.39 & 0.66 & 0 &  \\ 
  $\nu^{(2)}_{41}$ & 0.47 & -0.03 & 0.01 & 2286.04 & 0.71 & 0.44 & 0 &  \\ 
  $\nu^{(2)}_{12}$ & 0 & 0.17 & 0.17 & 122.19 & 0.89 & 0.67 & 0 &  \\ 
  $\nu^{(2)}_{22}$ & 0.03 & 0.06 & 0.01 & 1788.34 & 0.31 & 0.4 & 0 &  \\ 
  $\nu^{(2)}_{32}$ & 0 & 0.55 & 0.54 & 34.84 & 0.31 & 0.05 & 0.02 &  \\ 
  $\nu^{(2)}_{42}$ & 0.97 & -0.01 & -0.02 & 2000 & 0.68 & 0.24 & 0 &  \\ 
  $\nu^{(2)}_{13}$ & 0.06 & 0.02 & 0 & 2000 & 0.82 & 0.11 & 0 &  \\ 
  $\nu^{(2)}_{23}$ & 0.68 & 0.03 & 0.01 & 1875.75 & 0.78 & 0.14 & 0 &  \\ 
  $\nu^{(2)}_{33}$ & 0.82 & -0.03 & -0.02 & 2000 & 0.48 & 0.46 & 0 &  \\ 
  $\nu^{(2)}_{43}$ & 0.78 & 0 & -0.01 & 2000 & 0.73 & 0.76 & 0 &  \\ 
  $\nu^{(2)}_{14}$ & 0.69 & -0.03 & -0.01 & 2000 & 0.56 & 0.46 & 0 &  \\ 
  $\nu^{(2)}_{24}$ & 0.18 & -0.01 & -0.02 & 2293.38 & 0.91 & 0.99 & 0 &  \\ 
  $\nu^{(2)}_{34}$ & 0.05 & 0.04 & 0.03 & 1849.94 & 0.79 & 0.27 & 0 &  \\ 
  $\nu^{(2)}_{44}$ & 0.65 & 0.01 & -0.01 & 2000 & 0.14 & 0.05 &  &  \\ 
  $\rho^{(1)}$ & 1 & 0 & -0.01 & 2000 & 0.01 & 0.2 & 0.03 &  \\ 
  $\rho^{(2)}$ & 0 & 0.22 & 0.06 & 877.28 & 0.14 & 0.77 & 0.04 &  \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_conn_res2.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:43:52 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters} 
\label{tab: MCMCcon}
\begin{tabular}{ccccccccc}
  \hline
Parameters & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0 & 0.02 & 0.01 & 15632.19 & 0.65 & 0.54 & 0 & 3834 \\ 
  $\alpha^{(1)}_{2}$ & 0.22 & 0.02 & 0.01 & 19239.7 & 0.28 & 0.24 & 0 & 3740 \\ 
  $\alpha^{(1)}_{3}$ & 0.76 & 0 & -0.01 & 20000 & 0.05 & 0.14 & 0 & 3881 \\ 
  $\alpha^{(1)}_{4}$ & 0.67 & 0 & 0.01 & 20000 & 0.01 & 0.07 & 0 & 3740 \\ 
  $\nu^{(1)}_{11}$ & 0 & 0.58 & 0.48 & 402.41 & 0.74 & 0.86 & 0 & 27135 \\ 
  $\nu^{(1)}_{21}$ & 0 & 0.39 & 0.32 & 946.25 & 0.52 & 0.82 & 0 & 14469 \\ 
  $\nu^{(1)}_{31}$ & 0 & 0.03 & 0.02 & 13943.07 & 0.66 & 0.56 & 0 & 3802 \\ 
  $\nu^{(1)}_{41}$ & 0 & 0.34 & 0.23 & 1756 & 0.54 & 0.69 & 0 & 14151 \\ 
  $\nu^{(1)}_{12}$ & 0 & 0.41 & 0.29 & 1477.15 & 0.92 & 0.69 & 0 & 20025 \\ 
  $\nu^{(1)}_{22}$ & 0 & 0.15 & 0.11 & 4632.5 & 0.14 & 0.11 & 0 & 8616 \\ 
  $\nu^{(1)}_{32}$ & 0 & 0.15 & 0.1 & 5689.37 & 0.42 & 0.26 & 0 & 8478 \\ 
  $\nu^{(1)}_{42}$ & 0 & 0.22 & 0.13 & 3433.81 & 0.63 & 0.48 & 0 & 4028 \\ 
  $\nu^{(1)}_{13}$ & 0 & 0.1 & 0.04 & 8759.48 & 0.02 & 0.16 & 0 & 3945 \\ 
  $\nu^{(1)}_{23}$ & 0 & 0.02 & -0.01 & 16477.96 & 0.6 & 0.08 & 0 & 3787 \\ 
  $\nu^{(1)}_{33}$ & 0.02 & 0.01 & -0.01 & 19742.08 & 0.04 & 0.3 & 0 & 3771 \\ 
  $\nu^{(1)}_{43}$ & 0 & 0.1 & 0.04 & 8085.67 & 0.75 & 0.38 & 0 & 3945 \\ 
  $\nu^{(1)}_{14}$ & 0 & 0.28 & 0.21 & 1670.53 & 0.8 & 0.98 & 0 & 11403 \\ 
  $\nu^{(1)}_{24}$ & 0 & 0.35 & 0.27 & 878.43 & 0.49 & 0.9 & 0 & 13413 \\ 
  $\nu^{(1)}_{34}$ & 0 & 0.03 & 0.03 & 11273.57 & 0.29 & 0.38 & 0 & 3818 \\ 
  $\nu^{(1)}_{44}$ & 0 & 0.19 & 0.11 & 3725.54 & 0.68 & 0.56 & 0 & 8138 \\ 
  $\beta^{(1)}_{0,11}$ & 0 & 0.08 & 0.07 & 4226.7 & 0.38 & 0.4 & 0.01 & 3929 \\ 
  $\beta^{(1)}_{0,21}$ & 0 & 0.1 & 0.05 & 6477.3 & 0.05 & 0.07 & 0 & 3961 \\ 
  $\beta^{(1)}_{0,31}$ & 0 & 0.16 & 0.08 & 5775.42 & 0.67 & 0.57 & 0 & 4028 \\ 
  $\beta^{(1)}_{0,41}$ & 0 & 0.05 & 0.03 & 12236.99 & 0.23 & 0.18 & 0 & 3849 \\ 
  $\beta^{(1)}_{0,12}$ & 0 & 0.1 & 0.06 & 7717.67 & 0.95 & 0.78 & 0 & 3865 \\ 
  $\beta^{(1)}_{0,22}$ & 0 & 0.09 & 0.06 & 5635.18 & 0.19 & 0.86 & 0 & 3929 \\ 
  $\beta^{(1)}_{0,32}$ & 0 & 0.08 & 0.05 & 5598.38 & 0.74 & 0.61 & 0 & 3913 \\ 
  $\beta^{(1)}_{0,42}$ & 0 & 0.07 & 0.04 & 8888.43 & 0.69 & 0.34 & 0 & 3913 \\ 
  $\beta^{(1)}_{0,13}$ & 0 & 0.09 & 0.05 & 8962.9 & 0.06 & 0.58 & 0 & 3929 \\ 
  $\beta^{(1)}_{0,23}$ & 0 & 0.04 & 0.02 & 14707.97 & 0.5 & 0.66 & 0 & 3929 \\ 
  $\beta^{(1)}_{0,33}$ & 0.68 & 0 & 0 & 20000 & 0.99 & 0.9 & 0 & 3771 \\ 
  $\beta^{(1)}_{0,43}$ & 0 & 0.04 & 0.02 & 15693.22 & 0.28 & 0.84 & 0 & 3849 \\ 
  $\beta^{(1)}_{0,14}$ & 0 & 0.04 & 0.01 & 13386.92 & 0.95 & 0.86 & 0 & 3818 \\ 
  $\beta^{(1)}_{0,24}$ & 0 & 0.07 & 0.03 & 11644.71 & 0.16 & 0.3 & 0 & 3834 \\ 
  $\beta^{(1)}_{0,34}$ & 0 & 0.03 & 0.01 & 13122.76 & 0.99 & 0.11 & 0 & 3849 \\ 
  $\beta^{(1)}_{0,44}$ & 0 & 0.04 & 0.02 & 13004.08 & 0.68 & 0.61 & 0 & 3881 \\ 
  $\beta^{(1)}_{1,11}$ & 0 & 0.05 & 0.04 & 7653.74 & 0.32 & 0.25 & 0 & 3834 \\ 
  $\beta^{(1)}_{1,21}$ & 0 & 0.05 & 0.02 & 12887.72 & 0.99 & 0.25 & 0 & 3882 \\ 
  $\beta^{(1)}_{1,31}$ & 0 & 0.2 & 0.12 & 4545.64 & 0.77 & 0.79 & 0 & 7742 \\ 
  $\beta^{(1)}_{1,41}$ & 0 & 0.01 & 0.01 & 16963.42 & 0.39 & 0.06 & 0 & 3818 \\ 
  $\beta^{(1)}_{1,12}$ & 0 & 0.04 & 0.02 & 13154.38 & 0.41 & 0.16 & 0 & 3771 \\ 
  $\beta^{(1)}_{1,22}$ & 0 & 0.08 & 0.04 & 8561.46 & 0.47 & 0.72 & 0 & 3787 \\ 
  $\beta^{(1)}_{1,32}$ & 0 & 0.13 & 0.1 & 3282.64 & 0.66 & 0.99 & 0 & 3978 \\ 
  $\beta^{(1)}_{1,42}$ & 0 & 0.02 & 0.01 & 14084.94 & 0.58 & 0.24 & 0 & 3755 \\ 
  $\beta^{(1)}_{1,13}$ & 0 & 0.02 & 0 & 18581.86 & 0.65 & 0.23 & 0 & 3945 \\ 
  $\beta^{(1)}_{1,23}$ & 0.43 & 0.01 & 0.01 & 20000 & 0.42 & 0.78 & 0 & 3802 \\ 
  $\beta^{(1)}_{1,33}$ & 0.43 & -0.02 & -0.01 & 20763.19 & 0.72 & 0.87 & 0 & 3771 \\ 
  $\beta^{(1)}_{1,43}$ & 0 & 0.03 & 0 & 17630.37 & 0.76 & 0.42 & 0 & 3787 \\ 
  $\beta^{(1)}_{1,14}$ & 0 & 0.05 & 0.01 & 13455.76 & 0.78 & 0.75 & 0 & 3929 \\ 
  $\beta^{(1)}_{1,24}$ & 0 & 0.05 & 0.03 & 9022.33 & 0.78 & 0.69 & 0 & 3913 \\ 
  $\beta^{(1)}_{1,34}$ & 0 & 0.09 & 0.04 & 9430.08 & 0.32 & 0.41 & 0 & 4045 \\ 
  $\beta^{(1)}_{1,44}$ & 0 & 0.05 & 0.03 & 12937.18 & 0.83 & 0.82 & 0 & 3865 \\ 
  $\beta^{(1)}_{2,11}$ & 0 & 0.13 & 0.09 & 3532.03 & 0.94 & 0.85 & 0 & 3961 \\ 
  $\beta^{(1)}_{2,21}$ & 0 & 0.21 & 0.16 & 2042.04 & 0.12 & 0.52 & 0 & 3994 \\ 
  $\beta^{(1)}_{2,31}$ & 0 & 0.03 & 0.01 & 14513.51 & 0.76 & 0.66 & 0 & 3849 \\ 
  $\beta^{(1)}_{2,41}$ & 0 & 0.09 & 0.05 & 8690.38 & 0.16 & 0.08 & 0 & 3929 \\ 
  $\beta^{(1)}_{2,12}$ & 0 & 0.11 & 0.06 & 6283.13 & 0.86 & 0.82 & 0 & 3865 \\ 
  $\beta^{(1)}_{2,22}$ & 0 & 0.25 & 0.18 & 1543.5 & 0.19 & 0.89 & 0 & 11847 \\ 
  $\beta^{(1)}_{2,32}$ & 0 & 0.01 & 0.01 & 14868.35 & 0.61 & 0.15 & 0 & 3945 \\ 
  $\beta^{(1)}_{2,42}$ & 0 & 0.09 & 0.05 & 8857.95 & 0.69 & 0.32 & 0 & 3994 \\ 
  $\beta^{(1)}_{2,13}$ & 0 & 0.18 & 0.11 & 5110.54 & 0.04 & 0.17 & 0 & 4180 \\ 
  $\beta^{(1)}_{2,23}$ & 0 & 0.09 & 0.06 & 8952.17 & 0.92 & 0.51 & 0 & 3818 \\ 
  $\beta^{(1)}_{2,33}$ & 0.12 & 0.01 & 0 & 19164.68 & 0.9 & 0.8 & 0 & 3725 \\ 
  $\beta^{(1)}_{2,43}$ & 0 & 0.08 & 0.04 & 10375.62 & 0.22 & 0.63 & 0 & 3818 \\ 
  $\beta^{(1)}_{2,14}$ & 0 & 0.06 & 0.03 & 11848.42 & 0.58 & 0.73 & 0 & 3881 \\ 
  $\beta^{(1)}_{2,24}$ & 0 & 0.1 & 0.06 & 6869.02 & 0.16 & 0.51 & 0 & 3913 \\ 
  $\beta^{(1)}_{2,34}$ & 0.71 & 0 & 0 & 20000 & 0.31 & 0.12 & 0 & 3802 \\ 
  $\beta^{(1)}_{2,44}$ & 0 & 0.04 & 0.04 & 10074.42 & 0.9 & 0.52 & 0 & 3834 \\ 
  $\beta^{(1)}_{3,11}$ & 0 & 0.11 & 0.06 & 6311.06 & 0.35 & 0.05 & 0 & 3897 \\ 
  $\beta^{(1)}_{3,21}$ & 0 & 0.15 & 0.1 & 1782.87 & 0.85 & 0.9 & 0 & 4078 \\ 
  $\beta^{(1)}_{3,31}$ & 0 & 0.06 & 0.02 & 11370.37 & 0.64 & 0.17 & 0 & 3802 \\ 
  $\beta^{(1)}_{3,41}$ & 0 & 0.03 & 0.01 & 16099.85 & 0.08 & 0.05 & 0 & 3913 \\ 
  $\beta^{(1)}_{3,12}$ & 0 & 0.08 & 0.05 & 9807.06 & 0.48 & 0.64 & 0 & 3865 \\ 
  $\beta^{(1)}_{3,22}$ & 0 & 0.08 & 0.04 & 7506.35 & 0.67 & 0.92 & 0 & 3849 \\ 
  $\beta^{(1)}_{3,32}$ & 0 & 0.06 & 0.04 & 7577.36 & 0.02 & 0.15 & 0 & 3929 \\ 
  $\beta^{(1)}_{3,42}$ & 0 & 0.03 & 0.01 & 15106.81 & 0.57 & 0.79 & 0 & 3740 \\ 
  $\beta^{(1)}_{3,13}$ & 0 & 0.03 & 0 & 17780.57 & 0.35 & 0.85 & 0 & 3802 \\ 
  $\beta^{(1)}_{3,23}$ & 0 & 0.04 & 0.02 & 12472.73 & 0.47 & 0.69 & 0 & 3881 \\ 
  $\beta^{(1)}_{3,33}$ & 0.15 & 0 & 0.01 & 20000 & 0.47 & 0.85 & 0 & 3834 \\ 
  $\beta^{(1)}_{3,43}$ & 0 & 0.03 & 0.01 & 16636.91 & 0.35 & 0.76 & 0 & 3802 \\ 
  $\beta^{(1)}_{3,14}$ & 0 & 0.03 & 0.02 & 15588.07 & 0.37 & 0.19 & 0 & 3802 \\ 
  $\beta^{(1)}_{3,24}$ & 0 & 0.05 & 0.01 & 14046.35 & 0.64 & 0.62 & 0 & 3771 \\ 
  $\beta^{(1)}_{3,34}$ & 0 & 0.03 & 0.01 & 15832 & 0.93 & 0.49 & 0 & 3865 \\ 
  $\beta^{(1)}_{3,44}$ & 0 & 0.02 & 0.01 & 16175.61 & 0.07 & 0.35 & 0 & 3881 \\ 
  $\sigma^{(1)2}_{11}$ & 0 & 0.06 & 0.02 & 11424.4 & 0.58 &  &  & 3849 \\ 
  $\sigma^{(1)2}_{21}$ & 0 & 0.41 & 0.35 & 737.15 & 0.75 &  &  & 14415 \\ 
  $\sigma^{(1)2}_{31}$ & 0 & 0.16 & 0.08 & 5032.01 & 0.38 &  &  & 14814 \\ 
  $\sigma^{(1)2}_{41}$ & 0 & 0.04 & 0.02 & 14915.43 & 0.28 &  &  & 3818 \\ 
  $\sigma^{(1)2}_{12}$ & 0 & 0.08 & 0.06 & 4181.07 & 0.57 &  &  & 3787 \\ 
  $\sigma^{(1)2}_{22}$ & 0 & 0.56 & 0.45 & 767.73 & 0.87 &  &  & 24710 \\ 
  $\sigma^{(1)2}_{32}$ & 0 & 0.07 & 0.04 & 9062.1 & 0.45 &  &  & 3929 \\ 
  $\sigma^{(1)2}_{42}$ & 0 & 0.04 & 0 & 17627.56 & 0.6 &  &  & 3818 \\ 
  $\sigma^{(1)2}_{13}$ & 0 & 0.12 & 0.07 & 6389.17 & 0.63 &  &  & 4061 \\ 
  $\sigma^{(1)2}_{23}$ & 0 & 0.17 & 0.14 & 1968.15 & 0.65 &  &  & 3929 \\ 
  $\sigma^{(1)2}_{33}$ & 0.02 & 0.02 & 0.01 & 18227.32 & 0.92 &  &  & 3865 \\ 
  $\sigma^{(1)2}_{43}$ & 0 & 0.03 & 0 & 16610.03 & 0.14 &  &  & 3787 \\ 
  $\sigma^{(1)2}_{14}$ & 0 & 0.02 & 0.01 & 17961.38 & 0.44 &  &  & 3834 \\ 
  $\sigma^{(1)2}_{24}$ & 0 & 0.09 & 0.06 & 4118.14 & 0.56 &  &  & 3913 \\ 
  $\sigma^{(1)2}_{34}$ & 0 & 0.04 & 0.01 & 16563.26 & 0.13 &  &  & 3818 \\ 
  $\sigma^{(1)2}_{44}$ & 0.06 & 0.02 & 0.01 & 18338.5 & 0.54 &  &  & 3834 \\ 
  $\alpha^{(2)}_{1}$ & 0.72 & 0 & -0.01 & 20000 & 0.38 & 0.99 & 0 & 3771 \\ 
  $\alpha^{(2)}_{2}$ & 0.34 & 0 & -0.02 & 20000 & 0.51 & 0.61 & 0 & 3755 \\ 
  $\alpha^{(2)}_{3}$ & 0.16 & 0 & 0 & 20157.99 & 0.4 & 0.68 & 0 & 3725 \\ 
  $\alpha^{(2)}_{4}$ & 0.03 & 0.01 & 0.01 & 16872.73 & 0.03 & 0.22 & 0 & 3849 \\ 
  $\nu^{(2)}_{11}$ & 0.04 & 0.02 & -0.01 & 19325.04 & 0.95 & 0.23 & 0 & 3802 \\ 
  $\nu^{(2)}_{21}$ & 0 & 0.03 & 0.02 & 13500.32 & 0.71 & 0.25 & 0 & 3849 \\ 
  $\nu^{(2)}_{31}$ & 0.46 & 0.01 & 0 & 19086.05 & 0.34 & 0.32 & 0 & 3818 \\ 
  $\nu^{(2)}_{41}$ & 0 & 0.04 & 0.02 & 14071.37 & 0.51 & 0.21 & 0 & 3787 \\ 
  $\nu^{(2)}_{12}$ & 0 & 0.03 & 0.01 & 14574.94 & 0.65 & 0.13 & 0 & 3818 \\ 
  $\nu^{(2)}_{22}$ & 0 & 0.07 & 0.05 & 9789.19 & 0.27 & 0.08 & 0 & 3849 \\ 
  $\nu^{(2)}_{32}$ & 0 & 0.54 & 0.46 & 359.02 & 0.05 & 0.89 & 0 & 353496 \\ 
  $\nu^{(2)}_{42}$ & 0 & 0.1 & 0.08 & 3950.61 & 0.52 & 0.4 & 0 & 8310 \\ 
  $\nu^{(2)}_{13}$ & 0.61 & 0.01 & -0.01 & 19598.3 & 0.48 & 0.62 & 0 & 3755 \\ 
  $\nu^{(2)}_{23}$ & 0 & 0.04 & 0.02 & 9677.33 & 0.65 & 0.42 & 0 & 3849 \\ 
  $\nu^{(2)}_{33}$ & 0.55 & 0.01 & 0 & 20000 & 0.06 & 0.23 & 0 & 3695 \\ 
  $\nu^{(2)}_{43}$ & 0 & 0.31 & 0.23 & 1391.44 & 0.31 & 0.29 & 0 & 22705 \\ 
  $\nu^{(2)}_{14}$ & 0 & 0.03 & 0.02 & 14470.37 & 0.08 & 0.1 & 0 & 3865 \\ 
  $\nu^{(2)}_{24}$ & 0 & 0.12 & 0.1 & 3452.33 & 0.54 & 0.13 & 0 & 13533 \\ 
  $\nu^{(2)}_{34}$ & 0 & 0.05 & 0.04 & 4050 & 0.01 & 0.5 & 0 & 4045 \\ 
  $\nu^{(2)}_{44}$ & 0 & 0.24 & 0.18 & 1182.05 & 0.31 & 0.51 & 0 & 64458 \\ 
  $\rho^{(1)}$ & 0 & 0.8 & 0.55 & 595.44 & 0.28 & 0.32 & 0.04 & 69984 \\ 
  $\rho^{(2)}$ & 0 & 0.84 & 0.63 & 467.35 & 0.52 & 0.06 & 0.06 & 39933 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_conn_res2_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:43:52 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters} 
\label{tab: MCMCcon}
\begin{tabular}{ccccccccc}
  \hline
Parameters & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0.46 & -0.01 & 0.03 & 2000 & 0.33 & 0.23 & 0.01 &  \\ 
  $\alpha^{(1)}_{2}$ & 0.91 & -0.01 & 0 & 2000 & 0.19 & 0.32 & 0.01 &  \\ 
  $\alpha^{(1)}_{3}$ & 0.17 & -0.02 & -0.03 & 2292.16 & 0.15 & 0.14 & 0.01 &  \\ 
  $\alpha^{(1)}_{4}$ & 0.43 & -0.03 & 0 & 1953.56 & 0.37 & 0.44 & 0 &  \\ 
  $\nu^{(1)}_{11}$ & 0 & 0.42 & 0.19 & 392.32 & 0.87 & 0.84 & 0 &  \\ 
  $\nu^{(1)}_{21}$ & 0 & 0.26 & 0.1 & 675.82 & 0.33 & 0.84 & 0 &  \\ 
  $\nu^{(1)}_{31}$ & 0.92 & -0.03 & -0.02 & 2000 & 0.11 & 0.11 & 0 &  \\ 
  $\nu^{(1)}_{41}$ & 0 & 0.19 & 0.05 & 1004.49 & 0.68 & 0.43 & 0 &  \\ 
  $\nu^{(1)}_{12}$ & 0 & 0.23 & 0.02 & 1091.09 & 0.99 & 0.6 & 0 &  \\ 
  $\nu^{(1)}_{22}$ & 0.01 & 0.09 & 0.03 & 1660.13 & 0.19 & 0.53 & 0 &  \\ 
  $\nu^{(1)}_{32}$ & 0.2 & 0.06 & 0.03 & 1651.2 & 0.26 & 0.15 & 0 &  \\ 
  $\nu^{(1)}_{42}$ & 0 & 0.06 & 0.01 & 1468.27 & 0.44 & 0.53 & 0 &  \\ 
  $\nu^{(1)}_{13}$ & 0.98 & 0.03 & -0.01 & 2000 & 0.13 & 0.42 & 0 &  \\ 
  $\nu^{(1)}_{23}$ & 0.14 & 0.08 & 0 & 1709.31 & 0.7 & 0.59 & 0 &  \\ 
  $\nu^{(1)}_{33}$ & 0.81 & 0 & 0.01 & 2000 & 0.03 & 0.25 & 0 &  \\ 
  $\nu^{(1)}_{43}$ & 0.47 & 0.04 & -0.01 & 1661.12 & 0.62 & 0.32 & 0 &  \\ 
  $\nu^{(1)}_{14}$ & 0 & 0.14 & 0.04 & 1038.62 & 0.42 & 0.46 & 0 &  \\ 
  $\nu^{(1)}_{24}$ & 0 & 0.24 & 0.05 & 673.37 & 0.28 & 0.92 & 0 &  \\ 
  $\nu^{(1)}_{34}$ & 0.05 & 0.02 & 0.04 & 2056.89 & 0.3 & 0.32 & 0 &  \\ 
  $\nu^{(1)}_{44}$ & 0.01 & 0.07 & 0.01 & 1596.43 & 0.8 & 0.92 & 0 &  \\ 
  $\beta^{(1)}_{0,11}$ & 0 & 0.08 & 0.04 & 10460.07 & 0.99 & 0.88 & 0.01 &  \\ 
  $\beta^{(1)}_{0,21}$ & 0 & 0.05 & 0.03 & 16784.41 & 0.99 & 0.81 & 0 &  \\ 
  $\beta^{(1)}_{0,31}$ & 0 & 0.05 & -0.01 & 21429.45 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,41}$ & 0 & 0.03 & -0.02 & 12037.99 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,12}$ & 0 & 0.03 & 0.02 & 13227.06 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,22}$ & 0 & 0.04 & 0 & 15842.49 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,32}$ & 0 & 0.05 & 0.02 & 13192.78 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,42}$ & 0 & 0.02 & 0.02 & 12048.83 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,13}$ & 0 & 0.07 & -0.04 & 20009.83 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,23}$ & 0 & 0.03 & 0.02 & 20642.92 & 0.99 & 0.96 & 0 &  \\ 
  $\beta^{(1)}_{0,33}$ & 0 & -0.01 & -0.03 & 51937.75 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,43}$ & 0 & 0.01 & 0.02 & 26885.32 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,14}$ & 0 & 0.01 & 0.02 & 18860.65 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,24}$ & 0 & 0.02 & 0.05 & 22786.9 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,34}$ & 0 & 0.03 & 0.02 & 16230.03 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{0,44}$ & 0 & 0 & -0.03 & 18467.74 & 0.98 & 0.99 & 0 &  \\ 
  $\beta^{(1)}_{1,11}$ & 0 & -0.01 & 0.02 & 20218.86 & 0.99 & 0.94 & 0 &  \\ 
  $\beta^{(1)}_{1,21}$ & 0 & 0 & 0.03 & 29231.73 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,31}$ & 0 & 0.04 & -0.02 & 18895.61 & 0.97 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,41}$ & 0 & 0.03 & -0.02 & 15418.98 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,12}$ & 0 & 0.04 & 0.02 & 33570.33 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,22}$ & 0 & 0.03 & 0.01 & 20078.82 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,32}$ & 0 & 0.07 & 0.03 & 14380.99 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,42}$ & 0 & -0.01 & 0.03 & 12156.62 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,13}$ & 0 & 0.02 & -0.01 & 17683.37 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,23}$ & 0 & 0.01 & -0.02 & 16153.38 & 0.98 & 0.97 & 0 &  \\ 
  $\beta^{(1)}_{1,33}$ & 0 & -0.01 & -0.01 & 32130.1 & 1 & 0.98 & 0 &  \\ 
  $\beta^{(1)}_{1,43}$ & 0 & 0.01 & 0 & 27380.46 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,14}$ & 0 & -0.02 & 0.03 & 21900.31 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,24}$ & 0 & 0.07 & 0.04 & 10054.51 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,34}$ & 0 & 0 & -0.01 & 19748.8 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{1,44}$ & 0 & -0.01 & 0.01 & 17123.79 & 0.97 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,11}$ & 0 & 0.1 & 0.03 & 10097.65 & 0.99 & 0.99 & 0 &  \\ 
  $\beta^{(1)}_{2,21}$ & 0 & 0.13 & 0.05 & 9778.89 & 0.99 & 0.99 & 0 &  \\ 
  $\beta^{(1)}_{2,31}$ & 0 & 0.05 & 0.01 & 11239.38 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,41}$ & 0 & 0.04 & -0.01 & 11869.85 & 0.97 & 0.84 & 0 &  \\ 
  $\beta^{(1)}_{2,12}$ & 0 & 0.03 & 0.02 & 10171.38 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,22}$ & 0 & 0.1 & 0.04 & 9372.23 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,32}$ & 0 & -0.01 & -0.02 & 16627.97 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,42}$ & 0 & 0.05 & 0.02 & 20394.01 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,13}$ & 0 & 0.1 & -0.02 & 12739.02 & 0.97 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,23}$ & 0 & 0.01 & 0.02 & 23492.69 & 0.99 & 0.99 & 0 &  \\ 
  $\beta^{(1)}_{2,33}$ & 0 & -0.01 & 0 & 23996.89 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,43}$ & 0 & 0 & 0 & 18735.15 & 0.98 & 0.99 & 0 &  \\ 
  $\beta^{(1)}_{2,14}$ & 0 & 0.03 & 0.04 & 16375.9 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,24}$ & 0 & 0.05 & 0 & 21354.86 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,34}$ & 0 & 0.02 & 0 & 22910.59 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{2,44}$ & 0 & 0.06 & -0.05 & 14667.79 & 0.99 & 0.98 & 0 &  \\ 
  $\beta^{(1)}_{3,11}$ & 0 & 0.02 & 0.02 & 17004.02 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,21}$ & 0 & 0.08 & 0.01 & 7092.58 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,31}$ & 0 & 0.07 & 0.01 & 17751.3 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,41}$ & 0 & -0.04 & -0.01 & 31199.49 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,12}$ & 0 & 0.03 & 0.01 & 15463.94 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,22}$ & 0 & 0 & -0.01 & 19549.06 & 0.98 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,32}$ & 0 & 0.04 & 0.04 & 16514.68 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,42}$ & 0 & 0 & 0 & 16543.39 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,13}$ & 0 & -0.01 & 0.02 & 17756.48 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,23}$ & 0 & 0.04 & -0.01 & 24474.94 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,33}$ & 0 & -0.01 & 0 & 17448.36 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,43}$ & 0 & 0.04 & 0.01 & 21614.39 & 0.98 & 0.99 & 0 &  \\ 
  $\beta^{(1)}_{3,14}$ & 0 & 0 & -0.01 & 16531.3 & 0.99 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,24}$ & 0 & 0.02 & 0.03 & 18504.2 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,34}$ & 0 & 0.02 & 0.01 & 18184.57 & 1 & 1 & 0 &  \\ 
  $\beta^{(1)}_{3,44}$ & 0 & 0.02 & -0.02 & 25525.75 & 0.99 & 1 & 0 &  \\ 
  $\sigma^{(1)2}_{11}$ & 0.98 & 0.02 & 0 & 2000 & 0.01 &  &  &  \\ 
  $\sigma^{(1)2}_{21}$ & 0 & 0.29 & 0.13 & 424.4 & 0.79 &  &  &  \\ 
  $\sigma^{(1)2}_{31}$ & 0.34 & 0.05 & -0.01 & 1820.52 & 0.67 &  &  &  \\ 
  $\sigma^{(1)2}_{41}$ & 0.31 & 0.05 & 0.03 & 1815.05 & 0.74 &  &  &  \\ 
  $\sigma^{(1)2}_{12}$ & 0.94 & 0.01 & -0.02 & 2000 & 0.9 &  &  &  \\ 
  $\sigma^{(1)2}_{22}$ & 0 & 0.37 & 0.11 & 416.39 & 0.94 &  &  &  \\ 
  $\sigma^{(1)2}_{32}$ & 0.53 & 0.02 & 0 & 1742.57 & 0.57 &  &  &  \\ 
  $\sigma^{(1)2}_{42}$ & 0.45 & 0.01 & 0 & 2000 & 0.22 &  &  &  \\ 
  $\sigma^{(1)2}_{13}$ & 0.1 & 0.05 & -0.01 & 1796.42 & 0.83 &  &  &  \\ 
  $\sigma^{(1)2}_{23}$ & 0 & 0.1 & 0.06 & 1048.36 & 0.64 &  &  &  \\ 
  $\sigma^{(1)2}_{33}$ & 0.66 & 0 & -0.02 & 2000 & 0.14 &  &  &  \\ 
  $\sigma^{(1)2}_{43}$ & 0.67 & -0.01 & 0.05 & 2000 & 0.99 &  &  &  \\ 
  $\sigma^{(1)2}_{14}$ & 0.97 & 0.01 & 0.02 & 2000 & 0.29 &  &  &  \\ 
  $\sigma^{(1)2}_{24}$ & 0.14 & 0.04 & 0.02 & 1599.35 & 0.8 &  &  &  \\ 
  $\sigma^{(1)2}_{34}$ & 0.28 & 0.03 & -0.01 & 2000 & 0.57 &  &  &  \\ 
  $\sigma^{(1)2}_{44}$ & 0.75 & -0.01 & -0.03 & 2000 & 0.2 &  &  &  \\ 
  $\alpha^{(2)}_{1}$ & 0.68 & 0 & 0.01 & 2000 & 0.3 & 0.53 & 0.01 &  \\ 
  $\alpha^{(2)}_{2}$ & 0.94 & -0.01 & 0 & 2000 & 0.03 & 0.16 & 0 &  \\ 
  $\alpha^{(2)}_{3}$ & 0.45 & 0 & -0.01 & 2000 & 0.69 & 0.98 & 0.01 &  \\ 
  $\alpha^{(2)}_{4}$ & 0.99 & 0 & -0.01 & 2000 & 0.35 & 0.15 & 0.01 &  \\ 
  $\nu^{(2)}_{11}$ & 0.82 & 0.02 & -0.03 & 2000 & 0.57 & 0.24 & 0 &  \\ 
  $\nu^{(2)}_{21}$ & 0.04 & 0.04 & 0.04 & 1621.23 & 0.65 & 0.43 & 0 &  \\ 
  $\nu^{(2)}_{31}$ & 0.62 & 0.01 & 0.01 & 2000 & 0.82 & 0.51 & 0 &  \\ 
  $\nu^{(2)}_{41}$ & 0.57 & 0.04 & -0.01 & 1966.65 & 0.85 & 0.27 & 0 &  \\ 
  $\nu^{(2)}_{12}$ & 0.98 & 0 & 0.02 & 2000 & 0.56 & 0.16 & 0 &  \\ 
  $\nu^{(2)}_{22}$ & 0.4 & 0.01 & 0 & 2000 & 0 & 0.14 & 0 &  \\ 
  $\nu^{(2)}_{32}$ & 0 & 0.4 & 0.23 & 368.97 & 0.09 & 0.76 & 0 &  \\ 
  $\nu^{(2)}_{42}$ & 0 & 0.04 & 0.07 & 1260.86 & 0.06 & 0.61 & 0 &  \\ 
  $\nu^{(2)}_{13}$ & 0.66 & -0.01 & -0.03 & 2000 & 0.71 & 0.11 & 0 &  \\ 
  $\nu^{(2)}_{23}$ & 0.12 & 0.02 & 0.02 & 2254.19 & 0.76 & 0.46 & 0 &  \\ 
  $\nu^{(2)}_{33}$ & 0.52 & 0.01 & -0.01 & 2000 & 0.04 & 0.39 & 0 &  \\ 
  $\nu^{(2)}_{43}$ & 0 & 0.19 & 0.07 & 872.95 & 0.61 & 0.27 & 0 &  \\ 
  $\nu^{(2)}_{14}$ & 0.97 & 0 & -0.01 & 2000 & 0.07 & 0.39 & 0 &  \\ 
  $\nu^{(2)}_{24}$ & 0 & 0.08 & 0.01 & 1690.08 & 0.95 & 0.35 & 0 &  \\ 
  $\nu^{(2)}_{34}$ & 0 & 0.06 & 0.03 & 1405.62 & 0 & 0.12 & 0 &  \\ 
  $\nu^{(2)}_{44}$ & 0 & 0.13 & 0.08 & 763.36 & 0.94 & 0.87 & 0 &  \\ 
  $\rho^{(1)}$ & 0 & 0.44 & 0.13 & 492.95 & 0.31 & 0.38 & 0.05 &  \\ 
  $\rho^{(2)}$ & 0 & 0.52 & 0.15 & 489.38 & 0.48 & 0.01 &  &  \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_conn_res_0_bf_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:33:04 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters before and after thinning} 
\label{tab: MCMCcon_ba_th}
\begin{tabular}{cccccccccc}
  \hline \multirow{2}{3cm}{\centering Parameters} & \multicolumn{4}{c}{Before thinning} & & \multicolumn{4}{c}{After thinning} \\ \cline{2-5} \cline{7-10}V1 & $AC1$ & $AC5$ & $GD$ & $HDS$ & V6 & $AC1$ & $AC5$ & $GD$ & $HDS$ \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0.01 & 0 & 0.24 & 0.54 &  & 0.03 & 0 & 0.25 & 0.86 \\ 
  $\alpha^{(1)}_{2}$ & 0.01 & 0 & 0.24 & 0.54 &  & 0.03 & 0 & 0.25 & 0.86 \\ 
  $\nu^{(1)}_{11}$ & 0.18 & 0.11 & 0.61 & 0.71 &  & 0.06 & 0 & 0.68 & 0.76 \\ 
  $\nu^{(1)}_{21}$ & 0.27 & 0.14 & 0.23 & 0.53 &  & 0.11 & 0.04 & 0.09 & 0.79 \\ 
  $\nu^{(1)}_{12}$ & 0.3 & 0.17 & 0.9 & 0.77 &  & 0.09 & 0 & 0.48 & 0.14 \\ 
  $\nu^{(1)}_{22}$ & 0.07 & 0.02 & 0.63 & 0.78 &  & 0.03 & 0 & 0.86 & 0.87 \\ 
  $\beta^{(1)}_{0,11}$ & 0.09 & 0.04 & 0.8 & 0.8 &  & 0.02 & -0.04 & 0.99 & 1 \\ 
  $\beta^{(1)}_{0,21}$ & 0.04 & 0.01 & 0.71 & 0.56 &  & -0.03 & 0.04 & 1 & 1 \\ 
  $\beta^{(1)}_{0,12}$ & 0.05 & 0.03 & 0.34 & 0.84 &  & 0.01 & 0.01 & 0.99 & 0.99 \\ 
  $\beta^{(1)}_{0,22}$ & 0.06 & 0.02 & 0.65 & 0.58 &  & -0.01 & -0.02 & 0.97 & 1 \\ 
  $\beta^{(1)}_{1,11}$ & 0.01 & 0 & 0.38 & 0.57 &  & -0.04 & -0.01 & 0.98 & 1 \\ 
  $\beta^{(1)}_{1,21}$ & 0.03 & 0.01 & 0.42 & 0.81 &  & 0 & 0.04 & 0.99 & 0.87 \\ 
  $\beta^{(1)}_{1,12}$ & 0.04 & 0.01 & 0.73 & 0.87 &  & 0.05 & -0.03 & 1 & 1 \\ 
  $\beta^{(1)}_{1,22}$ & 0.05 & 0.04 & 0.63 & 0.75 &  & 0.03 & 0.01 & 0.97 & 1 \\ 
  $\beta^{(1)}_{2,11}$ & 0.13 & 0.06 & 0.36 & 0.97 &  & 0.06 & -0.02 & 1 & 0.99 \\ 
  $\beta^{(1)}_{2,21}$ & 0.02 & 0.01 & 0.19 & 0.62 &  & -0.03 & 0.01 & 1 & 1 \\ 
  $\beta^{(1)}_{2,12}$ & 0.05 & 0.01 & 0.05 & 0.24 &  & 0.02 & 0.02 & 0.98 & 1 \\ 
  $\beta^{(1)}_{2,22}$ & 0.07 & 0.03 & 0.15 & 0.15 &  & -0.03 & -0.04 & 0.98 & 1 \\ 
  $\beta^{(1)}_{3,11}$ & 0.03 & 0.01 & 0.11 & 0.43 &  & 0.03 & -0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,21}$ & 0.04 & 0.02 & 0.19 & 0.71 &  & -0.03 & 0.01 & 1 & 1 \\ 
  $\beta^{(1)}_{3,12}$ & 0.05 & 0.02 & 0.39 & 0.39 &  & 0.01 & 0.03 & 0.99 & 0.9 \\ 
  $\beta^{(1)}_{3,22}$ & 0.08 & 0.05 & 0.01 & 0.1 &  & 0.03 & 0.01 & 0.99 & 1 \\ 
  $\sigma^{(1)2}_{11}$ & 0.01 & 0 & 0.79 &  &  & 0.02 & -0.02 & 0.84 &  \\ 
  $\sigma^{(1)2}_{21}$ & 0.07 & 0.04 & 0.93 &  &  & -0.01 & -0.02 & 0.91 &  \\ 
  $\sigma^{(1)2}_{12}$ & 0.05 & 0.02 & 0.43 &  &  & 0 & -0.02 & 0.06 &  \\ 
  $\sigma^{(1)2}_{22}$ & 0.26 & 0.15 & 0.28 &  &  & 0.08 & -0.03 & 0.24 &  \\ 
  $\alpha^{(2)}_{1}$ & 0 & 0 & 0.68 & 0.64 &  & 0.02 & 0.01 & 0.63 & 0.13 \\ 
  $\alpha^{(2)}_{2}$ & 0 & 0 & 0.68 & 0.64 &  & 0.02 & 0.01 & 0.63 & 0.13 \\ 
  $\nu^{(2)}_{11}$ & -0.01 & 0.01 & 0.56 & 0.26 &  & -0.03 & 0 & 0.44 & 0.79 \\ 
  $\nu^{(2)}_{21}$ & 0 & 0.01 & 0.94 & 0.28 &  & 0.01 & -0.02 & 0.66 & 0.98 \\ 
  $\nu^{(2)}_{12}$ & 0.01 & -0.01 & 0.06 & 0.08 &  & 0.01 & 0.01 & 0.26 & 0.28 \\ 
  $\nu^{(2)}_{22}$ & 0 & 0 & 0.59 & 0.47 &  & -0.02 & -0.01 & 0.2 & 0.71 \\ 
  $\rho^{(1)}$ & 0.42 & 0.09 & 0.51 & 0.62 &  & 0.03 & 0.01 & 0.36 & 0.86 \\ 
  $\rho^{(2)}$ & 0.39 & 0.09 & 0.76 & 0.42 &  & 0.07 & 0.01 & 0.31 & 0.37 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_conn_res_1_bf_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:36:58 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters before and after thinning under $Q^{(1)}=2$ and $Q^{(2)}=4$.} 
\label{tab: MCMCcon_ba_th}
\scriptsize
\begin{tabular}{cccccccccc}
  \hline \multirow{2}{3cm}{\centering Parameters} & \multicolumn{4}{c}{Before thinning} & & \multicolumn{4}{c}{After thinning} \\ \cline{2-5} \cline{7-10} & $AC1$ & $AC5$ & $GD$ & $HDS$ &  & $AC1$ & $AC5$ & $GD$ & $HDS$ \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0.02 & -0.01 & 0.44 & 0.73 &  & 0.02 & 0.02 & 0.71 & 0.9 \\ 
  $\alpha^{(1)}_{2}$ & 0.02 & -0.01 & 0.44 & 0.73 &  & 0.02 & 0.02 & 0.71 & 0.9 \\ 
  $\nu^{(1)}_{11}$ & 0.08 & 0.04 & 0.65 & 0.99 &  & 0.02 & 0 & 0.14 & 0.21 \\ 
  $\nu^{(1)}_{21}$ & 0.28 & 0.16 & 0.03 & 0.22 &  & 0.07 & -0.01 & 0.1 & 0.24 \\ 
  $\nu^{(1)}_{12}$ & 0.34 & 0.19 & 0.05 & 0.19 &  & 0.12 & -0.03 & 0.03 & 0.4 \\ 
  $\nu^{(1)}_{22}$ & 0.24 & 0.14 & 0.31 & 0.6 &  & 0.06 & 0.02 & 0.92 & 0.98 \\ 
  $\beta^{(1)}_{0,11}$ & 0.07 & 0.03 & 0.92 & 0.56 &  & -0.03 & -0.03 & 0.98 & 1 \\ 
  $\beta^{(1)}_{0,21}$ & 0.05 & 0.02 & 0.01 & 0.12 &  & 0.03 & -0.01 & 0.99 & 0.98 \\ 
  $\beta^{(1)}_{0,12}$ & 0.05 & 0.03 & 0.08 & 0.22 &  & 0.05 & 0.02 & 0.98 & 0.86 \\ 
  $\beta^{(1)}_{0,22}$ & 0.08 & 0.03 & 0.9 & 0.67 &  & -0.01 & 0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{1,11}$ & 0.07 & 0.03 & 0.6 & 0.83 &  & 0.02 & 0.01 & 0.98 & 1 \\ 
  $\beta^{(1)}_{1,21}$ & 0.05 & 0.02 & 0.08 & 0.71 &  & -0.02 & -0.03 & 0.99 & 1 \\ 
  $\beta^{(1)}_{1,12}$ & 0.04 & 0.02 & 0.38 & 0.21 &  & 0.02 & -0.01 & 0.99 & 0.98 \\ 
  $\beta^{(1)}_{1,22}$ & 0.01 & 0.02 & 0.62 & 0.58 &  & 0.02 & 0.01 & 0.99 & 1 \\ 
  $\beta^{(1)}_{2,11}$ & 0.1 & 0.05 & 0.52 & 0.7 &  & 0.01 & 0 & 0.98 & 1 \\ 
  $\beta^{(1)}_{2,21}$ & 0.05 & 0.03 & 0.21 & 0.56 &  & 0 & -0.04 & 1 & 1 \\ 
  $\beta^{(1)}_{2,12}$ & 0.03 & 0.01 & 0.08 & 0.07 &  & 0.04 & 0.01 & 0.99 & 0.82 \\ 
  $\beta^{(1)}_{2,22}$ & 0.11 & 0.05 & 0.42 & 0.72 &  & 0.02 & 0.03 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,11}$ & 0.12 & 0.06 & 0.09 & 0.25 &  & -0.02 & -0.03 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,21}$ & 0.06 & 0.02 & 0.08 & 0.28 &  & 0.05 & 0.04 & 0.99 & 0.95 \\ 
  $\beta^{(1)}_{3,12}$ & 0.06 & 0.04 & 0.93 & 0.45 &  & 0.06 & 0.02 & 0.96 & 1 \\ 
  $\beta^{(1)}_{3,22}$ & 0.03 & 0.01 & 0.2 & 0.64 &  & -0.03 & 0.01 & 0.99 & 1 \\ 
  $\sigma^{(1)2}_{11}$ & 0.29 & 0.18 & 0.49 &  &  & 0.12 & 0.01 & 0.3 &  \\ 
  $\sigma^{(1)2}_{21}$ & 0.07 & 0.04 & 0.17 &  &  & 0.01 & -0.01 & 0.46 &  \\ 
  $\sigma^{(1)2}_{12}$ & 0.09 & 0.06 & 0.35 &  &  & 0 & 0.04 & 0.03 &  \\ 
  $\sigma^{(1)2}_{22}$ & 0.01 & 0.01 & 0.2 &  &  & 0.05 & 0.03 & 0.3 &  \\ 
  $\alpha^{(2)}_{1}$ & 0.01 & 0 & 0.51 & 0.86 &  & 0.01 & 0 & 0.7 & 0.66 \\ 
  $\alpha^{(2)}_{2}$ & 0.01 & 0.01 & 0.79 & 0.53 &  & -0.01 & 0.03 & 0.25 & 0.22 \\ 
  $\alpha^{(2)}_{3}$ & 0 & 0 & 0.4 & 0.12 &  & -0.02 & -0.01 & 0.05 & 0.09 \\ 
  $\alpha^{(2)}_{4}$ & 0 & 0 & 0.12 & 0.05 &  & 0.02 & 0 & 0.87 & 0.8 \\ 
  $\nu^{(2)}_{11}$ & 0.21 & 0.14 & 0.95 & 0.75 &  & 0.13 & 0.1 & 0.03 & 0.22 \\ 
  $\nu^{(2)}_{21}$ & 0.21 & 0.21 & 0.82 & 0.09 &  & 0.2 & 0.23 & 0.83 & 0.25 \\ 
  $\nu^{(2)}_{31}$ & 0.12 & 0.11 & 0.49 & 0.6 &  & 0.11 & 0.07 & 0.39 & 0.66 \\ 
  $\nu^{(2)}_{41}$ & 0 & 0 & 0.97 & 0.07 &  & -0.03 & 0.01 & 0.71 & 0.44 \\ 
  $\nu^{(2)}_{12}$ & 0.2 & 0.18 & 0.08 & 0.09 &  & 0.17 & 0.17 & 0.89 & 0.67 \\ 
  $\nu^{(2)}_{22}$ & 0.21 & 0.09 & 0.54 & 0.4 &  & 0.06 & 0.01 & 0.31 & 0.4 \\ 
  $\nu^{(2)}_{32}$ & 0.55 & 0.55 & 0.64 & 0.22 &  & 0.55 & 0.54 & 0.31 & 0.05 \\ 
  $\nu^{(2)}_{42}$ & 0 & 0 & 0.55 & 0.19 &  & -0.01 & -0.02 & 0.68 & 0.24 \\ 
  $\nu^{(2)}_{13}$ & 0.13 & 0.06 & 0.07 & 0.47 &  & 0.02 & 0 & 0.82 & 0.11 \\ 
  $\nu^{(2)}_{23}$ & 0.21 & 0.09 & 0.97 & 0.67 &  & 0.03 & 0.01 & 0.78 & 0.14 \\ 
  $\nu^{(2)}_{33}$ & 0.01 & 0 & 0.74 & 0.99 &  & -0.03 & -0.02 & 0.48 & 0.46 \\ 
  $\nu^{(2)}_{43}$ & 0 & -0.01 & 0.45 & 0.82 &  & 0 & -0.01 & 0.73 & 0.76 \\ 
  $\nu^{(2)}_{14}$ & 0.01 & -0.01 & 0.15 & 0.7 &  & -0.03 & -0.01 & 0.56 & 0.46 \\ 
  $\nu^{(2)}_{24}$ & 0.04 & 0.01 & 0.18 & 0.56 &  & -0.01 & -0.02 & 0.91 & 0.99 \\ 
  $\nu^{(2)}_{34}$ & 0.01 & 0.01 & 0.84 & 0.89 &  & 0.04 & 0.03 & 0.79 & 0.27 \\ 
  $\nu^{(2)}_{44}$ & -0.01 & 0.01 & 0.67 & 0.8 &  & 0.01 & -0.01 & 0.14 & 0.05 \\ 
  $\rho^{(1)}$ & 0.49 & 0.1 & 0.03 & 0.06 &  & 0 & -0.01 & 0.01 & 0.2 \\ 
  $\rho^{(2)}$ & 0.68 & 0.36 & 0.05 & 0.26 &  & 0.22 & 0.06 & 0.14 & 0.77 \\ 
\hline
\multicolumn{10}{l}{\begin{minipage}[hs!]{1\textwidth}
		\textit{Note}: Number of draws used in the diagnostic: 20,000, a burn-in of 10,000 and thinning 10. $AC1$ ($AC5$) are the auto--correlation coefficients at the first (fifth) lag. $GD$ is p--value of the Geweke's convergence diagnostic test, null hypothesis is convergence. $HDS$ and $HDHW$ are the Heidelberger and Welch's convergence diagnostics, where $HDS$ is the p--value (null hypothesis is stationarity). %Same applies to Table \ref{tab: MCMCcon_ba_th}
\end{minipage}	}
\end{tabular}
\end{table}


==> Tables/App_MCMC_conn_res_2_bf_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:43:52 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters before and after thinning} 
\label{tab: MCMCcon_ba_th}
\begin{tabular}{cccccccccc}
  \hline \multirow{2}{3cm}{\centering Parameters} & \multicolumn{4}{c}{Before thinning} & & \multicolumn{4}{c}{After thinning} \\ \cline{2-5} \cline{7-10}V1 & $AC1$ & $AC5$ & $GD$ & $HDS$ & V6 & $AC1$ & $AC5$ & $GD$ & $HDS$ \\ 
  \hline  \hline
$\alpha^{(1)}_{1}$ & 0.02 & 0.01 & 0.65 & 0.54 &  & -0.01 & 0.03 & 0.33 & 0.23 \\ 
  $\alpha^{(1)}_{2}$ & 0.02 & 0.01 & 0.28 & 0.24 &  & -0.01 & 0 & 0.19 & 0.32 \\ 
  $\alpha^{(1)}_{3}$ & 0 & -0.01 & 0.05 & 0.14 &  & -0.02 & -0.03 & 0.15 & 0.14 \\ 
  $\alpha^{(1)}_{4}$ & 0 & 0.01 & 0.01 & 0.07 &  & -0.03 & 0 & 0.37 & 0.44 \\ 
  $\nu^{(1)}_{11}$ & 0.58 & 0.48 & 0.74 & 0.86 &  & 0.42 & 0.19 & 0.87 & 0.84 \\ 
  $\nu^{(1)}_{21}$ & 0.39 & 0.32 & 0.52 & 0.82 &  & 0.26 & 0.1 & 0.33 & 0.84 \\ 
  $\nu^{(1)}_{31}$ & 0.03 & 0.02 & 0.66 & 0.56 &  & -0.03 & -0.02 & 0.11 & 0.11 \\ 
  $\nu^{(1)}_{41}$ & 0.34 & 0.23 & 0.54 & 0.69 &  & 0.19 & 0.05 & 0.68 & 0.43 \\ 
  $\nu^{(1)}_{12}$ & 0.41 & 0.29 & 0.92 & 0.69 &  & 0.23 & 0.02 & 0.99 & 0.6 \\ 
  $\nu^{(1)}_{22}$ & 0.15 & 0.11 & 0.14 & 0.11 &  & 0.09 & 0.03 & 0.19 & 0.53 \\ 
  $\nu^{(1)}_{32}$ & 0.15 & 0.1 & 0.42 & 0.26 &  & 0.06 & 0.03 & 0.26 & 0.15 \\ 
  $\nu^{(1)}_{42}$ & 0.22 & 0.13 & 0.63 & 0.48 &  & 0.06 & 0.01 & 0.44 & 0.53 \\ 
  $\nu^{(1)}_{13}$ & 0.1 & 0.04 & 0.02 & 0.16 &  & 0.03 & -0.01 & 0.13 & 0.42 \\ 
  $\nu^{(1)}_{23}$ & 0.02 & -0.01 & 0.6 & 0.08 &  & 0.08 & 0 & 0.7 & 0.59 \\ 
  $\nu^{(1)}_{33}$ & 0.01 & -0.01 & 0.04 & 0.3 &  & 0 & 0.01 & 0.03 & 0.25 \\ 
  $\nu^{(1)}_{43}$ & 0.1 & 0.04 & 0.75 & 0.38 &  & 0.04 & -0.01 & 0.62 & 0.32 \\ 
  $\nu^{(1)}_{14}$ & 0.28 & 0.21 & 0.8 & 0.98 &  & 0.14 & 0.04 & 0.42 & 0.46 \\ 
  $\nu^{(1)}_{24}$ & 0.35 & 0.27 & 0.49 & 0.9 &  & 0.24 & 0.05 & 0.28 & 0.92 \\ 
  $\nu^{(1)}_{34}$ & 0.03 & 0.03 & 0.29 & 0.38 &  & 0.02 & 0.04 & 0.3 & 0.32 \\ 
  $\nu^{(1)}_{44}$ & 0.19 & 0.11 & 0.68 & 0.56 &  & 0.07 & 0.01 & 0.8 & 0.92 \\ 
  $\beta^{(1)}_{0,11}$ & 0.08 & 0.07 & 0.38 & 0.4 &  & 0.08 & 0.04 & 0.99 & 0.88 \\ 
  $\beta^{(1)}_{0,21}$ & 0.1 & 0.05 & 0.05 & 0.07 &  & 0.05 & 0.03 & 0.99 & 0.81 \\ 
  $\beta^{(1)}_{0,31}$ & 0.16 & 0.08 & 0.67 & 0.57 &  & 0.05 & -0.01 & 0.99 & 1 \\ 
  $\beta^{(1)}_{0,41}$ & 0.05 & 0.03 & 0.23 & 0.18 &  & 0.03 & -0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{0,12}$ & 0.1 & 0.06 & 0.95 & 0.78 &  & 0.03 & 0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{0,22}$ & 0.09 & 0.06 & 0.19 & 0.86 &  & 0.04 & 0 & 1 & 1 \\ 
  $\beta^{(1)}_{0,32}$ & 0.08 & 0.05 & 0.74 & 0.61 &  & 0.05 & 0.02 & 1 & 1 \\ 
  $\beta^{(1)}_{0,42}$ & 0.07 & 0.04 & 0.69 & 0.34 &  & 0.02 & 0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{0,13}$ & 0.09 & 0.05 & 0.06 & 0.58 &  & 0.07 & -0.04 & 0.99 & 1 \\ 
  $\beta^{(1)}_{0,23}$ & 0.04 & 0.02 & 0.5 & 0.66 &  & 0.03 & 0.02 & 0.99 & 0.96 \\ 
  $\beta^{(1)}_{0,33}$ & 0 & 0 & 0.99 & 0.9 &  & -0.01 & -0.03 & 1 & 1 \\ 
  $\beta^{(1)}_{0,43}$ & 0.04 & 0.02 & 0.28 & 0.84 &  & 0.01 & 0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{0,14}$ & 0.04 & 0.01 & 0.95 & 0.86 &  & 0.01 & 0.02 & 0.98 & 1 \\ 
  $\beta^{(1)}_{0,24}$ & 0.07 & 0.03 & 0.16 & 0.3 &  & 0.02 & 0.05 & 0.99 & 1 \\ 
  $\beta^{(1)}_{0,34}$ & 0.03 & 0.01 & 0.99 & 0.11 &  & 0.03 & 0.02 & 1 & 1 \\ 
  $\beta^{(1)}_{0,44}$ & 0.04 & 0.02 & 0.68 & 0.61 &  & 0 & -0.03 & 0.98 & 0.99 \\ 
  $\beta^{(1)}_{1,11}$ & 0.05 & 0.04 & 0.32 & 0.25 &  & -0.01 & 0.02 & 0.99 & 0.94 \\ 
  $\beta^{(1)}_{1,21}$ & 0.05 & 0.02 & 0.99 & 0.25 &  & 0 & 0.03 & 1 & 1 \\ 
  $\beta^{(1)}_{1,31}$ & 0.2 & 0.12 & 0.77 & 0.79 &  & 0.04 & -0.02 & 0.97 & 1 \\ 
  $\beta^{(1)}_{1,41}$ & 0.01 & 0.01 & 0.39 & 0.06 &  & 0.03 & -0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{1,12}$ & 0.04 & 0.02 & 0.41 & 0.16 &  & 0.04 & 0.02 & 0.98 & 1 \\ 
  $\beta^{(1)}_{1,22}$ & 0.08 & 0.04 & 0.47 & 0.72 &  & 0.03 & 0.01 & 0.99 & 1 \\ 
  $\beta^{(1)}_{1,32}$ & 0.13 & 0.1 & 0.66 & 0.99 &  & 0.07 & 0.03 & 0.99 & 1 \\ 
  $\beta^{(1)}_{1,42}$ & 0.02 & 0.01 & 0.58 & 0.24 &  & -0.01 & 0.03 & 0.99 & 1 \\ 
  $\beta^{(1)}_{1,13}$ & 0.02 & 0 & 0.65 & 0.23 &  & 0.02 & -0.01 & 0.98 & 1 \\ 
  $\beta^{(1)}_{1,23}$ & 0.01 & 0.01 & 0.42 & 0.78 &  & 0.01 & -0.02 & 0.98 & 0.97 \\ 
  $\beta^{(1)}_{1,33}$ & -0.02 & -0.01 & 0.72 & 0.87 &  & -0.01 & -0.01 & 1 & 0.98 \\ 
  $\beta^{(1)}_{1,43}$ & 0.03 & 0 & 0.76 & 0.42 &  & 0.01 & 0 & 0.99 & 1 \\ 
  $\beta^{(1)}_{1,14}$ & 0.05 & 0.01 & 0.78 & 0.75 &  & -0.02 & 0.03 & 0.98 & 1 \\ 
  $\beta^{(1)}_{1,24}$ & 0.05 & 0.03 & 0.78 & 0.69 &  & 0.07 & 0.04 & 1 & 1 \\ 
  $\beta^{(1)}_{1,34}$ & 0.09 & 0.04 & 0.32 & 0.41 &  & 0 & -0.01 & 1 & 1 \\ 
  $\beta^{(1)}_{1,44}$ & 0.05 & 0.03 & 0.83 & 0.82 &  & -0.01 & 0.01 & 0.97 & 1 \\ 
  $\beta^{(1)}_{2,11}$ & 0.13 & 0.09 & 0.94 & 0.85 &  & 0.1 & 0.03 & 0.99 & 0.99 \\ 
  $\beta^{(1)}_{2,21}$ & 0.21 & 0.16 & 0.12 & 0.52 &  & 0.13 & 0.05 & 0.99 & 0.99 \\ 
  $\beta^{(1)}_{2,31}$ & 0.03 & 0.01 & 0.76 & 0.66 &  & 0.05 & 0.01 & 0.99 & 1 \\ 
  $\beta^{(1)}_{2,41}$ & 0.09 & 0.05 & 0.16 & 0.08 &  & 0.04 & -0.01 & 0.97 & 0.84 \\ 
  $\beta^{(1)}_{2,12}$ & 0.11 & 0.06 & 0.86 & 0.82 &  & 0.03 & 0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{2,22}$ & 0.25 & 0.18 & 0.19 & 0.89 &  & 0.1 & 0.04 & 0.99 & 1 \\ 
  $\beta^{(1)}_{2,32}$ & 0.01 & 0.01 & 0.61 & 0.15 &  & -0.01 & -0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{2,42}$ & 0.09 & 0.05 & 0.69 & 0.32 &  & 0.05 & 0.02 & 1 & 1 \\ 
  $\beta^{(1)}_{2,13}$ & 0.18 & 0.11 & 0.04 & 0.17 &  & 0.1 & -0.02 & 0.97 & 1 \\ 
  $\beta^{(1)}_{2,23}$ & 0.09 & 0.06 & 0.92 & 0.51 &  & 0.01 & 0.02 & 0.99 & 0.99 \\ 
  $\beta^{(1)}_{2,33}$ & 0.01 & 0 & 0.9 & 0.8 &  & -0.01 & 0 & 1 & 1 \\ 
  $\beta^{(1)}_{2,43}$ & 0.08 & 0.04 & 0.22 & 0.63 &  & 0 & 0 & 0.98 & 0.99 \\ 
  $\beta^{(1)}_{2,14}$ & 0.06 & 0.03 & 0.58 & 0.73 &  & 0.03 & 0.04 & 0.99 & 1 \\ 
  $\beta^{(1)}_{2,24}$ & 0.1 & 0.06 & 0.16 & 0.51 &  & 0.05 & 0 & 1 & 1 \\ 
  $\beta^{(1)}_{2,34}$ & 0 & 0 & 0.31 & 0.12 &  & 0.02 & 0 & 0.99 & 1 \\ 
  $\beta^{(1)}_{2,44}$ & 0.04 & 0.04 & 0.9 & 0.52 &  & 0.06 & -0.05 & 0.99 & 0.98 \\ 
  $\beta^{(1)}_{3,11}$ & 0.11 & 0.06 & 0.35 & 0.05 &  & 0.02 & 0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,21}$ & 0.15 & 0.1 & 0.85 & 0.9 &  & 0.08 & 0.01 & 1 & 1 \\ 
  $\beta^{(1)}_{3,31}$ & 0.06 & 0.02 & 0.64 & 0.17 &  & 0.07 & 0.01 & 1 & 1 \\ 
  $\beta^{(1)}_{3,41}$ & 0.03 & 0.01 & 0.08 & 0.05 &  & -0.04 & -0.01 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,12}$ & 0.08 & 0.05 & 0.48 & 0.64 &  & 0.03 & 0.01 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,22}$ & 0.08 & 0.04 & 0.67 & 0.92 &  & 0 & -0.01 & 0.98 & 1 \\ 
  $\beta^{(1)}_{3,32}$ & 0.06 & 0.04 & 0.02 & 0.15 &  & 0.04 & 0.04 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,42}$ & 0.03 & 0.01 & 0.57 & 0.79 &  & 0 & 0 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,13}$ & 0.03 & 0 & 0.35 & 0.85 &  & -0.01 & 0.02 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,23}$ & 0.04 & 0.02 & 0.47 & 0.69 &  & 0.04 & -0.01 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,33}$ & 0 & 0.01 & 0.47 & 0.85 &  & -0.01 & 0 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,43}$ & 0.03 & 0.01 & 0.35 & 0.76 &  & 0.04 & 0.01 & 0.98 & 0.99 \\ 
  $\beta^{(1)}_{3,14}$ & 0.03 & 0.02 & 0.37 & 0.19 &  & 0 & -0.01 & 0.99 & 1 \\ 
  $\beta^{(1)}_{3,24}$ & 0.05 & 0.01 & 0.64 & 0.62 &  & 0.02 & 0.03 & 1 & 1 \\ 
  $\beta^{(1)}_{3,34}$ & 0.03 & 0.01 & 0.93 & 0.49 &  & 0.02 & 0.01 & 1 & 1 \\ 
  $\beta^{(1)}_{3,44}$ & 0.02 & 0.01 & 0.07 & 0.35 &  & 0.02 & -0.02 & 0.99 & 1 \\ 
  $\sigma^{(1)2}_{11}$ & 0.06 & 0.02 & 0.58 &  &  & 0.02 & 0 & 0.01 &  \\ 
  $\sigma^{(1)2}_{21}$ & 0.41 & 0.35 & 0.75 &  &  & 0.29 & 0.13 & 0.79 &  \\ 
  $\sigma^{(1)2}_{31}$ & 0.16 & 0.08 & 0.38 &  &  & 0.05 & -0.01 & 0.67 &  \\ 
  $\sigma^{(1)2}_{41}$ & 0.04 & 0.02 & 0.28 &  &  & 0.05 & 0.03 & 0.74 &  \\ 
  $\sigma^{(1)2}_{12}$ & 0.08 & 0.06 & 0.57 &  &  & 0.01 & -0.02 & 0.9 &  \\ 
  $\sigma^{(1)2}_{22}$ & 0.56 & 0.45 & 0.87 &  &  & 0.37 & 0.11 & 0.94 &  \\ 
  $\sigma^{(1)2}_{32}$ & 0.07 & 0.04 & 0.45 &  &  & 0.02 & 0 & 0.57 &  \\ 
  $\sigma^{(1)2}_{42}$ & 0.04 & 0 & 0.6 &  &  & 0.01 & 0 & 0.22 &  \\ 
  $\sigma^{(1)2}_{13}$ & 0.12 & 0.07 & 0.63 &  &  & 0.05 & -0.01 & 0.83 &  \\ 
  $\sigma^{(1)2}_{23}$ & 0.17 & 0.14 & 0.65 &  &  & 0.1 & 0.06 & 0.64 &  \\ 
  $\sigma^{(1)2}_{33}$ & 0.02 & 0.01 & 0.92 &  &  & 0 & -0.02 & 0.14 &  \\ 
  $\sigma^{(1)2}_{43}$ & 0.03 & 0 & 0.14 &  &  & -0.01 & 0.05 & 0.99 &  \\ 
  $\sigma^{(1)2}_{14}$ & 0.02 & 0.01 & 0.44 &  &  & 0.01 & 0.02 & 0.29 &  \\ 
  $\sigma^{(1)2}_{24}$ & 0.09 & 0.06 & 0.56 &  &  & 0.04 & 0.02 & 0.8 &  \\ 
  $\sigma^{(1)2}_{34}$ & 0.04 & 0.01 & 0.13 &  &  & 0.03 & -0.01 & 0.57 &  \\ 
  $\sigma^{(1)2}_{44}$ & 0.02 & 0.01 & 0.54 &  &  & -0.01 & -0.03 & 0.2 &  \\ 
  $\alpha^{(2)}_{1}$ & 0 & -0.01 & 0.38 & 0.99 &  & 0 & 0.01 & 0.3 & 0.53 \\ 
  $\alpha^{(2)}_{2}$ & 0 & -0.02 & 0.51 & 0.61 &  & -0.01 & 0 & 0.03 & 0.16 \\ 
  $\alpha^{(2)}_{3}$ & 0 & 0 & 0.4 & 0.68 &  & 0 & -0.01 & 0.69 & 0.98 \\ 
  $\alpha^{(2)}_{4}$ & 0.01 & 0.01 & 0.03 & 0.22 &  & 0 & -0.01 & 0.35 & 0.15 \\ 
  $\nu^{(2)}_{11}$ & 0.02 & -0.01 & 0.95 & 0.23 &  & 0.02 & -0.03 & 0.57 & 0.24 \\ 
  $\nu^{(2)}_{21}$ & 0.03 & 0.02 & 0.71 & 0.25 &  & 0.04 & 0.04 & 0.65 & 0.43 \\ 
  $\nu^{(2)}_{31}$ & 0.01 & 0 & 0.34 & 0.32 &  & 0.01 & 0.01 & 0.82 & 0.51 \\ 
  $\nu^{(2)}_{41}$ & 0.04 & 0.02 & 0.51 & 0.21 &  & 0.04 & -0.01 & 0.85 & 0.27 \\ 
  $\nu^{(2)}_{12}$ & 0.03 & 0.01 & 0.65 & 0.13 &  & 0 & 0.02 & 0.56 & 0.16 \\ 
  $\nu^{(2)}_{22}$ & 0.07 & 0.05 & 0.27 & 0.08 &  & 0.01 & 0 & 0 & 0.14 \\ 
  $\nu^{(2)}_{32}$ & 0.54 & 0.46 & 0.05 & 0.89 &  & 0.4 & 0.23 & 0.09 & 0.76 \\ 
  $\nu^{(2)}_{42}$ & 0.1 & 0.08 & 0.52 & 0.4 &  & 0.04 & 0.07 & 0.06 & 0.61 \\ 
  $\nu^{(2)}_{13}$ & 0.01 & -0.01 & 0.48 & 0.62 &  & -0.01 & -0.03 & 0.71 & 0.11 \\ 
  $\nu^{(2)}_{23}$ & 0.04 & 0.02 & 0.65 & 0.42 &  & 0.02 & 0.02 & 0.76 & 0.46 \\ 
  $\nu^{(2)}_{33}$ & 0.01 & 0 & 0.06 & 0.23 &  & 0.01 & -0.01 & 0.04 & 0.39 \\ 
  $\nu^{(2)}_{43}$ & 0.31 & 0.23 & 0.31 & 0.29 &  & 0.19 & 0.07 & 0.61 & 0.27 \\ 
  $\nu^{(2)}_{14}$ & 0.03 & 0.02 & 0.08 & 0.1 &  & 0 & -0.01 & 0.07 & 0.39 \\ 
  $\nu^{(2)}_{24}$ & 0.12 & 0.1 & 0.54 & 0.13 &  & 0.08 & 0.01 & 0.95 & 0.35 \\ 
  $\nu^{(2)}_{34}$ & 0.05 & 0.04 & 0.01 & 0.5 &  & 0.06 & 0.03 & 0 & 0.12 \\ 
  $\nu^{(2)}_{44}$ & 0.24 & 0.18 & 0.31 & 0.51 &  & 0.13 & 0.08 & 0.94 & 0.87 \\ 
  $\rho^{(1)}$ & 0.8 & 0.55 & 0.28 & 0.32 &  & 0.44 & 0.13 & 0.31 & 0.38 \\ 
  $\rho^{(2)}$ & 0.84 & 0.63 & 0.52 & 0.06 &  & 0.52 & 0.15 & 0.48 & 0.01 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res0.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:33:04 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the transition parameters} 
\label{tab: MCMCtran}
\begin{tabular}{ccccccccccc}
  \hline
Parameters & $\ell$ & $q$ & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0 & 0.88 & 0.55 & 1183.06 & 0.68 & 0.89 & 0 & 23280 \\ 
  $W_{11}$ & 1 & 1 & 0 & 0.87 & 0.52 & 1287.79 & 0.79 & 0.95 & 0 & 29128 \\ 
  $W_{21}$ & 1 & 1 & 0 & 0.73 & 0.26 & 2570.49 & 0.73 & 0.82 & 0.02 & 10598 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0 & 0.78 & 0.36 & 1930.22 & 0.8 & 0.76 & -0.03 & 15894 \\ 
  $intercept$ & 2 & 1 & 0 & 0.98 & 0.88 & 251.52 & 0.41 & 0.2 & -0.01 & 98060 \\ 
  $W_{11}$ & 2 & 1 & 0 & 0.97 & 0.88 & 255.45 & 0.6 & 0.67 & -0.25 & 95796 \\ 
  $W_{21}$ & 2 & 1 & 0 & 0.87 & 0.54 & 878.66 & 0.02 & 0.06 & 0.01 & 28809 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0 & 0.86 & 0.52 & 745.26 & 0.56 & 0.11 & 0.11 & 44916 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res0_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:33:04 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the transition parameters} 
\label{tab: MCMCtran}
\begin{tabular}{ccccccccccc}
  \hline
Parameters & $\ell$ & $q$ & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0 & 0.32 & 0.03 & 1028.44 & 0.49 & 0.92 & 0 &  \\ 
  $W_{11}$ & 1 & 1 & 0 & 0.28 & 0.01 & 1119 & 0.4 & 0.9 & 0 &  \\ 
  $W_{21}$ & 1 & 1 & 0 & 0.13 & 0.01 & 1531.01 & 0.54 & 0.72 & 0.02 &  \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0 & 0.19 & 0.02 & 1366.47 & 0.84 & 0.66 & -0.04 &  \\ 
  $intercept$ & 2 & 1 & 0 & 0.79 & 0.33 & 229.54 & 0.42 & 0.27 & -0.01 &  \\ 
  $W_{11}$ & 2 & 1 & 0 & 0.77 & 0.31 & 260.9 & 0.64 & 0.68 & -0.25 &  \\ 
  $W_{21}$ & 2 & 1 & 0 & 0.37 & 0.09 & 513.01 & 0.04 & 0.22 & 0.01 &  \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0 & 0.35 & 0.11 & 525.71 & 0.48 & 0.24 & 0.14 &  \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res1.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:36:58 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the transition parameters} 
\label{tab: MCMCtran}
\begin{tabular}{ccccccccccc}
  \hline
Parameters & $\ell$ & $q$ & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0 & 0.81 & 0.38 & 1872.87 & 0.31 & 0.79 & 0 & 20814 \\ 
  $W_{11}$ & 1 & 1 & 0 & 0.68 & 0.22 & 2712.25 & 0.72 & 0.3 & 0 & 12369 \\ 
  $W_{21}$ & 1 & 1 & 0 & 0.8 & 0.37 & 1991.66 & 0.14 & 0.82 & 0.05 & 15482 \\ 
  $W_{22}$ & 1 & 1 & 0 & 0.83 & 0.4 & 1864.46 & 0.9 & 0.5 & -0.07 & 21252 \\ 
  $W_{23}$ & 1 & 1 & 0 & 0.54 & 0.17 & 3362.35 & 0.01 & 0.59 & 0.01 & 13302 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0 & 0.71 & 0.26 & 2443.97 & 0.77 & 0.94 & 0.04 & 13656 \\ 
  $W_{11} \cdot W_{22}$ & 1 & 1 & 0 & 0.74 & 0.3 & 2287.69 & 0.02 & 0.09 & 0.03 & 16512 \\ 
  $W_{11} \cdot W_{23}$ & 1 & 1 & 0 & 0.69 & 0.39 & 1001.93 & 0.12 & 0.15 & 0.12 & 49658 \\ 
  $intercept$ & 2 & 1 & 0 & 0.93 & 0.72 & 672.48 & 0.62 & 0.38 & -0.01 & 44634 \\ 
  $W_{11}$ & 2 & 1 & 0 & 0.76 & 0.4 & 898.37 & 0.86 & 0.47 & -0.13 & 29064 \\ 
  $W_{21}$ & 2 & 1 & 0 & 0.95 & 0.77 & 324.31 & 0 & 0.18 & 0.01 & 71654 \\ 
  $W_{22}$ & 2 & 1 & 0 & 0.95 & 0.78 & 330.72 & 0.04 & 0.08 & 0.01 & 59990 \\ 
  $W_{23}$ & 2 & 1 & 0 & 0.95 & 0.87 & 57.86 & 0.52 & 0.78 & -4.65 & 148590 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0 & 0.77 & 0.43 & 777.07 & 0.55 & 0.5 & -1.2 & 42132 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 1 & 0 & 0.83 & 0.56 & 388.47 & 0.34 & 0.56 & -2.89 & 117552 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 1 & 0 & 0.64 & 0.22 & 1442.09 & 0.2 & 0.22 & 10.03 & 25544 \\ 
  $intercept$ & 2 & 2 & 0 & 0.93 & 0.7 & 703.58 & 0.53 & 0.62 & -0.01 & 44936 \\ 
  $W_{11}$ & 2 & 2 & 0 & 0.75 & 0.37 & 1144.16 & 0.09 & 0 &  & 20793 \\ 
  $W_{21}$ & 2 & 2 & 0 & 0.96 & 0.84 & 297.35 & 0.04 & 0.19 & 0.03 & 77056 \\ 
  $W_{22}$ & 2 & 2 & 0 & 0.94 & 0.78 & 445.51 & 0.05 & 0.21 & 0.01 & 62958 \\ 
  $W_{23}$ & 2 & 2 & 0 & 0.95 & 0.85 & 63.68 & 0.4 & 0.24 & -3.16 & 309876 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 2 & 0 & 0.83 & 0.52 & 842.6 & 0.32 & 0.37 & -33.37 & 42371 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 2 & 0 & 0.85 & 0.61 & 243.8 & 0.05 & 0.52 & 0.33 & 198800 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 2 & 0 & 0.67 & 0.26 & 1115.91 & 0.47 & 0.09 & -3.74 & 24132 \\ 
  $intercept$ & 2 & 3 & 0 & 0.93 & 0.72 & 666.3 & 0.87 & 0.51 & -0.01 & 42168 \\ 
  $W_{11}$ & 2 & 3 & 0 & 0.81 & 0.45 & 831.23 & 0.5 & 0.99 & 0.06 & 32358 \\ 
  $W_{21}$ & 2 & 3 & 0 & 0.95 & 0.79 & 394.02 & 0 & 0.52 & 0.01 & 52962 \\ 
  $W_{22}$ & 2 & 3 & 0 & 0.98 & 0.9 & 159.51 & 0.12 & 0.26 & 0.07 & 190484 \\ 
  $W_{23}$ & 2 & 3 & 0 & 0.86 & 0.57 & 623.17 & 0.05 & 0.21 & 0.01 & 48496 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 3 & 0 & 0.81 & 0.45 & 916.34 & 0.9 & 0.65 & 0.14 & 24464 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 3 & 0 & 0.93 & 0.78 & 180.05 & 0.25 & 0.61 & 0.25 & 222633 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 3 & 0 & 0.79 & 0.43 & 1083 & 0 & 0.29 & 0.08 & 31204 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res1_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:36:58 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the transition parameters} 
\label{tab: MCMCtran}
\begin{tabular}{ccccccccccc}
  \hline
Parameters & $\ell$ & $q$ & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0 & 0.17 & -0.01 & 1405.35 & 0.68 & 0.78 & 0 &  \\ 
  $W_{11}$ & 1 & 1 & 0.04 & 0.09 & 0 & 1683.46 & 0.55 & 0.61 & 0 &  \\ 
  $W_{21}$ & 1 & 1 & 0 & 0.18 & -0.01 & 1400.9 & 0.34 & 0.88 & 0.06 &  \\ 
  $W_{22}$ & 1 & 1 & 0 & 0.18 & 0 & 1392.63 & 0.88 & 0.61 & -0.08 &  \\ 
  $W_{23}$ & 1 & 1 & 0.31 & 0.05 & -0.01 & 1794.87 & 0.14 & 0.66 & 0.01 &  \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0 & 0.11 & 0 & 1592.39 & 0.37 & 0.93 & 0.04 &  \\ 
  $W_{11} \cdot W_{22}$ & 1 & 1 & 0 & 0.1 & -0.02 & 1819.07 & 0.15 & 0.13 & 0.03 &  \\ 
  $W_{11} \cdot W_{23}$ & 1 & 1 & 0 & 0.31 & 0.08 & 776.54 & 0.01 & 0.1 & 0.13 &  \\ 
  $intercept$ & 2 & 1 & 0 & 0.52 & 0.11 & 527.37 & 0.69 & 0.46 & -0.01 &  \\ 
  $W_{11}$ & 2 & 1 & 0 & 0.23 & 0.07 & 718.26 & 0.79 & 0.27 & -0.16 &  \\ 
  $W_{21}$ & 2 & 1 & 0 & 0.62 & 0.25 & 289.01 & 0.03 & 0.27 & 0.01 &  \\ 
  $W_{22}$ & 2 & 1 & 0 & 0.63 & 0.25 & 293 & 0.06 & 0.09 & 0.01 &  \\ 
  $W_{23}$ & 2 & 1 & 0 & 0.83 & 0.68 & 46.82 & 0.53 & 0.72 & -4.98 &  \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0 & 0.26 & 0.1 & 659.05 & 0.49 & 0.42 & -1.25 &  \\ 
  $W_{11} \cdot W_{22}$ & 2 & 1 & 0 & 0.43 & 0.22 & 279.86 & 0.54 & 0.86 & -3.1 &  \\ 
  $W_{11} \cdot W_{23}$ & 2 & 1 & 0 & 0.09 & 0.03 & 786.32 & 0.25 & 0.51 & 7.07 &  \\ 
  $intercept$ & 2 & 2 & 0 & 0.5 & 0.03 & 613.78 & 0.77 & 0.6 & -0.01 &  \\ 
  $W_{11}$ & 2 & 2 & 0 & 0.24 & 0.07 & 798.2 & 0.89 & 0.01 &  &  \\ 
  $W_{21}$ & 2 & 2 & 0 & 0.73 & 0.31 & 234.77 & 0.03 & 0.22 & 0.03 &  \\ 
  $W_{22}$ & 2 & 2 & 0 & 0.63 & 0.19 & 380.17 & 0.08 & 0.28 & 0.01 &  \\ 
  $W_{23}$ & 2 & 2 & 0 & 0.82 & 0.68 & 47.4 & 0.4 & 0.45 & -3.94 &  \\ 
  $W_{11} \cdot W_{21}$ & 2 & 2 & 0 & 0.37 & 0.06 & 752.84 & 0.17 & 0.6 & 4.91 &  \\ 
  $W_{11} \cdot W_{22}$ & 2 & 2 & 0 & 0.5 & 0.3 & 110.13 & 0.35 & 0.86 & 0.46 &  \\ 
  $W_{11} \cdot W_{23}$ & 2 & 2 & 0 & 0.19 & 0.09 & 302.34 & 0.63 & 0.58 & -6.54 &  \\ 
  $intercept$ & 2 & 3 & 0 & 0.52 & 0.05 & 528.78 & 0.87 & 0.79 & -0.01 &  \\ 
  $W_{11}$ & 2 & 3 & 0 & 0.33 & 0.07 & 716.3 & 0.42 & 0.95 & 0.06 &  \\ 
  $W_{21}$ & 2 & 3 & 0 & 0.64 & 0.24 & 259.79 & 0 & 0.06 & 0.02 &  \\ 
  $W_{22}$ & 2 & 3 & 0 & 0.83 & 0.52 & 110.08 & 0.17 & 0.55 & 0.09 &  \\ 
  $W_{23}$ & 2 & 3 & 0 & 0.43 & 0.16 & 404.27 & 0.07 & 0.47 & 0.01 &  \\ 
  $W_{11} \cdot W_{21}$ & 2 & 3 & 0 & 0.32 & 0.05 & 767.41 & 0.55 & 0.79 & 0.15 &  \\ 
  $W_{11} \cdot W_{22}$ & 2 & 3 & 0 & 0.69 & 0.42 & 84.79 & 0.33 & 0.89 & 0.36 &  \\ 
  $W_{11} \cdot W_{23}$ & 2 & 3 & 0 & 0.26 & 0.09 & 654.52 & 0.02 & 0.65 & 0.1 &  \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res2.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:43:52 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the transition parameters} 
\label{tab: MCMCtran}
\begin{tabular}{ccccccccccc}
  \hline
Parameters & $\ell$ & $q$ & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0 & 0.61 & 0.12 & 4521.36 & 0.02 & 0.21 & 0 & 9928 \\ 
  $W_{11}$ & 1 & 1 & 0 & 0.82 & 0.54 & 697.37 & 0.03 & 0.31 & 0 & 27708 \\ 
  $W_{12}$ & 1 & 1 & 0 & 0.9 & 0.72 & 278.65 & 0.6 & 0.43 & 0.02 & 48408 \\ 
  $W_{13}$ & 1 & 1 & 0 & 0.94 & 0.88 & 90.7 & 0.02 & 0.14 & -0.47 & 108992 \\ 
  $W_{21}$ & 1 & 1 & 0 & 0.62 & 0.16 & 3776.07 & 0.06 & 0.41 & -0.04 & 10132 \\ 
  $W_{22}$ & 1 & 1 & 0 & 0.64 & 0.15 & 3890.43 & 0.02 & 0.38 & -0.03 & 10192 \\ 
  $W_{23}$ & 1 & 1 & 0 & 0.5 & 0.37 & 711.35 & 0 & 0.24 & -0.46 & 46536 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0 & 0.76 & 0.41 & 1332.91 & 0.21 & 0.42 & 0.23 & 27216 \\ 
  $W_{11} \cdot W_{22}$ & 1 & 1 & 0 & 0.75 & 0.37 & 1355.61 & 0.81 & 0.69 & -0.07 & 25300 \\ 
  $W_{11} \cdot W_{23}$ & 1 & 1 & 0 & 0.41 & 0.22 & 3021.01 & 0.16 & 0.49 & -0.33 & 27225 \\ 
  $W_{12} \cdot W_{21}$ & 1 & 1 & 0 & 0.82 & 0.49 & 1139.64 & 0.4 & 0.48 & -0.17 & 28785 \\ 
  $W_{12} \cdot W_{22}$ & 1 & 1 & 0 & 0.87 & 0.58 & 940.29 & 0.63 & 0.3 & -0.06 & 38412 \\ 
  $W_{12} \cdot W_{23}$ & 1 & 1 & 0 & 0.61 & 0.4 & 1253.35 & 0.74 & 0.18 & -1.13 & 46512 \\ 
  $W_{13} \cdot W_{21}$ & 1 & 1 & 0 & 0.36 & 0.02 & 7055.8 & 0.69 & 0.63 & -4.73 & 9612 \\ 
  $W_{13} \cdot W_{22}$ & 1 & 1 & 0 & 0.64 & 0.29 & 1831.01 & 0.82 & 0.34 & -1.85 & 22448 \\ 
  $W_{13} \cdot W_{23}$ & 1 & 1 & 0 & 0.56 & 0.31 & 1212.41 & 0 & 0.09 & -1.2 & 21476 \\ 
  $intercept$ & 1 & 2 & 0 & 0.87 & 0.55 & 1011.31 & 0.24 & 0.49 & -0.01 & 23646 \\ 
  $W_{11}$ & 1 & 2 & 0 & 0.88 & 0.62 & 699.03 & 0 & 0.1 & 0.01 & 51205 \\ 
  $W_{12}$ & 1 & 2 & 0 & 0.9 & 0.67 & 402.6 & 0.78 & 0.87 & 0.01 & 35166 \\ 
  $W_{13}$ & 1 & 2 & 0 & 0.84 & 0.65 & 377.42 & 0.45 & 0.25 & 0.02 & 44838 \\ 
  $W_{21}$ & 1 & 2 & 0 & 0.81 & 0.42 & 1338.3 & 0.1 & 0.21 & -0.13 & 25960 \\ 
  $W_{22}$ & 1 & 2 & 0 & 0.89 & 0.62 & 585.53 & 0.58 & 0.12 & -0.05 & 69251 \\ 
  $W_{23}$ & 1 & 2 & 0 & 0.56 & 0.42 & 478.49 & 0.81 & 0.17 & 0.07 & 63310 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 2 & 0 & 0.8 & 0.42 & 1186.09 & 0.26 & 0.62 & -0.15 & 30715 \\ 
  $W_{11} \cdot W_{22}$ & 1 & 2 & 0 & 0.82 & 0.44 & 1411.87 & 0.33 & 0.06 & -0.2 & 23880 \\ 
  $W_{11} \cdot W_{23}$ & 1 & 2 & 0 & 0.38 & 0.18 & 3340.54 & 0.16 & 0.07 & 0.05 & 15420 \\ 
  $W_{12} \cdot W_{21}$ & 1 & 2 & 0 & 0.79 & 0.42 & 1117.53 & 0.64 & 0.99 & 0.08 & 29088 \\ 
  $W_{12} \cdot W_{22}$ & 1 & 2 & 0 & 0.83 & 0.51 & 649.05 & 0.19 & 0.16 & 0.07 & 25842 \\ 
  $W_{12} \cdot W_{23}$ & 1 & 2 & 0 & 0.46 & 0.24 & 1644.07 & 0.32 & 0.56 & 0.16 & 21700 \\ 
  $W_{13} \cdot W_{21}$ & 1 & 2 & 0 & 0.56 & 0.25 & 1331.4 & 0.46 & 0.61 & 0.05 & 22728 \\ 
  $W_{13} \cdot W_{22}$ & 1 & 2 & 0 & 0.71 & 0.38 & 1225.03 & 0.63 & 0.38 & -0.16 & 42360 \\ 
  $W_{13} \cdot W_{23}$ & 1 & 2 & 0 & 0.51 & 0.26 & 1299.57 & 0.29 & 0.07 & 0.22 & 15411 \\ 
  $intercept$ & 1 & 3 & 0 & 0.95 & 0.8 & 383.32 & 0.03 & 0.21 & -0.01 & 42348 \\ 
  $W_{11}$ & 1 & 3 & 0 & 0.97 & 0.9 & 139.13 & 0.03 & 0.18 & 0.12 & 97150 \\ 
  $W_{12}$ & 1 & 3 & 0 & 0.94 & 0.77 & 409.74 & 0.01 & 0.43 & 0.02 & 38476 \\ 
  $W_{13}$ & 1 & 3 & 0 & 0.84 & 0.67 & 349.23 & 0.32 & 0.11 & 0.01 & 57618 \\ 
  $W_{21}$ & 1 & 3 & 0 & 0.88 & 0.6 & 689.02 & 0.49 & 0.44 & -0.14 & 51808 \\ 
  $W_{22}$ & 1 & 3 & 0 & 0.89 & 0.64 & 685.79 & 0.83 & 0.99 & 0.64 & 40704 \\ 
  $W_{23}$ & 1 & 3 & 0 & 0.64 & 0.45 & 477.95 & 0.25 & 0.15 & 0.1 & 23220 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 3 & 0 & 0.86 & 0.54 & 896.73 & 0.58 & 0.9 & 0.69 & 33850 \\ 
  $W_{11} \cdot W_{22}$ & 1 & 3 & 0 & 0.88 & 0.58 & 881.05 & 0.57 & 0.96 & -1 & 49236 \\ 
  $W_{11} \cdot W_{23}$ & 1 & 3 & 0 & 0.55 & 0.18 & 3454.6 & 0.09 & 0.34 & -0.97 & 17460 \\ 
  $W_{12} \cdot W_{21}$ & 1 & 3 & 0 & 0.85 & 0.53 & 926.18 & 0.45 & 0.9 & 0.1 & 34132 \\ 
  $W_{12} \cdot W_{22}$ & 1 & 3 & 0 & 0.83 & 0.47 & 1216.74 & 0.46 & 0.9 & 0.09 & 33744 \\ 
  $W_{12} \cdot W_{23}$ & 1 & 3 & 0 & 0.62 & 0.36 & 1320.78 & 0.42 & 0.14 & 0.09 & 27265 \\ 
  $W_{13} \cdot W_{21}$ & 1 & 3 & 0 & 0.46 & 0.16 & 3039.03 & 0.74 & 0.68 & -0.04 & 15159 \\ 
  $W_{13} \cdot W_{22}$ & 1 & 3 & 0 & 0.7 & 0.36 & 1497.74 & 0.73 & 0.75 & 0.06 & 33540 \\ 
  $W_{13} \cdot W_{23}$ & 1 & 3 & 0 & 0.5 & 0.23 & 1380.73 & 0.42 & 0.22 & 0.1 & 16323 \\ 
  $intercept$ & 2 & 1 & 0 & 0.93 & 0.74 & 458.08 & 0.88 & 0.99 & -0.01 & 44988 \\ 
  $W_{11}$ & 2 & 1 & 0 & 0.9 & 0.65 & 693.3 & 0.55 & 0.77 & -0.11 & 42664 \\ 
  $W_{12}$ & 2 & 1 & 0 & 0.9 & 0.63 & 669.4 & 0.55 & 0.32 & -0.16 & 51606 \\ 
  $W_{13}$ & 2 & 1 & 0 & 0.75 & 0.47 & 667.3 & 0.06 & 0.06 & -0.13 & 31227 \\ 
  $W_{21}$ & 2 & 1 & 0 & 0.92 & 0.73 & 420.01 & 0.33 & 0.44 & 0.01 & 48391 \\ 
  $W_{22}$ & 2 & 1 & 0 & 0.94 & 0.76 & 463.48 & 0.34 & 0.41 & 0.02 & 35755 \\ 
  $W_{23}$ & 2 & 1 & 0 & 0.94 & 0.91 & 62.28 & 0.55 & 0.18 & -1.22 & 209040 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0 & 0.86 & 0.53 & 887.19 & 0.48 & 0.7 & 0.15 & 34870 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 1 & 0 & 0.87 & 0.55 & 1039.79 & 0.15 & 0.85 & 0.14 & 27126 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 1 & 0 & 0.49 & 0.13 & 4057.82 & 0.82 & 0.59 & -1.47 & 16629 \\ 
  $W_{12} \cdot W_{21}$ & 2 & 1 & 0 & 0.82 & 0.44 & 1114.42 & 0.04 & 0.18 & -0.1 & 20337 \\ 
  $W_{12} \cdot W_{22}$ & 2 & 1 & 0 & 0.88 & 0.58 & 835.15 & 0.69 & 0.52 & -0.15 & 44515 \\ 
  $W_{12} \cdot W_{23}$ & 2 & 1 & 0 & 0.58 & 0.38 & 1147.69 & 0.63 & 0.38 & 2.68 & 23328 \\ 
  $W_{13} \cdot W_{21}$ & 2 & 1 & 0 & 0.5 & 0.13 & 3742.82 & 0.53 & 0.36 & -3.31 & 15576 \\ 
  $W_{13} \cdot W_{22}$ & 2 & 1 & 0 & 0.77 & 0.47 & 1057.41 & 0.87 & 0.81 & -0.16 & 54774 \\ 
  $W_{13} \cdot W_{23}$ & 2 & 1 & 0 & 0.55 & 0.36 & 1057.41 & 0.12 & 0.36 & -1.67 & 38456 \\ 
  $intercept$ & 2 & 2 & 0 & 0.81 & 0.4 & 1607.47 & 0.69 & 0.41 & 0 & 24186 \\ 
  $W_{11}$ & 2 & 2 & 0 & 0.82 & 0.41 & 1550.66 & 0.53 & 0.66 & -0.04 & 20144 \\ 
  $W_{12}$ & 2 & 2 & 0 & 0.79 & 0.35 & 1801.11 & 0.15 & 0.75 & -0.42 & 18429 \\ 
  $W_{13}$ & 2 & 2 & 0 & 0.69 & 0.39 & 959.18 & 0.54 & 0.1 & 0.03 & 15774 \\ 
  $W_{21}$ & 2 & 2 & 0 & 0.93 & 0.74 & 339.43 & 0.72 & 0.15 & 0.03 & 52552 \\ 
  $W_{22}$ & 2 & 2 & 0 & 0.8 & 0.37 & 1689.86 & 0.63 & 0.11 & 0 & 18951 \\ 
  $W_{23}$ & 2 & 2 & 0 & 0.91 & 0.87 & 70.25 & 0.96 & 0.22 & -0.55 & 114169 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 2 & 0 & 0.9 & 0.63 & 714.66 & 0.19 & 0.06 & 0.08 & 42680 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 2 & 0 & 0.76 & 0.32 & 1977.55 & 0.22 & 0.19 & -0.06 & 19856 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 2 & 0 & 0.52 & 0.18 & 3686.09 & 0.08 & 0.24 & -1.89 & 15645 \\ 
  $W_{12} \cdot W_{21}$ & 2 & 2 & 0 & 0.87 & 0.56 & 732.48 & 0.68 & 0.17 & 0.11 & 67522 \\ 
  $W_{12} \cdot W_{22}$ & 2 & 2 & 0 & 0.75 & 0.29 & 2211.6 & 0.17 & 0.53 & -0.11 & 14469 \\ 
  $W_{12} \cdot W_{23}$ & 2 & 2 & 0 & 0.63 & 0.47 & 538.58 & 0.03 & 0.32 & -3.22 & 28235 \\ 
  $W_{13} \cdot W_{21}$ & 2 & 2 & 0 & 0.54 & 0.16 & 2901.48 & 0.19 & 0.27 & 0.18 & 20480 \\ 
  $W_{13} \cdot W_{22}$ & 2 & 2 & 0 & 0.77 & 0.48 & 764.87 & 0.37 & 0 &  & 23056 \\ 
  $W_{13} \cdot W_{23}$ & 2 & 2 & 0 & 0.56 & 0.42 & 690.27 & 0.89 & 0.92 & -0.66 & 40530 \\ 
  $intercept$ & 2 & 3 & 0 & 0.93 & 0.71 & 581.65 & 0.12 & 0.89 & -0.01 & 52146 \\ 
  $W_{11}$ & 2 & 3 & 0 & 0.91 & 0.65 & 633.85 & 0.73 & 0.39 & 0.12 & 48708 \\ 
  $W_{12}$ & 2 & 3 & 0 & 0.9 & 0.65 & 563.06 & 0.15 & 0.92 & 0.04 & 56640 \\ 
  $W_{13}$ & 2 & 3 & 0 & 0.75 & 0.41 & 1066.04 & 0.72 & 0.3 & 0.19 & 19264 \\ 
  $W_{21}$ & 2 & 3 & 0 & 0.96 & 0.85 & 169.93 & 0.98 & 0.21 & 0.11 & 82731 \\ 
  $W_{22}$ & 2 & 3 & 0 & 0.94 & 0.75 & 438.07 & 0.72 & 0.09 & 0.04 & 71596 \\ 
  $W_{23}$ & 2 & 3 & 0 & 0.73 & 0.61 & 327.39 & 0.24 & 0.52 & 0.01 & 66264 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 3 & 0 & 0.87 & 0.57 & 799.76 & 0.06 & 0.26 & -0.8 & 37205 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 3 & 0 & 0.9 & 0.63 & 673.28 & 0.88 & 0.1 & 0.07 & 70048 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 3 & 0 & 0.51 & 0.21 & 3091.52 & 0.63 & 0.45 & 0.17 & 18784 \\ 
  $W_{12} \cdot W_{21}$ & 2 & 3 & 0 & 0.87 & 0.56 & 732.95 & 0.02 & 0.08 & 0.16 & 39354 \\ 
  $W_{12} \cdot W_{22}$ & 2 & 3 & 0 & 0.86 & 0.51 & 1157.21 & 0.08 & 0.09 & 0.1 & 31080 \\ 
  $W_{12} \cdot W_{23}$ & 2 & 3 & 0 & 0.6 & 0.41 & 898.17 & 0.06 & 0.7 & 0.17 & 37536 \\ 
  $W_{13} \cdot W_{21}$ & 2 & 3 & 0 & 0.52 & 0.09 & 5134.25 & 0.64 & 0.49 & -1.82 & 10900 \\ 
  $W_{13} \cdot W_{22}$ & 2 & 3 & 0 & 0.75 & 0.41 & 1179.14 & 0.98 & 0.07 & -0.16 & 24532 \\ 
  $W_{13} \cdot W_{23}$ & 2 & 3 & 0 & 0.57 & 0.37 & 921.57 & 0.37 & 0.1 & 0.08 & 37752 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res2_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:43:52 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the transition parameters} 
\label{tab: MCMCtran}
\begin{tabular}{ccccccccccc}
  \hline
Parameters & $\ell$ & $q$ & $LBT$ & $AC1$ & $AC5$ & $ES$ & $GD$ & $HDS$ & $HDHW$ & NrRaf \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0.45 & 0.02 & 0.01 & 2000 & 0.05 & 0.61 & 0 &  \\ 
  $W_{11}$ & 1 & 1 & 0 & 0.44 & 0.1 & 615.08 & 0.04 & 0.16 & 0 &  \\ 
  $W_{12}$ & 1 & 1 & 0 & 0.63 & 0.29 & 263.56 & 0.69 & 0.61 & 0.02 &  \\ 
  $W_{13}$ & 1 & 1 & 0 & 0.83 & 0.6 & 94.71 & 0.02 & 0.18 & -0.46 &  \\ 
  $W_{21}$ & 1 & 1 & 0.01 & 0.05 & 0.02 & 1608.24 & 0.04 & 0.23 & -0.07 &  \\ 
  $W_{22}$ & 1 & 1 & 0.07 & 0.03 & 0.04 & 1865.8 & 0.13 & 0.66 & -0.04 &  \\ 
  $W_{23}$ & 1 & 1 & 0 & 0.31 & 0.18 & 328.38 & 0.01 & 0.38 & -0.73 &  \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0 & 0.25 & 0 & 977.14 & 0.47 & 0.4 & 0.28 &  \\ 
  $W_{11} \cdot W_{22}$ & 1 & 1 & 0 & 0.24 & 0.01 & 975.76 & 0.83 & 0.22 & -0.08 &  \\ 
  $W_{11} \cdot W_{23}$ & 1 & 1 & 0 & 0.09 & 0.04 & 1491.17 & 0.11 & 0.77 & -0.46 &  \\ 
  $W_{12} \cdot W_{21}$ & 1 & 1 & 0 & 0.32 & 0.06 & 806.6 & 0.38 & 0.72 & -0.19 &  \\ 
  $W_{12} \cdot W_{22}$ & 1 & 1 & 0 & 0.4 & 0.03 & 815.49 & 0.98 & 0.68 & -0.06 &  \\ 
  $W_{12} \cdot W_{23}$ & 1 & 1 & 0 & 0.28 & 0.02 & 937.28 & 0.49 & 0.54 & -0.83 &  \\ 
  $W_{13} \cdot W_{21}$ & 1 & 1 & 0.09 & 0.02 & 0.02 & 2090.6 & 0.49 & 0.78 & 2.36 &  \\ 
  $W_{13} \cdot W_{22}$ & 1 & 1 & 0 & 0.15 & 0.04 & 1116.88 & 0.88 & 0.63 & -11.99 &  \\ 
  $W_{13} \cdot W_{23}$ & 1 & 1 & 0 & 0.21 & 0.05 & 1002.15 & 0.01 & 0.19 & -1.21 &  \\ 
  $intercept$ & 1 & 2 & 0 & 0.37 & 0.07 & 756.33 & 0.28 & 0.47 & -0.01 &  \\ 
  $W_{11}$ & 1 & 2 & 0 & 0.47 & 0.09 & 576.96 & 0.01 & 0.12 & 0.01 &  \\ 
  $W_{12}$ & 1 & 2 & 0 & 0.55 & 0.26 & 266.14 & 0.72 & 0.97 & 0.01 &  \\ 
  $W_{13}$ & 1 & 2 & 0 & 0.56 & 0.28 & 242.59 & 0.88 & 0.29 & 0.03 &  \\ 
  $W_{21}$ & 1 & 2 & 0 & 0.25 & 0.02 & 888.24 & 0.24 & 0.82 & -0.16 &  \\ 
  $W_{22}$ & 1 & 2 & 0 & 0.48 & 0.1 & 447.74 & 0.42 & 0.08 & -0.05 &  \\ 
  $W_{23}$ & 1 & 2 & 0 & 0.32 & 0.15 & 321.16 & 0.49 & 0.07 & 0.08 &  \\ 
  $W_{11} \cdot W_{21}$ & 1 & 2 & 0 & 0.23 & 0.01 & 1140.1 & 0.05 & 0.24 & -0.15 &  \\ 
  $W_{11} \cdot W_{22}$ & 1 & 2 & 0 & 0.23 & -0.03 & 1288.22 & 0.37 & 0.05 & -0.19 &  \\ 
  $W_{11} \cdot W_{23}$ & 1 & 2 & 0 & 0.1 & 0.02 & 1525.51 & 0.75 & 0.49 & 0.08 &  \\ 
  $W_{12} \cdot W_{21}$ & 1 & 2 & 0 & 0.25 & 0.04 & 1019.14 & 0.55 & 0.93 & 0.08 &  \\ 
  $W_{12} \cdot W_{22}$ & 1 & 2 & 0 & 0.35 & 0.07 & 430.9 & 0.17 & 0.08 & 0.08 &  \\ 
  $W_{12} \cdot W_{23}$ & 1 & 2 & 0 & 0.17 & 0.02 & 1050.51 & 0.09 & 0.39 & 0.18 &  \\ 
  $W_{13} \cdot W_{21}$ & 1 & 2 & 0 & 0.17 & 0.03 & 1087.09 & 0.43 & 0.5 & 0.06 &  \\ 
  $W_{13} \cdot W_{22}$ & 1 & 2 & 0 & 0.23 & 0.05 & 921.46 & 0.27 & 0.38 & -0.19 &  \\ 
  $W_{13} \cdot W_{23}$ & 1 & 2 & 0 & 0.2 & 0.06 & 881.03 & 0.6 & 0.16 & 0.22 &  \\ 
  $intercept$ & 1 & 3 & 0 & 0.67 & 0.2 & 319.33 & 0.02 & 0.15 & -0.01 &  \\ 
  $W_{11}$ & 1 & 3 & 0 & 0.83 & 0.52 & 125.56 & 0.05 & 0.09 & 0.13 &  \\ 
  $W_{12}$ & 1 & 3 & 0 & 0.63 & 0.2 & 342.39 & 0.01 & 0.07 & 0.02 &  \\ 
  $W_{13}$ & 1 & 3 & 0 & 0.56 & 0.29 & 252.54 & 0.46 & 0.09 & 0.01 &  \\ 
  $W_{21}$ & 1 & 3 & 0 & 0.45 & 0.08 & 650.63 & 0.25 & 0.31 & -0.15 &  \\ 
  $W_{22}$ & 1 & 3 & 0 & 0.48 & 0.1 & 560.78 & 0.83 & 0.98 & 0.69 &  \\ 
  $W_{23}$ & 1 & 3 & 0 & 0.34 & 0.16 & 366.77 & 0.16 & 0.32 & 0.12 &  \\ 
  $W_{11} \cdot W_{21}$ & 1 & 3 & 0 & 0.35 & 0.05 & 748.99 & 0.4 & 0.77 & 0.89 &  \\ 
  $W_{11} \cdot W_{22}$ & 1 & 3 & 0 & 0.4 & 0.01 & 715.8 & 0.56 & 0.95 & -1.11 &  \\ 
  $W_{11} \cdot W_{23}$ & 1 & 3 & 0 & 0.1 & -0.01 & 1416.84 & 0.63 & 0.38 & -0.81 &  \\ 
  $W_{12} \cdot W_{21}$ & 1 & 3 & 0 & 0.35 & 0.07 & 645.65 & 0.8 & 0.9 & 0.12 &  \\ 
  $W_{12} \cdot W_{22}$ & 1 & 3 & 0 & 0.28 & 0.04 & 950.76 & 0.41 & 0.92 & 0.11 &  \\ 
  $W_{12} \cdot W_{23}$ & 1 & 3 & 0 & 0.23 & 0.08 & 824.71 & 0.96 & 0.34 & 0.11 &  \\ 
  $W_{13} \cdot W_{21}$ & 1 & 3 & 0 & 0.11 & -0.03 & 1471.43 & 0.36 & 0.3 & -0.06 &  \\ 
  $W_{13} \cdot W_{22}$ & 1 & 3 & 0 & 0.22 & 0.06 & 986.88 & 0.88 & 0.76 & 0.07 &  \\ 
  $W_{13} \cdot W_{23}$ & 1 & 3 & 0 & 0.13 & 0.02 & 982.77 & 0.37 & 0.42 & 0.12 &  \\ 
  $intercept$ & 2 & 1 & 0 & 0.6 & 0.09 & 449.22 & 0.69 & 0.94 & -0.01 &  \\ 
  $W_{11}$ & 2 & 1 & 0 & 0.48 & 0.1 & 612.84 & 0.84 & 0.63 & -0.11 &  \\ 
  $W_{12}$ & 2 & 1 & 0 & 0.46 & 0.08 & 626.36 & 0.8 & 0.19 & -0.17 &  \\ 
  $W_{13}$ & 2 & 1 & 0 & 0.37 & 0.08 & 497.61 & 0.13 & 0.19 & -0.15 &  \\ 
  $W_{21}$ & 2 & 1 & 0 & 0.59 & 0.2 & 367.13 & 0.24 & 0.32 & 0.01 &  \\ 
  $W_{22}$ & 2 & 1 & 0 & 0.61 & 0.16 & 383.48 & 0.36 & 0.4 & 0.02 &  \\ 
  $W_{23}$ & 2 & 1 & 0 & 0.87 & 0.72 & 55 & 0.54 & 0.21 & -1.32 &  \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0 & 0.35 & 0.03 & 810.76 & 0.85 & 0.87 & 0.16 &  \\ 
  $W_{11} \cdot W_{22}$ & 2 & 1 & 0 & 0.34 & 0.05 & 660.8 & 0.16 & 0.91 & 0.18 &  \\ 
  $W_{11} \cdot W_{23}$ & 2 & 1 & 0.05 & 0.03 & 0.02 & 1882.69 & 0.71 & 0.68 & -3.34 &  \\ 
  $W_{12} \cdot W_{21}$ & 2 & 1 & 0 & 0.29 & 0.04 & 929.98 & 0.01 & 0.08 & -0.11 &  \\ 
  $W_{12} \cdot W_{22}$ & 2 & 1 & 0 & 0.38 & 0.06 & 707.13 & 0.85 & 0.73 & -0.16 &  \\ 
  $W_{12} \cdot W_{23}$ & 2 & 1 & 0 & 0.24 & 0.06 & 919.33 & 0.28 & 0.07 & -2.5 &  \\ 
  $W_{13} \cdot W_{21}$ & 2 & 1 & 0 & 0.14 & 0 & 1517.43 & 0.77 & 0.79 & -5.41 &  \\ 
  $W_{13} \cdot W_{22}$ & 2 & 1 & 0 & 0.29 & 0.07 & 787.65 & 0.77 & 0.82 & -0.2 &  \\ 
  $W_{13} \cdot W_{23}$ & 2 & 1 & 0 & 0.27 & 0.05 & 794.99 & 0.54 & 0.82 & -1.96 &  \\ 
  $intercept$ & 2 & 2 & 0 & 0.24 & 0.03 & 1157.42 & 0.78 & 0.63 & 0 &  \\ 
  $W_{11}$ & 2 & 2 & 0 & 0.21 & -0.01 & 1141.55 & 0.55 & 0.7 & -0.05 &  \\ 
  $W_{12}$ & 2 & 2 & 0 & 0.22 & 0.03 & 1198.21 & 0.75 & 0.93 & -0.63 &  \\ 
  $W_{13}$ & 2 & 2 & 0 & 0.29 & 0.09 & 620.35 & 0.46 & 0.26 & 0.03 &  \\ 
  $W_{21}$ & 2 & 2 & 0 & 0.59 & 0.25 & 287.3 & 0.64 & 0.33 & 0.03 &  \\ 
  $W_{22}$ & 2 & 2 & 0 & 0.22 & 0.03 & 1074.45 & 0.53 & 0.14 & 0 &  \\ 
  $W_{23}$ & 2 & 2 & 0 & 0.84 & 0.67 & 65.23 & 0.91 & 0.39 & -0.56 &  \\ 
  $W_{11} \cdot W_{21}$ & 2 & 2 & 0 & 0.42 & 0.01 & 695.06 & 0.26 & 0.06 & 0.08 &  \\ 
  $W_{11} \cdot W_{22}$ & 2 & 2 & 0 & 0.16 & -0.03 & 1453.37 & 0.16 & 0.14 & -0.07 &  \\ 
  $W_{11} \cdot W_{23}$ & 2 & 2 & 0.35 & 0.01 & -0.01 & 2000 & 0.23 & 0.41 & -6.99 &  \\ 
  $W_{12} \cdot W_{21}$ & 2 & 2 & 0 & 0.38 & 0.08 & 658.4 & 0.71 & 0.26 & 0.12 &  \\ 
  $W_{12} \cdot W_{22}$ & 2 & 2 & 0 & 0.15 & 0.04 & 1374.79 & 0.37 & 0.7 & -0.13 &  \\ 
  $W_{12} \cdot W_{23}$ & 2 & 2 & 0 & 0.38 & 0.17 & 440.66 & 0.09 & 0.56 & -31.84 &  \\ 
  $W_{13} \cdot W_{21}$ & 2 & 2 & 0 & 0.09 & 0.03 & 1547.56 & 0.93 & 0.91 & 0.27 &  \\ 
  $W_{13} \cdot W_{22}$ & 2 & 2 & 0 & 0.37 & 0.13 & 462.76 & 0.31 & 0.11 & -0.04 &  \\ 
  $W_{13} \cdot W_{23}$ & 2 & 2 & 0 & 0.35 & 0.1 & 557.53 & 0.78 & 0.59 & -1.26 &  \\ 
  $intercept$ & 2 & 3 & 0 & 0.55 & 0.08 & 574.78 & 0.33 & 0.99 & -0.01 &  \\ 
  $W_{11}$ & 2 & 3 & 0 & 0.47 & 0.11 & 508.53 & 0.99 & 0.34 & 0.13 &  \\ 
  $W_{12}$ & 2 & 3 & 0 & 0.51 & 0.1 & 539.13 & 0.19 & 0.98 & 0.04 &  \\ 
  $W_{13}$ & 2 & 3 & 0 & 0.28 & 0.08 & 757.71 & 0.82 & 0.26 & 0.22 &  \\ 
  $W_{21}$ & 2 & 3 & 0 & 0.77 & 0.45 & 179.62 & 0.96 & 0.17 & 0.11 &  \\ 
  $W_{22}$ & 2 & 3 & 0 & 0.62 & 0.15 & 425.38 & 0.97 & 0.1 & 0.04 &  \\ 
  $W_{23}$ & 2 & 3 & 0 & 0.54 & 0.29 & 256.9 & 0.28 & 0.49 & 0.02 &  \\ 
  $W_{11} \cdot W_{21}$ & 2 & 3 & 0 & 0.4 & 0.08 & 696.71 & 0.24 & 0.33 & -0.84 &  \\ 
  $W_{11} \cdot W_{22}$ & 2 & 3 & 0 & 0.47 & 0.09 & 440.17 & 0.78 & 0.18 & 0.09 &  \\ 
  $W_{11} \cdot W_{23}$ & 2 & 3 & 0 & 0.08 & 0.01 & 1648.64 & 0.46 & 0.82 & 0.24 &  \\ 
  $W_{12} \cdot W_{21}$ & 2 & 3 & 0 & 0.39 & 0.1 & 462.52 & 0.05 & 0.24 & 0.19 &  \\ 
  $W_{12} \cdot W_{22}$ & 2 & 3 & 0 & 0.32 & 0.07 & 769.6 & 0.38 & 0.24 & 0.12 &  \\ 
  $W_{12} \cdot W_{23}$ & 2 & 3 & 0 & 0.3 & 0.06 & 754.57 & 0.32 & 0.91 & 0.21 &  \\ 
  $W_{13} \cdot W_{21}$ & 2 & 3 & 0.71 & 0.04 & 0 & 1855.21 & 0.98 & 0.73 & -3.58 &  \\ 
  $W_{13} \cdot W_{22}$ & 2 & 3 & 0 & 0.26 & 0.04 & 986.89 & 0.68 & 0.1 & -0.18 &  \\ 
  $W_{13} \cdot W_{23}$ & 2 & 3 & 0 & 0.27 & 0.11 & 613.8 & 0.21 & 0.2 & 0.1 &  \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res_0_bf_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:33:04 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters before and after thinning} 
\label{tab: MCMCtran_ba_th}
\begin{tabular}{cccccccccccc}
  \hline \multirow{2}{3cm}{\centering Parameters} & \multirow{2}{1cm}{\centering $\ell$} & \multirow{2}{1cm}{\centering $q$}  & \multicolumn{4}{c}{Before thinning} & & \multicolumn{4}{c}{After thinning} \\ \cline{4-7} \cline{9-12}V1 & $\ell$ & $q$ & $AC1$ & $AC5$ & $GD$ & $HDS$ & V8 & $AC1$ & $AC5$ & $GD$ & $HDS$ \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0.88 & 0.55 & 0.68 & 0.89 &  & 0.32 & 0.03 & 0.49 & 0.92 \\ 
  $W_{11}$ & 1 & 1 & 0.87 & 0.52 & 0.79 & 0.95 &  & 0.28 & 0.01 & 0.4 & 0.9 \\ 
  $W_{21}$ & 1 & 1 & 0.73 & 0.26 & 0.73 & 0.82 &  & 0.13 & 0.01 & 0.54 & 0.72 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0.78 & 0.36 & 0.8 & 0.76 &  & 0.19 & 0.02 & 0.84 & 0.66 \\ 
  $intercept$ & 2 & 1 & 0.98 & 0.88 & 0.41 & 0.2 &  & 0.79 & 0.33 & 0.42 & 0.27 \\ 
  $W_{11}$ & 2 & 1 & 0.97 & 0.88 & 0.6 & 0.67 &  & 0.77 & 0.31 & 0.64 & 0.68 \\ 
  $W_{21}$ & 2 & 1 & 0.87 & 0.54 & 0.02 & 0.06 &  & 0.37 & 0.09 & 0.04 & 0.22 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0.86 & 0.52 & 0.56 & 0.11 &  & 0.35 & 0.11 & 0.48 & 0.24 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res_1_bf_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:36:58 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters before and after thinning under $Q^{(1)}=2$ and $Q^{(2)}=4$.} 
\label{tab: MCMCtran_ba_th}
\scriptsize
\begin{tabular}{cccccccccccc}
  \hline \multirow{2}{3cm}{\centering Parameters} & \multirow{2}{1cm}{\centering $\ell$} & \multirow{2}{1cm}{\centering $q$}  & \multicolumn{4}{c}{Before thinning} & & \multicolumn{4}{c}{After thinning} \\ \cline{4-7} \cline{9-12} &  &  & $AC1$ & $AC5$ & $GD$ & $HDS$ &  & $AC1$ & $AC5$ & $GD$ & $HDS$ \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0.81 & 0.38 & 0.31 & 0.79 &  & 0.17 & -0.01 & 0.68 & 0.78 \\ 
  $W_{11}$ & 1 & 1 & 0.68 & 0.22 & 0.72 & 0.3 &  & 0.09 & 0 & 0.55 & 0.61 \\ 
  $W_{21}$ & 1 & 1 & 0.8 & 0.37 & 0.14 & 0.82 &  & 0.18 & -0.01 & 0.34 & 0.88 \\ 
  $W_{22}$ & 1 & 1 & 0.83 & 0.4 & 0.9 & 0.5 &  & 0.18 & 0 & 0.88 & 0.61 \\ 
  $W_{23}$ & 1 & 1 & 0.54 & 0.17 & 0.01 & 0.59 &  & 0.05 & -0.01 & 0.14 & 0.66 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0.71 & 0.26 & 0.77 & 0.94 &  & 0.11 & 0 & 0.37 & 0.93 \\ 
  $W_{11} \cdot W_{22}$ & 1 & 1 & 0.74 & 0.3 & 0.02 & 0.09 &  & 0.1 & -0.02 & 0.15 & 0.13 \\ 
  $W_{11} \cdot W_{23}$ & 1 & 1 & 0.69 & 0.39 & 0.12 & 0.15 &  & 0.31 & 0.08 & 0.01 & 0.1 \\ 
  $intercept$ & 2 & 1 & 0.93 & 0.72 & 0.62 & 0.38 &  & 0.52 & 0.11 & 0.69 & 0.46 \\ 
  $W_{11}$ & 2 & 1 & 0.76 & 0.4 & 0.86 & 0.47 &  & 0.23 & 0.07 & 0.79 & 0.27 \\ 
  $W_{21}$ & 2 & 1 & 0.95 & 0.77 & 0 & 0.18 &  & 0.62 & 0.25 & 0.03 & 0.27 \\ 
  $W_{22}$ & 2 & 1 & 0.95 & 0.78 & 0.04 & 0.08 &  & 0.63 & 0.25 & 0.06 & 0.09 \\ 
  $W_{23}$ & 2 & 1 & 0.95 & 0.87 & 0.52 & 0.78 &  & 0.83 & 0.68 & 0.53 & 0.72 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0.77 & 0.43 & 0.55 & 0.5 &  & 0.26 & 0.1 & 0.49 & 0.42 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 1 & 0.83 & 0.56 & 0.34 & 0.56 &  & 0.43 & 0.22 & 0.54 & 0.86 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 1 & 0.64 & 0.22 & 0.2 & 0.22 &  & 0.09 & 0.03 & 0.25 & 0.51 \\ 
  $intercept$ & 2 & 2 & 0.93 & 0.7 & 0.53 & 0.62 &  & 0.5 & 0.03 & 0.77 & 0.6 \\ 
  $W_{11}$ & 2 & 2 & 0.75 & 0.37 & 0.09 & 0 &  & 0.24 & 0.07 & 0.89 & 0.01 \\ 
  $W_{21}$ & 2 & 2 & 0.96 & 0.84 & 0.04 & 0.19 &  & 0.73 & 0.31 & 0.03 & 0.22 \\ 
  $W_{22}$ & 2 & 2 & 0.94 & 0.78 & 0.05 & 0.21 &  & 0.63 & 0.19 & 0.08 & 0.28 \\ 
  $W_{23}$ & 2 & 2 & 0.95 & 0.85 & 0.4 & 0.24 &  & 0.82 & 0.68 & 0.4 & 0.45 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 2 & 0.83 & 0.52 & 0.32 & 0.37 &  & 0.37 & 0.06 & 0.17 & 0.6 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 2 & 0.85 & 0.61 & 0.05 & 0.52 &  & 0.5 & 0.3 & 0.35 & 0.86 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 2 & 0.67 & 0.26 & 0.47 & 0.09 &  & 0.19 & 0.09 & 0.63 & 0.58 \\ 
  $intercept$ & 2 & 3 & 0.93 & 0.72 & 0.87 & 0.51 &  & 0.52 & 0.05 & 0.87 & 0.79 \\ 
  $W_{11}$ & 2 & 3 & 0.81 & 0.45 & 0.5 & 0.99 &  & 0.33 & 0.07 & 0.42 & 0.95 \\ 
  $W_{21}$ & 2 & 3 & 0.95 & 0.79 & 0 & 0.52 &  & 0.64 & 0.24 & 0 & 0.06 \\ 
  $W_{22}$ & 2 & 3 & 0.98 & 0.9 & 0.12 & 0.26 &  & 0.83 & 0.52 & 0.17 & 0.55 \\ 
  $W_{23}$ & 2 & 3 & 0.86 & 0.57 & 0.05 & 0.21 &  & 0.43 & 0.16 & 0.07 & 0.47 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 3 & 0.81 & 0.45 & 0.9 & 0.65 &  & 0.32 & 0.05 & 0.55 & 0.79 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 3 & 0.93 & 0.78 & 0.25 & 0.61 &  & 0.69 & 0.42 & 0.33 & 0.89 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 3 & 0.79 & 0.43 & 0 & 0.29 &  & 0.26 & 0.09 & 0.02 & 0.65 \\ 
   \hline
   \multicolumn{12}{l}{\begin{minipage}[hs!]{1\textwidth}
   		\textit{Note}: See the note of Table \ref{tab: MCMCcon_ba_th}
   \end{minipage}	}
\end{tabular}
\end{table}


==> Tables/App_MCMC_tran_res_2_bf_th.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:43:52 2022
\begin{table}[h!]
\centering
\caption{MCMC diagnostic for the connectivity parameters before and after thinning} 
\label{tab: MCMCtran_ba_th}
\begin{tabular}{cccccccccccc}
  \hline \multirow{2}{3cm}{\centering Parameters} & \multirow{2}{1cm}{\centering $\ell$} & \multirow{2}{1cm}{\centering $q$}  & \multicolumn{4}{c}{Before thinning} & & \multicolumn{4}{c}{After thinning} \\ \cline{4-7} \cline{9-12}V1 & $\ell$ & $q$ & $AC1$ & $AC5$ & $GD$ & $HDS$ & V8 & $AC1$ & $AC5$ & $GD$ & $HDS$ \\ 
  \hline  \hline
$intercept$ & 1 & 1 & 0.61 & 0.12 & 0.02 & 0.21 &  & 0.02 & 0.01 & 0.05 & 0.61 \\ 
  $W_{11}$ & 1 & 1 & 0.82 & 0.54 & 0.03 & 0.31 &  & 0.44 & 0.1 & 0.04 & 0.16 \\ 
  $W_{12}$ & 1 & 1 & 0.9 & 0.72 & 0.6 & 0.43 &  & 0.63 & 0.29 & 0.69 & 0.61 \\ 
  $W_{13}$ & 1 & 1 & 0.94 & 0.88 & 0.02 & 0.14 &  & 0.83 & 0.6 & 0.02 & 0.18 \\ 
  $W_{21}$ & 1 & 1 & 0.62 & 0.16 & 0.06 & 0.41 &  & 0.05 & 0.02 & 0.04 & 0.23 \\ 
  $W_{22}$ & 1 & 1 & 0.64 & 0.15 & 0.02 & 0.38 &  & 0.03 & 0.04 & 0.13 & 0.66 \\ 
  $W_{23}$ & 1 & 1 & 0.5 & 0.37 & 0 & 0.24 &  & 0.31 & 0.18 & 0.01 & 0.38 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 1 & 0.76 & 0.41 & 0.21 & 0.42 &  & 0.25 & 0 & 0.47 & 0.4 \\ 
  $W_{11} \cdot W_{22}$ & 1 & 1 & 0.75 & 0.37 & 0.81 & 0.69 &  & 0.24 & 0.01 & 0.83 & 0.22 \\ 
  $W_{11} \cdot W_{23}$ & 1 & 1 & 0.41 & 0.22 & 0.16 & 0.49 &  & 0.09 & 0.04 & 0.11 & 0.77 \\ 
  $W_{12} \cdot W_{21}$ & 1 & 1 & 0.82 & 0.49 & 0.4 & 0.48 &  & 0.32 & 0.06 & 0.38 & 0.72 \\ 
  $W_{12} \cdot W_{22}$ & 1 & 1 & 0.87 & 0.58 & 0.63 & 0.3 &  & 0.4 & 0.03 & 0.98 & 0.68 \\ 
  $W_{12} \cdot W_{23}$ & 1 & 1 & 0.61 & 0.4 & 0.74 & 0.18 &  & 0.28 & 0.02 & 0.49 & 0.54 \\ 
  $W_{13} \cdot W_{21}$ & 1 & 1 & 0.36 & 0.02 & 0.69 & 0.63 &  & 0.02 & 0.02 & 0.49 & 0.78 \\ 
  $W_{13} \cdot W_{22}$ & 1 & 1 & 0.64 & 0.29 & 0.82 & 0.34 &  & 0.15 & 0.04 & 0.88 & 0.63 \\ 
  $W_{13} \cdot W_{23}$ & 1 & 1 & 0.56 & 0.31 & 0 & 0.09 &  & 0.21 & 0.05 & 0.01 & 0.19 \\ 
  $intercept$ & 1 & 2 & 0.87 & 0.55 & 0.24 & 0.49 &  & 0.37 & 0.07 & 0.28 & 0.47 \\ 
  $W_{11}$ & 1 & 2 & 0.88 & 0.62 & 0 & 0.1 &  & 0.47 & 0.09 & 0.01 & 0.12 \\ 
  $W_{12}$ & 1 & 2 & 0.9 & 0.67 & 0.78 & 0.87 &  & 0.55 & 0.26 & 0.72 & 0.97 \\ 
  $W_{13}$ & 1 & 2 & 0.84 & 0.65 & 0.45 & 0.25 &  & 0.56 & 0.28 & 0.88 & 0.29 \\ 
  $W_{21}$ & 1 & 2 & 0.81 & 0.42 & 0.1 & 0.21 &  & 0.25 & 0.02 & 0.24 & 0.82 \\ 
  $W_{22}$ & 1 & 2 & 0.89 & 0.62 & 0.58 & 0.12 &  & 0.48 & 0.1 & 0.42 & 0.08 \\ 
  $W_{23}$ & 1 & 2 & 0.56 & 0.42 & 0.81 & 0.17 &  & 0.32 & 0.15 & 0.49 & 0.07 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 2 & 0.8 & 0.42 & 0.26 & 0.62 &  & 0.23 & 0.01 & 0.05 & 0.24 \\ 
  $W_{11} \cdot W_{22}$ & 1 & 2 & 0.82 & 0.44 & 0.33 & 0.06 &  & 0.23 & -0.03 & 0.37 & 0.05 \\ 
  $W_{11} \cdot W_{23}$ & 1 & 2 & 0.38 & 0.18 & 0.16 & 0.07 &  & 0.1 & 0.02 & 0.75 & 0.49 \\ 
  $W_{12} \cdot W_{21}$ & 1 & 2 & 0.79 & 0.42 & 0.64 & 0.99 &  & 0.25 & 0.04 & 0.55 & 0.93 \\ 
  $W_{12} \cdot W_{22}$ & 1 & 2 & 0.83 & 0.51 & 0.19 & 0.16 &  & 0.35 & 0.07 & 0.17 & 0.08 \\ 
  $W_{12} \cdot W_{23}$ & 1 & 2 & 0.46 & 0.24 & 0.32 & 0.56 &  & 0.17 & 0.02 & 0.09 & 0.39 \\ 
  $W_{13} \cdot W_{21}$ & 1 & 2 & 0.56 & 0.25 & 0.46 & 0.61 &  & 0.17 & 0.03 & 0.43 & 0.5 \\ 
  $W_{13} \cdot W_{22}$ & 1 & 2 & 0.71 & 0.38 & 0.63 & 0.38 &  & 0.23 & 0.05 & 0.27 & 0.38 \\ 
  $W_{13} \cdot W_{23}$ & 1 & 2 & 0.51 & 0.26 & 0.29 & 0.07 &  & 0.2 & 0.06 & 0.6 & 0.16 \\ 
  $intercept$ & 1 & 3 & 0.95 & 0.8 & 0.03 & 0.21 &  & 0.67 & 0.2 & 0.02 & 0.15 \\ 
  $W_{11}$ & 1 & 3 & 0.97 & 0.9 & 0.03 & 0.18 &  & 0.83 & 0.52 & 0.05 & 0.09 \\ 
  $W_{12}$ & 1 & 3 & 0.94 & 0.77 & 0.01 & 0.43 &  & 0.63 & 0.2 & 0.01 & 0.07 \\ 
  $W_{13}$ & 1 & 3 & 0.84 & 0.67 & 0.32 & 0.11 &  & 0.56 & 0.29 & 0.46 & 0.09 \\ 
  $W_{21}$ & 1 & 3 & 0.88 & 0.6 & 0.49 & 0.44 &  & 0.45 & 0.08 & 0.25 & 0.31 \\ 
  $W_{22}$ & 1 & 3 & 0.89 & 0.64 & 0.83 & 0.99 &  & 0.48 & 0.1 & 0.83 & 0.98 \\ 
  $W_{23}$ & 1 & 3 & 0.64 & 0.45 & 0.25 & 0.15 &  & 0.34 & 0.16 & 0.16 & 0.32 \\ 
  $W_{11} \cdot W_{21}$ & 1 & 3 & 0.86 & 0.54 & 0.58 & 0.9 &  & 0.35 & 0.05 & 0.4 & 0.77 \\ 
  $W_{11} \cdot W_{22}$ & 1 & 3 & 0.88 & 0.58 & 0.57 & 0.96 &  & 0.4 & 0.01 & 0.56 & 0.95 \\ 
  $W_{11} \cdot W_{23}$ & 1 & 3 & 0.55 & 0.18 & 0.09 & 0.34 &  & 0.1 & -0.01 & 0.63 & 0.38 \\ 
  $W_{12} \cdot W_{21}$ & 1 & 3 & 0.85 & 0.53 & 0.45 & 0.9 &  & 0.35 & 0.07 & 0.8 & 0.9 \\ 
  $W_{12} \cdot W_{22}$ & 1 & 3 & 0.83 & 0.47 & 0.46 & 0.9 &  & 0.28 & 0.04 & 0.41 & 0.92 \\ 
  $W_{12} \cdot W_{23}$ & 1 & 3 & 0.62 & 0.36 & 0.42 & 0.14 &  & 0.23 & 0.08 & 0.96 & 0.34 \\ 
  $W_{13} \cdot W_{21}$ & 1 & 3 & 0.46 & 0.16 & 0.74 & 0.68 &  & 0.11 & -0.03 & 0.36 & 0.3 \\ 
  $W_{13} \cdot W_{22}$ & 1 & 3 & 0.7 & 0.36 & 0.73 & 0.75 &  & 0.22 & 0.06 & 0.88 & 0.76 \\ 
  $W_{13} \cdot W_{23}$ & 1 & 3 & 0.5 & 0.23 & 0.42 & 0.22 &  & 0.13 & 0.02 & 0.37 & 0.42 \\ 
  $intercept$ & 2 & 1 & 0.93 & 0.74 & 0.88 & 0.99 &  & 0.6 & 0.09 & 0.69 & 0.94 \\ 
  $W_{11}$ & 2 & 1 & 0.9 & 0.65 & 0.55 & 0.77 &  & 0.48 & 0.1 & 0.84 & 0.63 \\ 
  $W_{12}$ & 2 & 1 & 0.9 & 0.63 & 0.55 & 0.32 &  & 0.46 & 0.08 & 0.8 & 0.19 \\ 
  $W_{13}$ & 2 & 1 & 0.75 & 0.47 & 0.06 & 0.06 &  & 0.37 & 0.08 & 0.13 & 0.19 \\ 
  $W_{21}$ & 2 & 1 & 0.92 & 0.73 & 0.33 & 0.44 &  & 0.59 & 0.2 & 0.24 & 0.32 \\ 
  $W_{22}$ & 2 & 1 & 0.94 & 0.76 & 0.34 & 0.41 &  & 0.61 & 0.16 & 0.36 & 0.4 \\ 
  $W_{23}$ & 2 & 1 & 0.94 & 0.91 & 0.55 & 0.18 &  & 0.87 & 0.72 & 0.54 & 0.21 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 1 & 0.86 & 0.53 & 0.48 & 0.7 &  & 0.35 & 0.03 & 0.85 & 0.87 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 1 & 0.87 & 0.55 & 0.15 & 0.85 &  & 0.34 & 0.05 & 0.16 & 0.91 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 1 & 0.49 & 0.13 & 0.82 & 0.59 &  & 0.03 & 0.02 & 0.71 & 0.68 \\ 
  $W_{12} \cdot W_{21}$ & 2 & 1 & 0.82 & 0.44 & 0.04 & 0.18 &  & 0.29 & 0.04 & 0.01 & 0.08 \\ 
  $W_{12} \cdot W_{22}$ & 2 & 1 & 0.88 & 0.58 & 0.69 & 0.52 &  & 0.38 & 0.06 & 0.85 & 0.73 \\ 
  $W_{12} \cdot W_{23}$ & 2 & 1 & 0.58 & 0.38 & 0.63 & 0.38 &  & 0.24 & 0.06 & 0.28 & 0.07 \\ 
  $W_{13} \cdot W_{21}$ & 2 & 1 & 0.5 & 0.13 & 0.53 & 0.36 &  & 0.14 & 0 & 0.77 & 0.79 \\ 
  $W_{13} \cdot W_{22}$ & 2 & 1 & 0.77 & 0.47 & 0.87 & 0.81 &  & 0.29 & 0.07 & 0.77 & 0.82 \\ 
  $W_{13} \cdot W_{23}$ & 2 & 1 & 0.55 & 0.36 & 0.12 & 0.36 &  & 0.27 & 0.05 & 0.54 & 0.82 \\ 
  $intercept$ & 2 & 2 & 0.81 & 0.4 & 0.69 & 0.41 &  & 0.24 & 0.03 & 0.78 & 0.63 \\ 
  $W_{11}$ & 2 & 2 & 0.82 & 0.41 & 0.53 & 0.66 &  & 0.21 & -0.01 & 0.55 & 0.7 \\ 
  $W_{12}$ & 2 & 2 & 0.79 & 0.35 & 0.15 & 0.75 &  & 0.22 & 0.03 & 0.75 & 0.93 \\ 
  $W_{13}$ & 2 & 2 & 0.69 & 0.39 & 0.54 & 0.1 &  & 0.29 & 0.09 & 0.46 & 0.26 \\ 
  $W_{21}$ & 2 & 2 & 0.93 & 0.74 & 0.72 & 0.15 &  & 0.59 & 0.25 & 0.64 & 0.33 \\ 
  $W_{22}$ & 2 & 2 & 0.8 & 0.37 & 0.63 & 0.11 &  & 0.22 & 0.03 & 0.53 & 0.14 \\ 
  $W_{23}$ & 2 & 2 & 0.91 & 0.87 & 0.96 & 0.22 &  & 0.84 & 0.67 & 0.91 & 0.39 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 2 & 0.9 & 0.63 & 0.19 & 0.06 &  & 0.42 & 0.01 & 0.26 & 0.06 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 2 & 0.76 & 0.32 & 0.22 & 0.19 &  & 0.16 & -0.03 & 0.16 & 0.14 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 2 & 0.52 & 0.18 & 0.08 & 0.24 &  & 0.01 & -0.01 & 0.23 & 0.41 \\ 
  $W_{12} \cdot W_{21}$ & 2 & 2 & 0.87 & 0.56 & 0.68 & 0.17 &  & 0.38 & 0.08 & 0.71 & 0.26 \\ 
  $W_{12} \cdot W_{22}$ & 2 & 2 & 0.75 & 0.29 & 0.17 & 0.53 &  & 0.15 & 0.04 & 0.37 & 0.7 \\ 
  $W_{12} \cdot W_{23}$ & 2 & 2 & 0.63 & 0.47 & 0.03 & 0.32 &  & 0.38 & 0.17 & 0.09 & 0.56 \\ 
  $W_{13} \cdot W_{21}$ & 2 & 2 & 0.54 & 0.16 & 0.19 & 0.27 &  & 0.09 & 0.03 & 0.93 & 0.91 \\ 
  $W_{13} \cdot W_{22}$ & 2 & 2 & 0.77 & 0.48 & 0.37 & 0 &  & 0.37 & 0.13 & 0.31 & 0.11 \\ 
  $W_{13} \cdot W_{23}$ & 2 & 2 & 0.56 & 0.42 & 0.89 & 0.92 &  & 0.35 & 0.1 & 0.78 & 0.59 \\ 
  $intercept$ & 2 & 3 & 0.93 & 0.71 & 0.12 & 0.89 &  & 0.55 & 0.08 & 0.33 & 0.99 \\ 
  $W_{11}$ & 2 & 3 & 0.91 & 0.65 & 0.73 & 0.39 &  & 0.47 & 0.11 & 0.99 & 0.34 \\ 
  $W_{12}$ & 2 & 3 & 0.9 & 0.65 & 0.15 & 0.92 &  & 0.51 & 0.1 & 0.19 & 0.98 \\ 
  $W_{13}$ & 2 & 3 & 0.75 & 0.41 & 0.72 & 0.3 &  & 0.28 & 0.08 & 0.82 & 0.26 \\ 
  $W_{21}$ & 2 & 3 & 0.96 & 0.85 & 0.98 & 0.21 &  & 0.77 & 0.45 & 0.96 & 0.17 \\ 
  $W_{22}$ & 2 & 3 & 0.94 & 0.75 & 0.72 & 0.09 &  & 0.62 & 0.15 & 0.97 & 0.1 \\ 
  $W_{23}$ & 2 & 3 & 0.73 & 0.61 & 0.24 & 0.52 &  & 0.54 & 0.29 & 0.28 & 0.49 \\ 
  $W_{11} \cdot W_{21}$ & 2 & 3 & 0.87 & 0.57 & 0.06 & 0.26 &  & 0.4 & 0.08 & 0.24 & 0.33 \\ 
  $W_{11} \cdot W_{22}$ & 2 & 3 & 0.9 & 0.63 & 0.88 & 0.1 &  & 0.47 & 0.09 & 0.78 & 0.18 \\ 
  $W_{11} \cdot W_{23}$ & 2 & 3 & 0.51 & 0.21 & 0.63 & 0.45 &  & 0.08 & 0.01 & 0.46 & 0.82 \\ 
  $W_{12} \cdot W_{21}$ & 2 & 3 & 0.87 & 0.56 & 0.02 & 0.08 &  & 0.39 & 0.1 & 0.05 & 0.24 \\ 
  $W_{12} \cdot W_{22}$ & 2 & 3 & 0.86 & 0.51 & 0.08 & 0.09 &  & 0.32 & 0.07 & 0.38 & 0.24 \\ 
  $W_{12} \cdot W_{23}$ & 2 & 3 & 0.6 & 0.41 & 0.06 & 0.7 &  & 0.3 & 0.06 & 0.32 & 0.91 \\ 
  $W_{13} \cdot W_{21}$ & 2 & 3 & 0.52 & 0.09 & 0.64 & 0.49 &  & 0.04 & 0 & 0.98 & 0.73 \\ 
  $W_{13} \cdot W_{22}$ & 2 & 3 & 0.75 & 0.41 & 0.98 & 0.07 &  & 0.26 & 0.04 & 0.68 & 0.1 \\ 
  $W_{13} \cdot W_{23}$ & 2 & 3 & 0.57 & 0.37 & 0.37 & 0.1 &  & 0.27 & 0.11 & 0.21 & 0.2 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_rand_global_ini_map_res0.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:30:57 2022
\begin{table}[h!]
\centering
\caption{Global Adjusted Rand Index (Initialization and MAP)} 
\label{rand_global}
\begin{tabular}{ccc}
  \hline \\[-1.8ex] & L1 & L2 \\ 
  \hline \hline \\[-1.8ex]ARI & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_rand_global_ini_map_res1.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:33:58 2022
\begin{table}[h!]
\centering
\caption{Global Adjusted Rand Index (Initialization and MAP)} 
\label{rand_global}
\begin{tabular}{ccc}
  \hline \\[-1.8ex] & L1 & L2 \\ 
  \hline \hline \\[-1.8ex]ARI & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/App_rand_global_ini_map_res2.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Jun 22 21:38:03 2022
\begin{table}[h!]
\centering
\caption{Global Adjusted Rand Index (Initialization and MAP)} 
\label{rand_global}
\begin{tabular}{ccc}
  \hline \\[-1.8ex] & L1 & L2 \\ 
  \hline \hline \\[-1.8ex]ARI & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/Comparison_DSBM_M_GP.tex <==
% latex table generated in R 4.5.0 by xtable 1.8-4 package
% Fri Jul  4 10:16:59 2025
\begin{tabular}{cccccccc}
  \hline \multirow{2}{2cm}{\centering Target} & \multirow{2}{2cm}{\centering Measure} & \multirow{2}{2cm}{\centering Layer} 
                                      & \multicolumn{2}{c}{In-sample} & & \multicolumn{2}{c}{Out-of-sample} \\
                                      \cline{4-5} \cline{7-8} & & & DSBMM & BLDMN & & DSBMM & BLDMN \\ \hline \hline  \multirow{14}{2cm}{$D$} & \multirow{2}{2cm}{AUC} &   1 & -0.00 & 0.01 &  &  &  \\ 
   & &  2 & 0.00 & 0.00 &  & 0.03 & -0.03 \\ 
   \cline{2-8} &  \multirow{2}{2cm}{Corr} &  1 & 0.00 & -0.05 &  &  &  \\ 
   & &  2 & 0.08 & -0.03 &  & 0.68 & 0.52 \\ 
    \cline{2-8} & \multirow{2}{2cm}{CorrK ($\tau$)} &  1 & 0.00 & -0.12 &  &  &  \\ 
   & &  2 & 0.15 & -0.05 &  & 0.51 & 0.41 \\ 
   \cline{2-8} & \multirow{2}{2cm}{CorrSp ($\rho$)} &  1 & 0.00 & -0.05 &  &  &  \\ 
   & &  2 & 0.09 & -0.02 &  & 0.66 & 0.53 \\ 
   \cline{2-8} & \multirow{2}{2cm}{ECE} &  1 & 0.00 & 0.06 &  &  &  \\ 
   & &  2 & -0.10 & -0.02 &  & -0.18 & -0.10 \\ 
   \cline{2-8} & \multirow{2}{2cm}{Var} &  1 & 0.00 & 0.00 &  &  &  \\ 
   & &  2 & -0.00 & 0.01 &  &  &  \\ 
   \cline{2-8} & \multirow{2}{2cm}{SBias} &  1 & 0.00 & 0.01 &  &  &  \\ 
   & &  2 & -0.03 & -0.00 &  &  &  \\ 
   \cline{1-8}& & & & & & & \\\cline{1-8} \multirow{6}{2cm}{$Z$} & \multirow{2}{2cm}{AUC} &  1 & 0.00 &  &  &  &  \\ 
   & &  2 & 0.13 &  &  & 0.14 &  \\ 
   \cline{2-8} & \multirow{2}{2cm}{Bsc} &  1 & 0.00 &  &  &  &  \\ 
   & &  2 & -0.18 &  &  & -0.27 &  \\ 
   \cline{2-8} & \multirow{2}{2cm}{RandI} &  1 & 0.00 &  &  &  &  \\ 
   & &  2 & 0.14 &  &  & 0.08 &  \\ 
   \hline \end{tabular}


==> Tables/causBVAR.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Sun Oct 24 23:49:43 2021
\begin{table}[h!]
\centering
\caption{Proportion of experiments where the true causality structure has been estimated. The results refer to different model settings, sample sizes and BVAR specifications.} 
\label{tab:causBVAR}
\begin{tabular}{llrrrrrrrrrrrr}
  \hline
  \multirow{2}{*}{Cases} & \multirow{2}{*}{Sample Size} & \multicolumn{3}{c}{Panel VAR} & \multicolumn{3}{c}{Panel BVAR Pooled} & \multicolumn{3}{c}{Panel BVAR RE mCI} & \multicolumn{3}{c}{BVAR RE sCI} \\ &  & WNZ & WZ & UW & WNZ & WZ & UW & WNZ & WZ & UW & WNZ & WZ & UW \\ \hline \hline \multirow{2}{*}{No Causality} & Reference & 0.00 & 0.00 & 0.00 & 1.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
   & Larger T & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
   \multirow{2}{*}{Unidirectional} & Reference & 0.00 & 0.00 & 0.00 & 0.30 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
   & Larger T & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
   \multirow{2}{*}{Bidirectional} & Reference & 0.00 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.10 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 \\ 
   & Larger T & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/caustabcov.tex <==
% latex table generated in R 4.5.0 by xtable 1.8-4 package
% Mon May  5 09:12:16 2025
\begin{table}[h!]
\centering
\caption{\color{red} Proportion of simulated data sets where the true causality structure is successfully retrieved by model setting, sample size and prior.} 
\label{tab:propsynt}
\begin{tabular}{lll>{\color{red}}ll>{\color{red}}l}
  \hline
  \multirow{2}{*}{Model setting} & \multirow{2}{*}{Sample size} & \multirow{2}{*}{Normal Prior} & \multicolumn{3}{c}{Bayesian Group Lasso} \\ \cline{4-6}
                                    & & & Tight  & Medium & Diffuse  \\ \hline\hline \multirow{3}{*}{No causality}  & Reference & 0.25 & 1 & 0.96 & 1 \\ 
   & Larger T & 0.1 & 1 & 0.92 & 1 \\ 
   & Larger N & 0.27 & 0.98 & 0.88 & 0.98 \\ 
    \hline \multirow{3}{*}{Unidirectional} & Reference & 0.52 & 1 & 0.96 & 1 \\ 
   & Larger T & 0.46 & 0.98 & 0.92 & 0.94 \\ 
   & Larger N & 0.46 & 0.96 & 0.83 & 0.96 \\ 
    \hline \multirow{3}{*}{Bidirectional}  & Reference & 0.52 & 1 & 0.92 & 0.88 \\ 
   & Larger T & 0.31 & 0.96 & 0.88 & 0.88 \\ 
   & Larger N & 0.44 & 0.96 & 0.79 & 0.92 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/commupdt_lay1mod1.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Wed Oct  9 13:12:24 2024
\begin{tabular}{lp{3.75cm}p{3.75cm}}
  \hline
 & \multicolumn{1}{c}{1995} & \multicolumn{1}{c}{2017} \\ 
  \hline
1 & ARG, \textbf{\scriptsize AUS}, \textbf{\scriptsize AUT}, BGR, \textbf{\scriptsize BRA}, \textbf{\scriptsize CAN}, \textbf{\scriptsize CHE}, CHL, \textbf{\scriptsize CHN}, COL, CRI, CYP, CZE, \textbf{\scriptsize DEU}, DNK, EGY, \textbf{\scriptsize ESP}, FIN, \textbf{\scriptsize FRA}, \textbf{\scriptsize GBR}, GRC, \textbf{\scriptsize IDN}, IND, \textbf{\scriptsize IRL}, ISR, \textbf{\scriptsize ITA}, \textbf{\scriptsize JPN}, \textbf{\scriptsize KOR}, MAR, \textbf{\scriptsize MYS}, \textbf{\scriptsize NLD}, NOR, NZL, PAK, PER, \textbf{\scriptsize PHL}, POL, PRT, \textbf{\scriptsize RUS}, \textbf{\scriptsize SGP}, SVK, SVN, \textbf{\scriptsize SWE}, \textbf{\scriptsize THA}, TUN, TUR, \textbf{\scriptsize USA}. & ALB, \textbf{\scriptsize ARE}, ARG, \textbf{\scriptsize AUS}, AUT, BGD, BGR, BHR, BIH, BLR, \textbf{\scriptsize BRA}, \textbf{\scriptsize CAN}, \textbf{\scriptsize CHE}, CHL, \textbf{\scriptsize CHN}, CIV, COL, CRI, CYP, CZE, \textbf{\scriptsize DEU}, DNK, DOM, ECU, \textbf{\scriptsize ESP}, EST, FIN, \textbf{\scriptsize FRA}, \textbf{\scriptsize GBR}, GRC, HRV, HUN, \textbf{\scriptsize IDN}, \textbf{\scriptsize IND}, IRL, ISL, ISR, \textbf{\scriptsize ITA}, JOR, \textbf{\scriptsize JPN}, KEN, KHM, \textbf{\scriptsize KOR}, LBN, LKA, LTU, LVA, MAR, MDG, \textbf{\scriptsize MEX}, MLT, MUS, \textbf{\scriptsize MYS}, \textbf{\scriptsize NLD}, NOR, NZL, PAK, PER, PHL, \textbf{\scriptsize POL}, PRT, \textbf{\scriptsize RUS}, \textbf{\scriptsize SAU}, \textbf{\scriptsize SGP}, SVK, SVN, SWE, \textbf{\scriptsize THA}, TUN, TUR, UKR, URY, \textbf{\scriptsize USA}, \textbf{\scriptsize VNM}. \\ 
  2 & AGO, ALB, ARE, ARM, AZE, BDI, BEN, BFA, BGD, BHR, BHS, BIH, BLR, BLZ, BOL, BRB, BRN, CAF, CIV, CMR, COD, COG, COM, CPV, CUB, DMA, DOM, DZA, ECU, EST, ETH, FJI, GAB, GEO, GHA, GIN, GMB, GNB, GNQ, GRD, GRL, GTM, GUY, HND, HRV, HTI, HUN, IRN, IRQ, ISL, JAM, JOR, KAZ, KEN, KGZ, KHM, KNA, KWT, LAO, LBN, LCA, LKA, LTU, LVA, MDA, MDG, MDV, \textbf{\scriptsize MEX}, MKD, MLI, MLT, MMR, MNG, MOZ, MRT, MUS, MWI, NER, NGA, NIC, NPL, OMN, PAN, PNG, PRY, RWA, \textbf{\scriptsize SAU}, SDN, SEN, SLB, SLE, SLV, SUR, SYC, TCD, TGO, TJK, TKM, TON, TTO, TZA, UGA, UKR, URY, UZB, VCT, VNM, VUT, WSM, YEM, ZMB, ZWE. & AGO, ARM, AZE, BDI, BEN, BFA, BHS, BLZ, BOL, BRB, BRN, CAF, CMR, COD, COG, COM, CPV, CUB, DMA, DZA, EGY, ETH, FJI, GAB, GEO, GHA, GIN, GMB, GNB, GNQ, GRD, GRL, GTM, GUY, HND, HTI, IRN, IRQ, JAM, KAZ, KGZ, KNA, KWT, LAO, LCA, MDA, MDV, MKD, MLI, MMR, MNG, MOZ, MRT, MWI, NER, NGA, NIC, NPL, OMN, PAN, PNG, PRY, RWA, SDN, SEN, SLB, SLE, SLV, SUR, SYC, TCD, TGO, TJK, TKM, TON, TTO, TZA, UGA, UZB, VCT, VUT, WSM, YEM, ZMB, ZWE. \\ 
   \hline
\end{tabular}


==> Tables/commupdt_lay2mod1.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Wed Oct  9 13:12:24 2024
\begin{tabular}{lp{3.75cm}p{3.75cm}}
  \hline
 & \multicolumn{1}{c}{1995} & \multicolumn{1}{c}{2017} \\ 
  \hline
1 & ARE, ARG, ARM, AZE, BGR, BHR, BHS, BLR, BLZ, BOL, BRA, BRB, CHL, CHN, COL, CRI, CYP, DMA, DZA, ECU, EGY, EST, GEO, GRD, GRL, GTM, GUY, HND, IRQ, \textbf{\scriptsize ISL}, ISR, JAM, KAZ, KGZ, KNA, KWT, LBN, LCA, LTU, LVA, MDA, MEX, MKD, MLT, NIC, OMN, PAN, PER, PRY, RUS, SAU, SLV, SUR, \textbf{\scriptsize SVK}, SVN, TJK, TKM, TTO, TUN, TUR, UKR, URY, UZB, VCT, YEM. & ALB, ARE, ARG, AZE, BHR, BHS, BIH, BLZ, BOL, BRA, BRB, COL, CRI, CUB, DMA, DOM, DZA, ECU, FJI, GEO, GRD, GRL, GTM, GUY, HND, HTI, IRN, IRQ, ISR, JAM, JOR, KNA, KWT, LBN, LCA, MAR, MDA, MEX, MKD, NIC, OMN, PAN, PER, PNG, PRY, SAU, SLV, SUR, TJK, TKM, TTO, TUN, UKR, URY, UZB, VCT, YEM. \\ 
  2 & ALB, BEN, BFA, BGD, BIH, BRN, CAF, CIV, CMR, COG, CPV, CUB, DOM, FJI, GAB, GHA, GIN, GMB, GNB, GNQ, HRV, HTI, IDN, IND, IRN, JOR, KHM, KOR, LAO, LKA, MAR, MDV, MLI, MMR, MNG, MRT, MYS, NER, NGA, NPL, PAK, PHL, PNG, SEN, SGP, SLB, SLE, TCD, TGO, THA, TON, VNM, VUT, WSM. & BEN, BFA, BGD, BRN, CAF, CHN, CIV, CMR, COG, CPV, GAB, GHA, GIN, GMB, GNB, GNQ, IDN, IND, KHM, LAO, LKA, MDV, MLI, MMR, MNG, MRT, MYS, NER, NGA, NPL, PAK, PHL, SEN, SGP, SLB, SLE, TCD, TGO, THA, TON, VNM, VUT, WSM. \\ 
  3 & \textbf{\scriptsize AUS}, \textbf{\scriptsize AUT}, \textbf{\scriptsize CAN}, \textbf{\scriptsize CHE}, \textbf{\scriptsize CZE}, \textbf{\scriptsize DEU}, \textbf{\scriptsize DNK}, \textbf{\scriptsize ESP}, \textbf{\scriptsize FIN}, \textbf{\scriptsize FRA}, \textbf{\scriptsize GBR}, \textbf{\scriptsize GRC}, \textbf{\scriptsize HUN}, \textbf{\scriptsize IRL}, \textbf{\scriptsize ITA}, \textbf{\scriptsize JPN}, \textbf{\scriptsize NLD}, \textbf{\scriptsize NOR}, \textbf{\scriptsize NZL}, \textbf{\scriptsize POL}, \textbf{\scriptsize PRT}, \textbf{\scriptsize SWE}, \textbf{\scriptsize USA}. & ARM, AUS, \textbf{\scriptsize AUT}, \textbf{\scriptsize BGR}, BLR, CAN, CHE, CHL, \textbf{\scriptsize CYP}, \textbf{\scriptsize CZE}, \textbf{\scriptsize DEU}, \textbf{\scriptsize DNK}, \textbf{\scriptsize ESP}, \textbf{\scriptsize EST}, \textbf{\scriptsize FIN}, \textbf{\scriptsize FRA}, \textbf{\scriptsize GBR}, \textbf{\scriptsize GRC}, HRV, \textbf{\scriptsize HUN}, \textbf{\scriptsize IRL}, ISL, \textbf{\scriptsize ITA}, JPN, KAZ, KGZ, KOR, \textbf{\scriptsize LTU}, \textbf{\scriptsize LVA}, \textbf{\scriptsize MLT}, \textbf{\scriptsize NLD}, NOR, NZL, \textbf{\scriptsize POL}, \textbf{\scriptsize PRT}, RUS, \textbf{\scriptsize SVK}, \textbf{\scriptsize SVN}, \textbf{\scriptsize SWE}, \textbf{\scriptsize TUR}, USA. \\ 
  4 & AGO, BDI, COD, COM, ETH, KEN, MDG, MOZ, MUS, MWI, RWA, SDN, SYC, TZA, UGA, ZMB, ZWE. & AGO, BDI, COD, COM, EGY, ETH, KEN, MDG, MOZ, MUS, MWI, RWA, SDN, SYC, TZA, UGA, ZMB, ZWE. \\ 
   \hline
\end{tabular}


==> Tables/corr2000.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:33 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2000} 
\label{corr2000}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.13 & 0.26 \\ 
  FDI & 0.13 & 1.00 & 0.26 \\ 
  Trade & 0.26 & 0.26 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2001.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:33 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2001} 
\label{corr2001}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.02 & 0.32 \\ 
  FDI & 0.02 & 1.00 & 0.30 \\ 
  Trade & 0.32 & 0.30 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2002.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:33 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2002} 
\label{corr2002}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.02 & 0.27 \\ 
  FDI & 0.02 & 1.00 & 0.36 \\ 
  Trade & 0.27 & 0.36 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2003.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:33 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2003} 
\label{corr2003}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.09 & 0.33 \\ 
  FDI & 0.09 & 1.00 & 0.07 \\ 
  Trade & 0.33 & 0.07 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2004.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:33 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2004} 
\label{corr2004}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.06 & 0.33 \\ 
  FDI & 0.06 & 1.00 & 0.30 \\ 
  Trade & 0.33 & 0.30 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2005.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:33 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2005} 
\label{corr2005}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & -0.01 & 0.20 \\ 
  FDI & -0.01 & 1.00 & 0.19 \\ 
  Trade & 0.20 & 0.19 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2006.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:33 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2006} 
\label{corr2006}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.05 & 0.32 \\ 
  FDI & 0.05 & 1.00 & 0.10 \\ 
  Trade & 0.32 & 0.10 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2007.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2007} 
\label{corr2007}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & -0.08 & 0.14 \\ 
  FDI & -0.08 & 1.00 & 0.41 \\ 
  Trade & 0.14 & 0.41 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2008.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2008} 
\label{corr2008}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.07 & 0.33 \\ 
  FDI & 0.07 & 1.00 & 0.20 \\ 
  Trade & 0.33 & 0.20 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2009.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2009} 
\label{corr2009}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.03 & 0.41 \\ 
  FDI & 0.03 & 1.00 & 0.10 \\ 
  Trade & 0.41 & 0.10 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2010.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2010} 
\label{corr2010}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.07 & 0.57 \\ 
  FDI & 0.07 & 1.00 & 0.24 \\ 
  Trade & 0.57 & 0.24 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2011.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2011} 
\label{corr2011}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.02 & 0.24 \\ 
  FDI & 0.02 & 1.00 & 0.21 \\ 
  Trade & 0.24 & 0.21 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2012.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2012} 
\label{corr2012}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & -0.01 & 0.24 \\ 
  FDI & -0.01 & 1.00 & 0.18 \\ 
  Trade & 0.24 & 0.18 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2013.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2013} 
\label{corr2013}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & 0.02 & 0.29 \\ 
  FDI & 0.02 & 1.00 & 0.27 \\ 
  Trade & 0.29 & 0.27 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2014.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2014} 
\label{corr2014}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & -0.09 & 0.29 \\ 
  FDI & -0.09 & 1.00 & 0.19 \\ 
  Trade & 0.29 & 0.19 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/corr2015.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:34 2020
\begin{table}[!h]
\centering
\caption{Correlation Matrix 2015} 
\label{corr2015}
\begin{tabular}{rrrr}
  \hline \\[-1.8ex] & Migration & FDI & Trade \\ 
  \hline \hline \\[-1.8ex]Migration & 1.00 & -0.09 & 0.32 \\ 
  FDI & -0.09 & 1.00 & 0.32 \\ 
  Trade & 0.32 & 0.32 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/country_list.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Sun Apr 16 13:00:21 2023
\begin{table}[htp!]
\centering
\caption{List of countries included in the multiplex FTAs-Trade Flows} 
\label{tab:list}
\begin{tabular}{cccc}
  \hline
  \hline
Angola & Denmark & Kenya & Poland \\ 
  Albania & Dominican Republic & Kyrgyzstan & Portugal \\ 
  United Arab Emirates & Algeria & Cambodia & Paraguay \\ 
  Argentina & Ecuador & St. Kitts -- Nevis & Russia \\ 
  Armenia & Egypt & South Korea & Rwanda \\ 
  Australia & Spain & Kuwait & Saudi Arabia \\ 
  Austria & Estonia & Laos & Sudan \\ 
  Azerbaijan & Ethiopia & Lebanon & Senegal \\ 
  Burundi & Finland & St. Lucia & Singapore \\ 
  Benin & Fiji & Sri Lanka & Solomon Islands \\ 
  Burkina Faso & France & Lithuania & Sierra Leone \\ 
  Bangladesh & Gabon & Latvia & El Salvador \\ 
  Bulgaria & United Kingdom & Morocco & Suriname \\ 
  Bahrain & Georgia & Moldova & Slovakia \\ 
  Bahamas & Ghana & Madagascar & Slovenia \\ 
  Bosnia -- Herzegovina & Guinea & Maldives & Sweden \\ 
  Belarus & Gambia & Mexico & Seychelles \\ 
  Belize & Guinea--Bissau & North Macedonia & Chad \\ 
  Bolivia & Equatorial Guinea & Mali & Togo \\ 
  Brazil & Greece & Malta & Thailand \\ 
  Barbados & Grenada & Myanmar (Burma) & Tajikistan \\ 
  Brunei & Greenland & Mongolia & Turkmenistan \\ 
  Central African Republic & Guatemala & Mozambique & Tonga \\ 
  Canada & Guyana & Mauritania & Trinidad -- Tobago \\ 
  Switzerland & Honduras & Mauritius & Tunisia \\ 
  Chile & Croatia & Malawi & Turkey \\ 
  China & Haiti & Malaysia & Tanzania \\ 
  Cote d'Ivoire & Hungary & Niger & Uganda \\ 
  Cameroon & Indonesia & Nigeria & Ukraine \\ 
  Congo -- Kinshasa & India & Nicaragua & Uruguay \\ 
  Congo -- Brazzaville & Ireland & Netherlands & United States \\ 
  Colombia & Iran & Norway & Uzbekistan \\ 
  Comoros & Iraq & Nepal & St. Vincent -- Grenadines \\ 
  Cape Verde & Iceland & New Zealand & Vietnam \\ 
  Costa Rica & Israel & Oman & Vanuatu \\ 
  Cuba & Italy & Pakistan & Samoa \\ 
  Cyprus & Jamaica & Panama & Yemen \\ 
  Czechia & Jordan & Peru & Zambia \\ 
  Germany & Japan & Philippines & Zimbabwe \\ 
  Dominica & Kazakhstan & Papua New Guinea &  \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_global_case_2.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Tue Apr 20 16:18:45 2021
\begin{table}[h!]
\centering
\caption{Global Adjusted Rand Index} 
\label{rand_global}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]ARI & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_global_case_3.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu Apr 22 00:34:39 2021
\begin{table}[h!]
\centering
\caption{Global Adjusted Rand Index} 
\label{rand_global}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]ARI & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_global_case_4.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Wed Apr 21 23:50:26 2021
\begin{table}[h!]
\centering
\caption{Global Adjusted Rand Index} 
\label{rand_global}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]ARI & 1.00 & 0.93 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_miss.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:34:58 2020
\begin{table}[!h]
\centering
\caption{Adjusted Rand Index, Setting missing values to zero vs Modelling Sampling} 
\label{rand_miss}
\begin{tabular}{llr}
  \hline \\[-1.8ex]Network & Year & Index \\ 
  \hline \hline \\[-1.8ex]\multirow{17}{*}{Migration} & 2000 & 0.44 \\ 
   & 2001 & 0.21 \\ 
   & 2002 & 0.25 \\ 
   & 2003 & 0.23 \\ 
   & 2004 & 0.20 \\ 
   & 2005 & 0.30 \\ 
   & 2006 & 0.38 \\ 
   & 2007 & 0.40 \\ 
   & 2008 & 0.58 \\ 
   & 2009 & 0.50 \\ 
   & 2010 & 0.36 \\ 
   & 2011 & 0.37 \\ 
   & 2012 & 0.54 \\ 
   & 2013 & 0.54 \\ 
   & 2014 & 0.58 \\ 
   & 2015 & 0.35 \\ 
   & 2016 & 0.47 \\ 
  \cline{2-3} \multirow{17}{*}{FDI} & 2000 & 0.13 \\ 
   & 2001 & 0.77 \\ 
   & 2002 & 0.44 \\ 
   & 2003 & 0.88 \\ 
   & 2004 & 0.78 \\ 
   & 2005 & 0.43 \\ 
   & 2006 & 0.78 \\ 
   & 2007 & 1.00 \\ 
   & 2008 & 0.78 \\ 
   & 2009 & 1.00 \\ 
   & 2010 & 1.00 \\ 
   & 2011 & 0.68 \\ 
   & 2012 & 0.89 \\ 
   & 2013 & 0.59 \\ 
   & 2014 & 0.50 \\ 
   & 2015 & 1.00 \\ 
   & 2016 & 1.00 \\ 
  \cline{2-3}  \multirow{17}{*}{Trade} & 2000 & 0.56 \\ 
   & 2001 & 1.00 \\ 
   & 2002 & 1.00 \\ 
   & 2003 & 0.91 \\ 
   & 2004 & 1.00 \\ 
   & 2005 & 1.00 \\ 
   & 2006 & 1.00 \\ 
   & 2007 & 1.00 \\ 
   & 2008 & 1.00 \\ 
   & 2009 & 1.00 \\ 
   & 2010 & 1.00 \\ 
   & 2011 & 1.00 \\ 
   & 2012 & 1.00 \\ 
   & 2013 & 1.00 \\ 
   & 2014 & 1.00 \\ 
   & 2015 & 1.00 \\ 
   & 2016 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_mnorm.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Thu May 28 00:02:33 2020
\begin{table}[!h]
\centering
\caption{Adjusted Rand Index comparing SBM MNormal for between years} 
\label{rand_mnorm}
\begin{tabular}{rrrrrrrrrrrrrrrrrr}
  \hline \\[-1.8ex] & 2000 & 2001 & 2002 & 2003 & 2004 & 2005 & 2006 & 2007 & 2008 & 2009 & 2010 & 2011 & 2012 & 2013 & 2014 & 2015 & 2016 \\ 
  \hline \hline \\[-1.8ex]2000 & 1.00 & 0.90 & 0.73 & 0.80 & 0.65 & 0.64 & 0.52 & 0.60 & 0.52 & 0.58 & 0.71 & 0.72 & 0.81 & 0.55 & 0.59 & 0.49 & 0.65 \\ 
  2001 & 0.90 & 1.00 & 0.66 & 0.72 & 0.57 & 0.56 & 0.45 & 0.53 & 0.57 & 0.51 & 0.63 & 0.64 & 0.72 & 0.47 & 0.64 & 0.41 & 0.73 \\ 
  2002 & 0.73 & 0.66 & 1.00 & 0.73 & 0.74 & 0.73 & 0.76 & 0.83 & 0.58 & 0.66 & 0.63 & 0.79 & 0.72 & 0.38 & 0.63 & 0.33 & 0.46 \\ 
  2003 & 0.80 & 0.72 & 0.73 & 1.00 & 0.64 & 0.63 & 0.50 & 0.58 & 0.50 & 0.56 & 0.70 & 0.72 & 0.80 & 0.52 & 0.57 & 0.46 & 0.48 \\ 
  2004 & 0.65 & 0.57 & 0.74 & 0.64 & 1.00 & 0.81 & 0.67 & 0.60 & 0.67 & 0.76 & 0.57 & 0.74 & 0.65 & 0.29 & 0.58 & 0.24 & 0.37 \\ 
  2005 & 0.64 & 0.56 & 0.73 & 0.63 & 0.81 & 1.00 & 0.80 & 0.73 & 0.79 & 0.88 & 0.72 & 0.89 & 0.82 & 0.38 & 0.59 & 0.32 & 0.51 \\ 
  2006 & 0.52 & 0.45 & 0.76 & 0.50 & 0.67 & 0.80 & 1.00 & 0.92 & 0.80 & 0.89 & 0.56 & 0.73 & 0.65 & 0.45 & 0.58 & 0.39 & 0.54 \\ 
  2007 & 0.60 & 0.53 & 0.83 & 0.58 & 0.60 & 0.73 & 0.92 & 1.00 & 0.73 & 0.82 & 0.64 & 0.80 & 0.73 & 0.54 & 0.66 & 0.49 & 0.61 \\ 
  2008 & 0.52 & 0.57 & 0.58 & 0.50 & 0.67 & 0.79 & 0.80 & 0.73 & 1.00 & 0.90 & 0.56 & 0.72 & 0.64 & 0.46 & 0.74 & 0.41 & 0.65 \\ 
  2009 & 0.58 & 0.51 & 0.66 & 0.56 & 0.76 & 0.88 & 0.89 & 0.82 & 0.90 & 1.00 & 0.63 & 0.81 & 0.72 & 0.51 & 0.66 & 0.45 & 0.59 \\ 
  2010 & 0.71 & 0.63 & 0.63 & 0.70 & 0.57 & 0.72 & 0.56 & 0.64 & 0.56 & 0.63 & 1.00 & 0.80 & 0.89 & 0.43 & 0.52 & 0.37 & 0.55 \\ 
  2011 & 0.72 & 0.64 & 0.79 & 0.72 & 0.74 & 0.89 & 0.73 & 0.80 & 0.72 & 0.81 & 0.80 & 1.00 & 0.89 & 0.48 & 0.66 & 0.43 & 0.57 \\ 
  2012 & 0.81 & 0.72 & 0.72 & 0.80 & 0.65 & 0.82 & 0.65 & 0.73 & 0.64 & 0.72 & 0.89 & 0.89 & 1.00 & 0.55 & 0.59 & 0.48 & 0.65 \\ 
  2013 & 0.55 & 0.47 & 0.38 & 0.52 & 0.29 & 0.38 & 0.45 & 0.54 & 0.46 & 0.51 & 0.43 & 0.48 & 0.55 & 1.00 & 0.45 & 0.90 & 0.71 \\ 
  2014 & 0.59 & 0.64 & 0.63 & 0.57 & 0.58 & 0.59 & 0.58 & 0.66 & 0.74 & 0.66 & 0.52 & 0.66 & 0.59 & 0.45 & 1.00 & 0.52 & 0.61 \\ 
  2015 & 0.49 & 0.41 & 0.33 & 0.46 & 0.24 & 0.32 & 0.39 & 0.49 & 0.41 & 0.45 & 0.37 & 0.43 & 0.48 & 0.90 & 0.52 & 1.00 & 0.64 \\ 
  2016 & 0.65 & 0.73 & 0.46 & 0.48 & 0.37 & 0.51 & 0.54 & 0.61 & 0.65 & 0.59 & 0.55 & 0.57 & 0.65 & 0.71 & 0.61 & 0.64 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_nodes_case_2.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Tue Apr 20 16:18:44 2021
\begin{table}[h!]
\centering
\caption{Adjusted Rand Index across nodes} 
\label{rand_nodes}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]1 &  & 1.00 &  \\ 
  2 & 1.00 & 1.00 &  \\ 
  3 & 1.00 & 1.00 &  \\ 
  4 & 1.00 &  &  \\ 
  5 & 1.00 & 1.00 &  \\ 
  6 &  & 1.00 &  \\ 
  7 & 1.00 & 1.00 & 1.00 \\ 
  8 &  & 1.00 &  \\ 
  9 & 1.00 & 1.00 &  \\ 
  10 &  & 1.00 &  \\ 
  11 &  & 1.00 &  \\ 
  12 & 1.00 & 1.00 &  \\ 
  13 & 1.00 & 1.00 &  \\ 
  14 & 1.00 & 1.00 &  \\ 
  15 &  & 1.00 &  \\ 
  16 & 1.00 & 1.00 &  \\ 
  17 & 1.00 & 1.00 &  \\ 
  18 & 1.00 & 1.00 &  \\ 
  19 & 1.00 & 1.00 & 1.00 \\ 
  20 & 1.00 & 1.00 &  \\ 
  21 & 1.00 & 1.00 &  \\ 
  22 & 1.00 & 1.00 &  \\ 
  23 &  &  &  \\ 
  24 &  & 1.00 &  \\ 
  25 & 1.00 & 1.00 &  \\ 
  26 & 1.00 & 1.00 &  \\ 
  27 & 1.00 & 1.00 &  \\ 
  28 & 1.00 & 1.00 & 1.00 \\ 
  29 & 1.00 & 1.00 &  \\ 
  30 & 1.00 & 1.00 &  \\ 
  31 & 1.00 & 1.00 &  \\ 
  32 & 1.00 & 1.00 & 1.00 \\ 
  33 & 1.00 & 1.00 &  \\ 
  34 & 1.00 & 1.00 &  \\ 
  35 & 1.00 &  &  \\ 
  36 & 1.00 &  &  \\ 
  37 & 1.00 &  &  \\ 
  38 &  &  &  \\ 
  39 & 1.00 &  &  \\ 
  40 & 1.00 & 1.00 &  \\ 
  41 & 1.00 & 1.00 &  \\ 
  42 & 1.00 & 1.00 &  \\ 
  43 & 1.00 & 1.00 & 1.00 \\ 
  44 &  & 1.00 & 1.00 \\ 
  45 & 1.00 &  &  \\ 
  46 & 1.00 & 1.00 &  \\ 
  47 & 1.00 & 1.00 &  \\ 
  48 &  & 1.00 &  \\ 
  49 & 1.00 &  &  \\ 
  50 & 1.00 & 1.00 &  \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_nodes_case_3.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu Apr 22 00:34:39 2021
\begin{table}[h!]
\centering
\caption{Adjusted Rand Index across nodes} 
\label{rand_nodes}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]1 & 1.00 & 1.00 & 1.00 \\ 
  2 & 1.00 & 1.00 & 1.00 \\ 
  3 & 1.00 &  & 1.00 \\ 
  4 & 1.00 & 1.00 &  \\ 
  5 & 1.00 & 1.00 & 1.00 \\ 
  6 &  & 1.00 &  \\ 
  7 & 1.00 & 1.00 & 1.00 \\ 
  8 & 1.00 & 1.00 & 1.00 \\ 
  9 & 1.00 &  &  \\ 
  10 & 1.00 & 1.00 & 1.00 \\ 
  11 & 1.00 & 1.00 & 1.00 \\ 
  12 & 1.00 & 1.00 &  \\ 
  13 & 1.00 & 1.00 & 1.00 \\ 
  14 & 1.00 & 1.00 & 1.00 \\ 
  15 &  &  & 1.00 \\ 
  16 & 1.00 &  & 1.00 \\ 
  17 & 1.00 & 1.00 & 1.00 \\ 
  18 & 1.00 & 1.00 & 1.00 \\ 
  19 & 1.00 & 1.00 & 1.00 \\ 
  20 & 1.00 & 1.00 & 1.00 \\ 
  21 & 1.00 & 1.00 & 1.00 \\ 
  22 & 1.00 & 1.00 & 1.00 \\ 
  23 & 1.00 & 1.00 & 1.00 \\ 
  24 &  & 1.00 & 1.00 \\ 
  25 & 1.00 & 1.00 & 1.00 \\ 
  26 &  &  & 1.00 \\ 
  27 & 1.00 & 1.00 &  \\ 
  28 & 1.00 & 1.00 & 1.00 \\ 
  29 & 1.00 & 1.00 & 1.00 \\ 
  30 & 1.00 & 1.00 & 1.00 \\ 
  31 & 1.00 & 1.00 & 1.00 \\ 
  32 & 1.00 & 1.00 & 1.00 \\ 
  33 & 1.00 & 1.00 & 1.00 \\ 
  34 &  & 1.00 & 1.00 \\ 
  35 & 1.00 & 1.00 & 1.00 \\ 
  36 & 1.00 &  & 1.00 \\ 
  37 & 1.00 & 1.00 & 1.00 \\ 
  38 &  &  &  \\ 
  39 & 1.00 & 1.00 & 1.00 \\ 
  40 & 1.00 & 1.00 & 1.00 \\ 
  41 & 1.00 & 1.00 & 1.00 \\ 
  42 & 1.00 & 1.00 &  \\ 
  43 & 1.00 & 1.00 & 1.00 \\ 
  44 & 1.00 & 1.00 & 1.00 \\ 
  45 & 1.00 &  & 1.00 \\ 
  46 & 1.00 & 1.00 & 1.00 \\ 
  47 & 1.00 & 1.00 & 1.00 \\ 
  48 & 1.00 & 1.00 & 1.00 \\ 
  49 & 1.00 & 1.00 & 1.00 \\ 
  50 & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_nodes_case_4.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Wed Apr 21 23:50:26 2021
\begin{table}[h!]
\centering
\caption{Adjusted Rand Index across nodes} 
\label{rand_nodes}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]1 & 1.00 & 0.87 & 1.00 \\ 
  2 & 1.00 & 0.88 & 1.00 \\ 
  3 & 1.00 & 1.00 & 1.00 \\ 
  4 & 1.00 & 0.88 & 1.00 \\ 
  5 & 1.00 & 0.87 & 1.00 \\ 
  6 & 1.00 & 0.96 & 1.00 \\ 
  7 & 1.00 & 1.00 & 1.00 \\ 
  8 & 1.00 & 0.87 & 1.00 \\ 
  9 & 1.00 & 0.88 & 1.00 \\ 
  10 & 1.00 & 1.00 & 1.00 \\ 
  11 & 1.00 & 0.87 & 1.00 \\ 
  12 & 1.00 & 0.87 & 1.00 \\ 
  13 & 1.00 & 0.89 & 1.00 \\ 
  14 & 1.00 & 0.87 & 1.00 \\ 
  15 & 1.00 & 1.00 & 1.00 \\ 
  16 & 1.00 & 0.88 & 1.00 \\ 
  17 & 1.00 & 1.00 & 1.00 \\ 
  18 & 1.00 & 1.00 & 1.00 \\ 
  19 & 1.00 & 0.87 & 1.00 \\ 
  20 & 1.00 & 0.87 & 1.00 \\ 
  21 & 1.00 & 1.00 & 1.00 \\ 
  22 & 1.00 & 1.00 & 1.00 \\ 
  23 & 1.00 & 0.87 & 1.00 \\ 
  24 & 1.00 & 1.00 & 1.00 \\ 
  25 & 1.00 & 1.00 & 1.00 \\ 
  26 & 1.00 & 1.00 & 1.00 \\ 
  27 & 1.00 & 0.88 & 1.00 \\ 
  28 & 1.00 & 1.00 & 1.00 \\ 
  29 & 1.00 & 1.00 & 1.00 \\ 
  30 & 1.00 & 0.88 & 1.00 \\ 
  31 & 1.00 & 0.87 & 1.00 \\ 
  32 & 1.00 & 1.00 & 1.00 \\ 
  33 & 1.00 & 0.92 & 1.00 \\ 
  34 & 1.00 & 0.94 & 1.00 \\ 
  35 & 1.00 & 1.00 & 1.00 \\ 
  36 & 1.00 & 1.00 & 1.00 \\ 
  37 & 1.00 & 0.87 & 1.00 \\ 
  38 & 1.00 & 1.00 & 1.00 \\ 
  39 & 1.00 & 0.87 & 1.00 \\ 
  40 & 1.00 & 1.00 & 1.00 \\ 
  41 & 1.00 & 1.00 & 1.00 \\ 
  42 & 1.00 & 1.00 & 1.00 \\ 
  43 & 1.00 & 0.90 & 1.00 \\ 
  44 & 1.00 & 0.95 & 1.00 \\ 
  45 & 1.00 & 1.00 & 1.00 \\ 
  46 & 1.00 & 1.00 & 1.00 \\ 
  47 & 1.00 & 1.00 & 1.00 \\ 
  48 & 1.00 & 1.00 & 1.00 \\ 
  49 & 1.00 & 0.97 & 1.00 \\ 
  50 & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_time_case_2.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Tue Apr 20 16:18:45 2021
\begin{table}[h!]
\centering
\caption{Adjusted Rand Index across time} 
\label{rand_time}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]1 & 1.00 & 1.00 & 1.00 \\ 
  2 & 1.00 & 1.00 & 1.00 \\ 
  3 & 1.00 & 1.00 & 1.00 \\ 
  4 & 1.00 & 1.00 & 1.00 \\ 
  5 & 1.00 & 1.00 & 1.00 \\ 
  6 & 1.00 & 1.00 & 1.00 \\ 
  7 & 1.00 & 1.00 & 1.00 \\ 
  8 & 1.00 & 1.00 & 1.00 \\ 
  9 & 1.00 & 1.00 & 1.00 \\ 
  10 & 1.00 & 1.00 & 1.00 \\ 
  11 & 1.00 & 1.00 & 1.00 \\ 
  12 & 1.00 & 1.00 & 1.00 \\ 
  13 & 1.00 & 1.00 & 1.00 \\ 
  14 & 1.00 & 1.00 & 1.00 \\ 
  15 & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_time_case_3.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu Apr 22 00:34:39 2021
\begin{table}[h!]
\centering
\caption{Adjusted Rand Index across time} 
\label{rand_time}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]1 & 1.00 & 1.00 & 1.00 \\ 
  2 & 1.00 & 1.00 & 1.00 \\ 
  3 & 1.00 & 1.00 & 1.00 \\ 
  4 & 1.00 & 1.00 & 1.00 \\ 
  5 & 1.00 & 1.00 & 1.00 \\ 
  6 & 1.00 & 1.00 & 1.00 \\ 
  7 & 1.00 & 1.00 & 1.00 \\ 
  8 & 1.00 & 1.00 & 1.00 \\ 
  9 & 1.00 & 1.00 & 1.00 \\ 
  10 & 1.00 & 1.00 & 1.00 \\ 
  11 & 1.00 & 1.00 & 1.00 \\ 
  12 & 1.00 & 1.00 & 1.00 \\ 
  13 & 1.00 & 1.00 & 1.00 \\ 
  14 & 1.00 & 1.00 & 1.00 \\ 
  15 & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables/rand_time_case_4.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Wed Apr 21 23:50:26 2021
\begin{table}[h!]
\centering
\caption{Adjusted Rand Index across time} 
\label{rand_time}
\begin{tabular}{cccc}
  \hline \\[-1.8ex] & 1 & 2 & 3 \\ 
  \hline \hline \\[-1.8ex]1 & 1.00 & 1.00 & 1.00 \\ 
  2 & 1.00 & 1.00 & 1.00 \\ 
  3 & 1.00 & 1.00 & 1.00 \\ 
  4 & 1.00 & 1.00 & 1.00 \\ 
  5 & 1.00 & 1.00 & 1.00 \\ 
  6 & 1.00 & 1.00 & 1.00 \\ 
  7 & 1.00 & 1.00 & 1.00 \\ 
  8 & 1.00 & 1.00 & 1.00 \\ 
  9 & 1.00 & 1.00 & 1.00 \\ 
  10 & 1.00 & 1.00 & 1.00 \\ 
  11 & 1.00 & 1.00 & 1.00 \\ 
  12 & 1.00 & 1.00 & 1.00 \\ 
  13 & 1.00 & 1.00 & 1.00 \\ 
  14 & 1.00 & 1.00 & 1.00 \\ 
  15 & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
